Topology Estimation Following Islanding and its Impact on Preventive Control of Cascading Failure

Knowledge of power grid's topology during cascading failure is an essential element of centralized blackout prevention control, given that multiple islands are typically formed, as a cascade progresses. Moreover, academic research on interdependency between cyber and physical layers of the grid indicate that power failure during a cascade may lead to outages in communication networks, which progressively reduce the observable areas. These challenge the current literature on line outage detection, which assumes that the grid remains as a single connected component. We propose a new approach to eliminate that assumption. Following an islanding event, first the buses forming that connected components are identified and then further line outages within the individual islands are detected. In addition to the power system measurements, observable breaker statuses are integrated as constraints in our topology identification algorithm. The impact of error propagation on the estimation process as reliance on previous estimates keeps growing during cascade is also studied. Finally, the estimated admittance matrix is used in preventive control of cascading failure, creating a closed-loop system. The impact of such an interlinked estimation and control on that total load served is studied for the first time. Simulations in IEEE-118 bus system and 2,383-bus Polish network demonstrate the effectiveness of our approach.

==> MyBib1.tex <==


%%================================Phulpin CLS and Balarko WFS===========================
@INPROCEEDINGS{phulpin_vfdroop, 
author={Jing Dai and Yannick Phulpin and Alain Sarlette and Damien Ernst}, 
booktitle={17th Power Systems Computation Conference}, 
title={Voltage control in an {HVDC} system to share primary frequency reserves between non-synchronous areas}, 
year={2011}, 
keywords={frequency control ; multi-terminal HVDC system ; primary frequency reserve}, 
month={August},}

@ARTICLE{CLSpoint, 
author={Y. Phulpin}, 
journal={IEEE Transactions on Power Systems}, 
title={Communication-Free Inertia and Frequency Control for Wind Generators Connected by an {HVDC}-Link}, 
year={2012}, 
volume={27}, 
number={2}, 
pages={1136-1137}, 
keywords={HVDC power convertors;frequency control;offshore installations;power generation control;voltage control;wind power plants;HVDC link;communication-free control;communication-free inertia;dc voltage control;frequency control;offshore converter;offshore frequency deviations;onshore frequency deviations;wind generators;Frequency control;Frequency conversion;Generators;Voltage control;Wind farms;Wind power generation;Wind turbines;Frequency control;HVDC transmission;inertia control;wind power generation}, 
doi={10.1109/TPWRS.2011.2175817}, 
ISSN={0885-8950}, 
month={May},}

@ARTICLE{CLSMTDC, 
author={B. Silva and C. L. Moreira and L. Seca and Y. Phulpin and J. A. Pecas Lopes}, 
journal={IEEE Transactions on Sustainable Energy}, 
title={Provision of Inertial and Primary Frequency Control Services Using Offshore Multiterminal {HVDC} Networks}, 
year={2012}, 
volume={3}, 
number={4}, 
pages={800-808}, 
keywords={HVDC power convertors;HVDC power transmission;frequency control;offshore installations;power generation control;power transmission control;voltage control;wind power plants;DC voltage regulation;cascading control mechanism;frequency regulation;inertia emulation;inertial frequency control service;nonsynchronous areas;offshore converters;offshore multiterminal HVDC networks;offshore wind farms;onshore converters;primary frequency control service;Frequency control;Frequency conversion;HVDC transmission;Mathematical model;Wind power generation;Frequency control;HVDC power transmission;inertial emulation;multiterminal HVDC system;offshore wind generation}, 
doi={10.1109/TSTE.2012.2199774}, 
ISSN={1949-3029}, 
month={Oct},}

@INPROCEEDINGS{freqdev_ss, 
author={I. M. Sanz and B. Chaudhuri and G. Strbac}, 
booktitle={2014 IEEE PES General Meeting | Conference Exposition}, 
title={Frequency changes in {AC} systems connected to {DC} grids: Impact of {AC} vs. {DC} side events}, 
year={2014}, 
pages={1-5}, 
keywords={HVDC power convertors;HVDC power transmission;frequency control;power grids;power system control;AC side disturbance;AC side events;AC systems;DC side disturbance;DC side events;DIgSILENT PowerFactory;MTDC grid;autonomous power sharing;converter station;four terminal DC grid model;frequency changes;frequency support;frequency variation;multiterminal DC grid;offshore wind farms;power frequency droop control;Analytical models;Frequency control;Frequency conversion;Power conversion;Simulation;Wind farms;AC/DC interaction;Multi-Terminal DC (MTDC);VSC-HVDC;frequency droop control}, 
doi={10.1109/PESGM.2014.6939914}, 
ISSN={1932-5517}, 
month={July},}

@ARTICLE{inertialWFS, 
author={I. Martínez Sanz and B. Chaudhuri and G. Strbac}, 
journal={IEEE Transactions on Power Systems}, 
title={Inertial Response From Offshore Wind Farms Connected Through {DC} Grids}, 
year={2015}, 
volume={30}, 
number={3}, 
pages={1518-1527}, 
keywords={DC-AC power convertors;offshore installations;power cables;power grids;wind power plants;wind turbines;4-terminal DC grid;WTG;communication-less approach;dc grids;frequency variations;inertial response;offshore converters;offshore wind farms;onshore AC system;onshore AC systems;point-to-point DC links;remote offshore wind farms;sub-sea cables;weighted frequency scheme;wind turbine generator;Frequency control;Generators;Optical frequency conversion;Voltage control;Wind farms;Wind turbines;DC grid;droop control;frequency support;inertial response;offshore wind farm;voltage source converter (VSC)}, 
doi={10.1109/TPWRS.2014.2349739}, 
ISSN={0885-8950}, 
month={May},}



%%================================Van Cutsem etc===========================
@INPROCEEDINGS{V_F_droop_coupling, 
author={S. Akkari and J. Dai and M. Petit and X. Guillaud}, 
booktitle={2015 IEEE Eindhoven PowerTech}, 
title={Coupling between the frequency droop and the voltage droop of an {AC/DC} converter in an {MTDC} system}, 
year={2015}, 
pages={1-6}, 
keywords={AC-DC power convertors;HVDC power convertors;couplings;frequency control;power generation control;power generation faults;power generation reliability;power grids;voltage control;5-terminal HVDC grid;AC grid frequency regulation;AC side fault;AC-DC converter frequency droop coupling;AC-DC converter voltage droop coupling;DC side fault;MTDC system reliability;frequency droop control technique;voltage droop control technique;Frequency control;Frequency conversion;HVDC transmission;Power conversion;Time-frequency analysis;Voltage control;HVDC;MTDC;frequency control;voltage control}, 
doi={10.1109/PTC.2015.7232285}, 
month={June},}

@INPROCEEDINGS{integrate, 
author={L. Papangelis and X. Guillaud and T. V. Cutsem}, 
booktitle={11th IET International Conference on AC and DC Power Transmission}, 
title={Frequency support among asynchronous {AC} systems through {VSCs} emulating power plants}, 
year={2015}, 
pages={1-9}, 
keywords={HVDC power convertors;HVDC power transmission;frequency control;frequency convertors;power grids;power plants;voltage control;HVDC grid;VSC;asynchronous AC system;frequency deviation detection;frequency droop characteristics;frequency support;high voltage direct current grid;integral control;power plant;voltage droop control;voltage source converter;HVDC grid;frequency support;integral control;speed droop;speed governor;voltage source converter}, 
doi={10.1049/cp.2015.0033}, 
month={Feb},}

@article{Receding_horizon,
title = "A receding horizon approach to incorporate frequency support into the {AC}/{DC} converters of a multi-terminal {DC} grid ",
journal = "Electric Power Systems Research ",
volume = "148",
number = "",
pages = "1 - 9",
year = "2017",
note = "",
issn = "0378-7796",
doi = "https://doi.org/10.1016/j.epsr.2017.03.007",
author = "Lampros Papangelis and Marie-Sophie Debry and Patrick Panciatici and Thierry Van Cutsem",
keywords = "Multi-terminal \{DC\} grid",
keywords = "Voltage source converter",
keywords = "Frequency support",
keywords = "Receding Horizon Control "
}

@INPROCEEDINGS{Receding_horizon_IEEE, 
author={L. Papangelis and M. S. Debry and T. Van Cutsem and P. Panciatici}, 
booktitle={2017 IEEE Manchester PowerTech}, 
title={Local control of {AC}/{DC} converters for frequency support between asynchronous {AC} areas}, 
year={2017}, 
volume={}, 
number={}, 
pages={1-6}, 
keywords={AC-DC power convertors;HVDC power transmission;power grids;power transmission control;AC/DC converter control;DC voltage droop;HVDC grids;asynchronous AC areas;model predictive control;voltage source converter;Frequency control;Frequency conversion;Frequency measurement;HVDC transmission;Steady-state;Voltage control;Voltage measurement;Model Predictive Control;Multi-Terminal Direct Current grid;frequency support;secondary frequency control;voltage droop}, 
doi={10.1109/PTC.2017.7980876}, 
ISSN={}, 
month={June},}

@article{frequency_containment,
title = "Decentralized model predictive control of voltage source converters for {AC} frequency containment",
journal = "International Journal of Electrical Power \& Energy Systems",
volume = "98",
pages = "342 - 349",
year = "2018",
issn = "0142-0615",
doi = "https://doi.org/10.1016/j.ijepes.2017.12.015",
author = "Lampros Papangelis and Marie-Sophie Debry and Thibault Prevost and Patrick Panciatici and Thierry Van Cutsem",
keywords = "Voltage source converter, Frequency support, Model predictive control, Multi-terminal DC grid, Point-to-point HVDC link"
}

%%================================Phulpina and coordinated control=================================
@INPROCEEDINGS{delayimpacts, 
author={J. Dai and Y. Phulpin and A. Sarlette and D. Ernst}, 
booktitle={2010 IREP Symposium Bulk Power System Dynamics and Control - VIII (IREP)}, 
title={Impact of delays on a consensus-based primary frequency control scheme for {AC} systems connected by a multi-terminal {HVDC} grid}, 
year={2010}, 
pages={1-9}, 
keywords={HVDC power transmission;delays;frequency control;power grids;power transmission control;DC grid;delays;frequency deviations;frequency measurement;multi-terminal HVDC grid;non synchronous AC systems;power injections;primary frequency control;Converters;Delay;Frequency control;Frequency measurement;HVDC transmission;Mathematical model;Power system dynamics}, 
doi={10.1109/IREP.2010.5563281}, 
month={Aug},}



@article{cooperative_FC,
title = "Cooperative frequency control with a multi-terminal high-voltage {DC} network ",
journal = "Automatica ",
volume = "48",
number = "12",
pages = "3128 - 3134",
year = "2012",
note = "",
issn = "0005-1098",
doi = "https://doi.org/10.1016/j.automatica.2012.08.017",
author = "Alain Sarlette and Jing Dai and Yannick Phulpin and Damien Ernst",
keywords = "Power system control",
keywords = "Frequency control",
keywords = "HVDC systems",
keywords = "Decentralized control "
}

@ARTICLE{coordinated_PFC, 
author={J. Dai and Y. Phulpin and A. Sarlette and D. Ernst}, 
journal={IET Generation, Transmission Distribution}, 
title={Coordinated primary frequency control among non-synchronous systems connected by a multi-terminal high-voltage direct current grid}, 
year={2012}, 
volume={6}, 
number={2}, 
pages={99-108}, 
keywords={HVDC power transmission;frequency control;high-voltage engineering;load regulation;power grids;power transmission control;DC grid;closed-loop system;control theory community;coordinated primary frequency control;distributed control scheme;frequency deviation;load imbalance;multiterminal high voltage direct current grid;nonsynchronous AC area;power injection;stability analysis}, 
doi={10.1049/iet-gtd.2011.0312}, 
ISSN={1751-8687}, 
month={February},}

@article{coordinated_FC,
title = "Coordinated Frequency Control through {MTDC} Transmission Systems",
journal = "IFAC-PapersOnLine",
volume = "48",
number = "22",
pages = "106 - 111",
year = "2015",
note = "",
issn = "2405-8963",
doi = "http://dx.doi.org/10.1016/j.ifacol.2015.10.315",
author = "Martin Andreasson and Roger Wiget and Dimos V. Dimarogonas and Karl H. Johansson and Göran Andersson",
}

@ARTICLE{distributed_FC, 
author={M. Andreasson and R. Wiget and D. V. Dimarogonas and K. H. Johansson and G. Andersson}, 
journal={IEEE Transactions on Power Systems}, 
title={Distributed Frequency Control Through {MTDC} Transmission Systems}, 
year={2017}, 
volume={32}, 
number={1}, 
pages={250-260}, 
keywords={HVDC power transmission;decentralised control;distributed control;frequency control;minimisation;power generation control;power grids;power system stability;power transmission control;synchronous machines;voltage control;HVDC grid distributed cable model;IEEE 14 bus network;MTDC grid voltage regulation;MTDC transmission system;asynchronous AC system restoration reserve;decentralized communication-free version;distributed dynamic controller;distributed frequency control;global quadratic power generation cost function minimized;multiterminal HVDC grid;nominal DC voltage;nominal frequency;power system high-order dynamic model;six-terminal HVDC grid;swing equation;synchronous machine;Frequency control;HVDC transmission;Mathematical model;Power system dynamics;Power system stability;Stability analysis;Voltage control;Distributed control;HVDC transmission;power system dynamics;power system stability}, 
doi={10.1109/TPWRS.2016.2555939}, 
ISSN={0885-8950}, 
month={Jan},}

@ARTICLE{distributed_PI, 
author={F. D. Bianchi and J. L. Domnguez-Garca}, 
journal={IEEE Transactions on Sustainable Energy}, 
title={Coordinated Frequency Control Using {MT}-{HVDC} Grids With Wind Power Plants}, 
year={2016}, 
volume={7}, 
number={1}, 
pages={213-220}, 
keywords={HVDC power transmission;frequency control;wind power plants;AC grids;MT-HVDC grids;coordinated frequency control;multiterminal high-voltage direct current systems;wind power generation;wind power plants;Frequency control;HVDC transmission;Power demand;Power system dynamics;Power system stability;Wind power generation;Wind turbines;Distributed control;grid integration;multiterminal high-voltage direct current (HVDC) grids;multiterminal high-voltage direct current (HVDC)grids;primary frequency support;wind power plants (WPPs)}, 
doi={10.1109/TSTE.2015.2488098}, 
ISSN={1949-3029}, 
month={Jan},}

@article{distributedMPC,
title = "Distributed {MPC} for frequency regulation in multi-terminal {HVDC} grids ",
journal = "Control Engineering Practice ",
volume = "46",
number = "",
pages = "176 - 187",
year = "2016",
note = "",
issn = "0967-0661",
doi = "https://doi.org/10.1016/j.conengprac.2015.11.001",
author = "Paul Mc Namara and Rudy R. Negenborn and Bart De Schutter and Gordon Lightbody and Seán McLoone",
keywords = "Distributed model predictive control",
keywords = "Convergence",
keywords = "Stability",
keywords = "Modal analysis",
keywords = "Auxiliary problem principle",
keywords = "Automatic generation control",
keywords = "Multi-terminal \{HVDC\} "
}

@ARTICLE{MPCAGC, 
author={P. McNamara and F. Milano}, 
journal={IEEE Transactions on Power Systems}, 
title={Model Predictive Control based {AGC} for Multi-terminal {HVDC}-connected {AC} grids}, 
year={2017}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Automatic generation control;Delays;Frequency control;HVDC transmission;Power system dynamics;Synchronous generators;Voltage control;Automatic Generation Control;Model Predictive Control;Multi-terminal HVDC}, 
doi={10.1109/TPWRS.2017.2694768}, 
ISSN={0885-8950}, 
month={},}

@ARTICLE{pilotDCreg, 
author={A. Kirakosyan and E. F. El-Saadany and M. S. El Moursi and K. Al Hosani}, 
journal={IEEE Transactions on Power Delivery}, 
title={{DC} Voltage Regulation and Frequency Support in Pilot Voltage Droop Controlled Multi Terminal {HVDC} Systems}, 
year={2017}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Frequency control;Frequency conversion;Frequency locked loops;Power conversion;Voltage control;Voltage measurement;DC voltage deviation;FLL;Multi Terminal HVDC;droop control;grid synchronization;pilot voltage droop;primary frequency response}, 
doi={10.1109/TPWRD.2017.2759302}, 
ISSN={0885-8977}, 
month={},}

%%============================cazythings============================

@ARTICLE{VSG_adaptive, 
author={R. Wang and L. Chen and T. Zheng and S. Mei}, 
journal={CSEE Journal of Power and Energy Systems}, 
title={{VSG}-based adaptive droop control for frequency and active power regulation in the {MTDC} system}, 
year={2017}, 
volume={3}, 
number={3}, 
pages={260-268}, 
keywords={Adaptive systems;Frequency control;HVDC transmission;Power generation;Radio spectrum management;Voltage control;Wind farms;Adaptive droop control;MTDC;frequency regulation;unbalanced power allocation;virtual inertial.}, 
doi={10.17775/CSEEJPES.2017.00040}, 
ISSN={}, 
month={Sept},}

@ARTICLE{adaptive_freq, 
author={W. Wang and Y. Li and Y. Cao and U. Haeger and C. Rehtanz}, 
journal={IEEE Transactions on Power Systems}, 
title={Adaptive Droop Control of {MTDC} System for Frequency Support and Power Sharing}, 
year={2017}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Control systems;Frequency control;Power conversion;Power system stability;Voltage control;Wind farms;Adaptive droop control;VSC based multi-terminal direct current (VSC-MTDC);frequency regulation;virtual inertia;voltage droop control;voltage source converter (VSC)}, 
doi={10.1109/TPWRS.2017.2719002}, 
ISSN={0885-8950}, 
month={},}

@ARTICLE{redistribution, 
author={H. Dong and Z. Xu and P. Song and G. Tang and Q. Xu and L. Sun}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={Optimized Power Redistribution of Offshore Wind Farms Integrated {VSC}-{MTDC} Transmissions After Onshore Converter Outage}, 
year={2017}, 
volume={64}, 
number={11}, 
pages={8948-8958}, 
keywords={HVDC power convertors;HVDC power transmission;offshore installations;optimisation;pitch control (position);power generation control;power generation reliability;power grids;power transmission control;power transmission reliability;wind power plants;VSC;VSC-MTDC transmissions;ac system disturbance;asynchronous grids;auxiliary pitch angle control;combined offshore wind farm control strategy;dc grid operating point setting;dc system converter outage;flexible control characteristics;frequency performance;gigawatt offshore wind energy;inertia control;large-scale clean electricity;modified New England 39-bus system;multiterminal HVDC transmission;nonself-distributed scenario;onshore ac grids;onshore converter outage;optimized power redistribution calculation;optimized power redistribution method;power system;renewable sources;self-distributed type outage;sensitive cluster identification;seven terminal VSC-HVDC transmission system;simulation verifications;successive power impulses;voltage source converter;Frequency control;Frequency conversion;Power conversion;Voltage control;Wind energy;Wind farms;Converter outage;frequency stability improvement;gigawatt offshore wind farm (WF);optimized power redistribution;sensitive cluster (SC);voltage source converter based multiterminal HVDC (VSC-MTDC)}, 
doi={10.1109/TIE.2016.2631136}, 
ISSN={0278-0046}, 
month={Nov},}

@article{WFandMTDC,
author = {Yujun Li and Zhao Xu},
title = {Coordinated Control of Wind Farms and {MTDC} Grids for System Frequency Support},
journal = {Electric Power Components and Systems},
volume = {45},
number = {4},
pages = {451-464},
year  = {2017},
publisher = {Taylor & Francis},
doi = {10.1080/15325008.2016.1264500},}



%%================================ Our papers==============================================

@INPROCEEDINGS{controlled, 
author={S. G. Vennelaganti and N. R. Chaudhuri}, 
booktitle={2018 IEEE Power Energy Society General Meeting}, 
title={Controlled Primary Frequency Support for Asynchronous {AC} Areas through an {MTDC} Grid}, 
year={accepted}, 
keywords={Frequency Support; Frequency Droop; MTDC;HVDC;VSC}, 
}

@ARTICLE{ratiobased, 
author={S. G. Vennelaganti and N. R. Chaudhuri}, 
journal={Early access in IEEE Transactions on Power Systems}, 
title={Ratio-based Selective Inertial and Primary Frequency Support through {MTDC} Grids with Offshore Wind Farms}, 
year={2018}, 
volume={}, 
number={}, 
pages={}, 
keywords={Frequency control;Frequency conversion;Frequency estimation;Frequency synchronization;Power system dynamics;Voltage control;Wind farms;Droop;Frequency support;HVDC;Inertial support;MTDC;VSC;Wind farm}, 
doi={10.1109/TPWRS.2018.2850145}, 
ISSN={0885-8950}, 
month={},}

@ARTICLE{selective, 
author={S. G. Vennelaganti and N. R. Chaudhuri}, 
journal={IEEE Transactions on Power Systems}, 
title={Selective Power Routing in {MTDC} Grids for Inertial and Primary Frequency Support}, 
year={submitted}, 
keywords={MPC; MTDC; Droop; VSC; HVDC; Inertial support; Frequency support}, 
}


@ARTICLE{adaptiveman, 
author={N. R. Chaudhuri and B. Chaudhuri}, 
journal={IEEE Transactions on Power Systems}, 
title={Adaptive Droop Control for Effective Power Sharing in Multi-Terminal {DC} ({MTDC}) Grids}, 
year={2013}, 
volume={28}, 
number={1}, 
pages={21-29}, 
keywords={adaptive control;mathematics computing;modal analysis;power convertors;power grids;power system control;power system stability;voltage control;DC link voltage control loops;EMTDC-PSCAD;MTDC grid;Matlab-Simulink;adaptive droop control;bipolar converter;converter outage;effective power sharing;healthy converter stations;inverter outages;metallic return;modal analysis;multiterminal DC grid;power mismatch-burden;power-voltage droop;stability analysis;transient simulation;Adaptation models;Analytical models;Mathematical model;Power system stability;Stability analysis;Steady-state;Voltage control;Autonomous power sharing;droop;modal analysis;multi-terminal DC (MTDC);stability;voltage source converter (VSC)}, 
doi={10.1109/TPWRS.2012.2203390}, 
ISSN={0885-8950}, 
month={Feb},}

@ARTICLE{droopman, 
author={R. G. de Almeida and J. A. Pecas Lopes}, 
journal={IEEE Transactions on Power Systems}, 
title={Participation of Doubly Fed Induction Wind Generators in System Frequency Regulation}, 
year={2007}, 
volume={22}, 
number={3}, 
pages={944-950}, 
keywords={frequency control;wind turbines;active power;deloaded optimum power extraction curve;doubly fed induction wind generator;pitch control;rotor speed;static converter;system frequency regulation;wind turbine;Control systems;Frequency control;Induction generators;Mesh generation;Power generation;Power systems;Synchronous generators;Wind energy;Wind energy generation;Wind power generation;Dynamic behavior;primary frequency control;wind generation}, 
doi={10.1109/TPWRS.2007.901096}, 
ISSN={0885-8950}, 
month={Aug}}

@ARTICLE{offshore, 
author={S. V. Bozhko and R. Blasco-Gimenez and R. Li and J. C. Clare and G. M. Asher}, 
journal={IEEE Transactions on Energy Conversion}, 
title={Control of Offshore {DFIG}-Based Wind Farm Grid With Line-Commutated {HVDC} Connection}, 
year={2007}, 
volume={22}, 
number={1}, 
pages={71-78}, 
keywords={EMTP;HVDC power transmission;asynchronous generators;commutation;control system synthesis;fault diagnosis;machine control;offshore installations;power generation control;power grids;power system CAD;static VAr compensators;wind power plants;collection bus;doubly fed induction generator control;electromagnetic transient program simulation;formal control design;high voltage direct current connection;line commutated HVDC connection;offshore DFIG-based wind farm grid;power system computer-aided design;static compensator;Control design;Control system synthesis;HVDC transmission;Induction generators;Power system faults;Power system modeling;Power system simulation;Power system transients;STATCOM;Wind farms;Controller design;doubly fed induction generator (DFIG);frequency;high-voltage direct current (HVDC) transmission;stability;static compensator (STATCOM);voltage;wind energy}, 
doi={10.1109/TEC.2006.889544}, 
ISSN={0885-8969}, 
month={March}}

@ARTICLE{5688311, 
author={H. Zhou and G. Yang and J. Wang}, 
journal={IEEE Transactions on Energy Conversion}, 
title={Modeling, Analysis, and Control for the Rectifier of Hybrid {HVdc} Systems for {DFIG}-Based Wind Farms}, 
year={2011}, 
volume={26}, 
number={1}, 
pages={340-353}, 
keywords={HVDC power transmission;PI control;asynchronous generators;commutation;compensation;constant current sources;eigenvalues and eigenfunctions;power generation control;power system simulation;rectifiers;wind power plants;DFIG-based wind farm;current source inverter subsystem;double loop control;doubly fed induction generator;eigenvalue analysis method;hybrid HVDC system;inverse system control;line-commutated rectifier control;propotional-integral controller;rectifier subsystem;state variable model;switchable phase-lead compensator;Analytical models;Automatic voltage control;Converters;HVDC transmission;Inverters;Wind farms;Doubly fed induction generator (DFIG);hybrid HVdc;line-commutated converter (LCC-HVdc);offshore wind farm;rectifier}, 
doi={10.1109/TEC.2010.2096819}, 
ISSN={0885-8969}, 
month={March}}

@INPROCEEDINGS{7286452, 
author={M. Zhang and X. Yuan and J. Hu and S. Wang and Shicong Ma and Q. He and Jun Yi}, 
booktitle={2015 IEEE Power Energy Society General Meeting}, 
title={Wind power transmission through {LCC-HVDC} with wind turbine inertial and primary frequency supports}, 
year={2015}, 
pages={1-5}, 
keywords={HVDC power convertors;asynchronous generators;load flow control;wind power plants;wind turbines;HVDC power flow;LCC-HVDC;PLL;doubly fed induction generators;line commutated converter HVDC link;positive feedback characteristic;wind power transmission;wind turbine inertial support;wind turbine primary frequency support;Frequency control;HVDC transmission;Load modeling;Phase locked loops;Voltage control;Wind power generation;Wind turbines;Doubly fed induction generator (DFIG);high voltage dc (HVDC) transmission;inertia support;primary frequency control;wind power transmission}, 
doi={10.1109/PESGM.2015.7286452}, 
ISSN={1932-5517}, 
month={July},}

@INPROCEEDINGS{5157546, 
author={Honglin Zhou and Geng Yang}, 
booktitle={2009 IEEE 6th International Power Electronics and Motion Control Conference}, 
title={Control of {DFIG}-based wind farms with hybrid {HVDC} connection}, 
year={2009}, 
pages={1085-1091}, 
keywords={HVDC power convertors;asynchronous generators;invertors;machine control;power generation control;static VAr compensators;wind power plants;DFIG-based wind farms control;STATCOM;ac fault;black-start capability;current source inverter;doubly fed induction generator;hybrid HVDC connection;line-commutated converter;reactive power support;static synchronous compensator;voltage source converter;wind energy system;Automatic voltage control;Converters;Couplings;HVDC transmission;Induction generators;Inverters;Power conversion;Stators;Topology;Wind farms}, 
doi={10.1109/IPEMC.2009.5157546}, 
month={May}}

@ARTICLE{4453977, 
author={S. Bozhko and G. Asher and R. Li and J. Clare and L. Yao}, 
journal={IEEE Transactions on Energy Conversion}, 
title={Large Offshore {DFIG}-Based Wind Farm With Line-Commutated {HVDC} Connection to the Main Grid: Engineering Studies}, 
year={2008}, 
volume={23}, 
number={1}, 
pages={119-127}, 
keywords={HVDC power convertors;asynchronous generators;commutation;offshore installations;power system CAD;power system control;power system simulation;static VAr compensators;wind power plants;EMTDC simulations;PSCAD simulations;STATCOM;large offshore DFIG;large offshore doubly fed induction generator;line-commutated HVDC connection;line-commutated high-voltage dc connection;onshore grid;wind farm;Automatic voltage control;Capacitors;Control system synthesis;DC generators;EMTDC;HVDC transmission;Induction generators;Mesh generation;PSCAD;Wind farms;Controller design;STATCOM;doubly fed induction generator (DFIG);frequency;high-voltage dc (HVdc) transmission;stability;voltage;wind energy}, 
doi={10.1109/TEC.2007.914155}, 
ISSN={0885-8969}, 
month={March}}

@INPROCEEDINGS{1633632, 
author={L. Ran and D. Xiang and L. Hu and K. Abbott}, 
booktitle={The 8th IEE International Conference on AC and DC Power Transmission}, 
title={Voltage stability of an { HVDC} system for a large offshore wind farm with {DFIGs}}, 
year={2006}, 
pages={150-154}, 
keywords={HVDC power convertors;asynchronous generators;frequency control;machine control;offshore installations;reactive power control;rectifying circuits;time-domain analysis;wind power plants;DFIG control;HVDC rectifier control system;excitation control;frequency regulation;offshore wind farm;reactive power control;reactive power-voltage characteristics;stator flux linkage;time domain simulation;voltage stability}, 
doi={10.1049/cp:20060031}, 
ISSN={0537-9989}, 
month={March}}

@ARTICLE{5688311, 
author={H. Zhou and G. Yang and J. Wang}, 
journal={IEEE Transactions on Energy Conversion}, 
title={Modeling, Analysis, and Control for the Rectifier of Hybrid HVdc Systems for DFIG-Based Wind Farms}, 
year={2011}, 
volume={26}, 
number={1}, 
pages={340-353}, 
keywords={HVDC power transmission;PI control;asynchronous generators;commutation;compensation;constant current sources;eigenvalues and eigenfunctions;power generation control;power system simulation;rectifiers;wind power plants;DFIG-based wind farm;current source inverter subsystem;double loop control;doubly fed induction generator;eigenvalue analysis method;hybrid HVDC system;inverse system control;line-commutated rectifier control;propotional-integral controller;rectifier subsystem;state variable model;switchable phase-lead compensator;Analytical models;Automatic voltage control;Converters;HVDC transmission;Inverters;Wind farms;Doubly fed induction generator (DFIG);hybrid HVdc;line-commutated converter (LCC-HVdc);offshore wind farm;rectifier}, 
doi={10.1109/TEC.2010.2096819}, 
ISSN={0885-8969}, 
month={March}}

@ARTICLE{1564232, 
author={Dawei Xiang and Li Ran and J. R. Bumby and P. J. Tavner and S. Yang}, 
journal={IEEE Transactions on Power Delivery}, 
title={Coordinated control of an {HVDC} link and doubly fed induction generators in a large offshore wind farm}, 
year={2006}, 
volume={21}, 
number={1}, 
pages={463-471}, 
keywords={HVDC power transmission;asynchronous generators;frequency control;machine control;offshore installations;power generation control;power transmission control;wind power plants;wind turbines;HVDC link;coordinated control;doubly fed induction generators;economic variable-speed solution;frequency regulation;generator control;grid voltage reference;high-voltage dc transmission;large offshore wind farm;machine control;power tracking;wind turbines;AC generators;Control systems;HVDC transmission;Induction generators;Mesh generation;Power generation economics;Topology;Voltage control;Wind farms;Wind turbines;Doubly fed induction generator;frequency;high-voltage dc (HVdc) transmission;real and reactive power;voltage;wind energy}, 
doi={10.1109/TPWRD.2005.858785}, 
ISSN={0885-8977}, 
month={Jan}}

@INPROCEEDINGS{5484066, 
author={H. Yin and L. Fan}, 
booktitle={41st North American Power Symposium}, 
title={Modeling and control of {DFIG}-based large offshore wind farm with {HVDC}-link integration}, 
year={2009}, 
pages={1-5}, 
keywords={HVDC transmission;Induction generators;Mathematical model;Rectifiers;Rotors;Stators;Tracking loops;Voltage control;Wind energy;Wind farms;DFIG;GSC;HVDC-link;RSC;Wind Farm}, 
doi={10.1109/NAPS.2009.5484066}, 
month={Oct}}

@ARTICLE{5629392, 
author={L. Wang and K. H. Wang}, 
journal={IEEE Transactions on Power Systems}, 
title={Dynamic Stability Analysis of a {DFIG}-Based Offshore Wind Farm Connected to a Power Grid Through an {HVDC} Link}, 
year={2011}, 
volume={26}, 
number={3}, 
pages={1501-1510}, 
keywords={HVDC power transmission;asynchronous generators;control system synthesis;damping;eigenvalues and eigenfunctions;electric current control;power generation control;power grids;time-frequency analysis;wind power plants;wind turbines;DFIG-based OWF;DFIG-based offshore wind farm;HVDC link;OWF;RCR;aggregation method;designed damping controller;doubly-fed induction generator;dynamic stability analysis;eigenvalue calculations;equivalent gearbox;equivalent wind turbine;frequency-domain approach;line-commutated high-voltage direct-current link;modal control theory;power 80 MW;power grid;rectifier current regulator;time-domain scheme;wind speeds;Converters;Damping;Eigenvalues and eigenfunctions;HVDC transmission;Mathematical model;Wind speed;Wind turbines;Doubly-fed induction generator;eigenvalue analysis;high-voltage direct-current;nonlinear model simulations;offshore wind farm;rectifier current regulator}, 
doi={10.1109/TPWRS.2010.2085053}, 
ISSN={0885-8950}, 
month={Aug},}

@INPROCEEDINGS{5948524, 
author={H. Yin and L. Fan and Z. Miao}, 
booktitle={IEEE 2011 EnergyTech}, 
title={Coordination between {DFIG}-based wind farm and {LCC-HVDC} transmission considering limiting factors}, 
year={2011}, 
pages={1-6}, 
keywords={HVDC power convertors;HVDC power transmission;asynchronous generators;reactive power;rectifying circuits;thyristor applications;time-domain analysis;wind power plants;DFIG-based wind farm;HVDC converters;HVDC rectifier voltage;LCC-HVDC transmission;Matlab-Simulink;doubly-fed induction generator;power 200 MW;thyristor-based line current commuting;time-domain simulation;Electromagnetics;Rectifiers;DFIG;LCC-HVDC;Reactive Power}, 
doi={10.1109/EnergyTech.2011.5948524}, 
month={May},}

@ARTICLE{fastman, 
author={H. Yin and L. Fan and Z. Miao}, 
journal={IEEE Transactions on Power Delivery}, 
title={Fast Power Routing Through {HVDC}}, 
year={2012}, 
volume={27}, 
number={3}, 
pages={1432-1441}, 
keywords={HVDC power transmission;asynchronous generators;power control;power system control;rectifiers;voltage control;wind power;wind power plants;HVDC power routing;HVDC rectifier ac bus;LCC-HVDC rectifier power order control;Matlab/SimPowersystems;ac fault recovery;ac voltage-mode control;doubly fed induction generator;fast power routing;infinite bus;line current commutating;renewable energy sources;wind farm;wind power;HVDC transmission;Routing;Stators;Synchronous generators;Voltage control;Wind farms;Wind power generation;Doubly fed induction generator (DFIG);high-voltage direct current (HVDC)}, 
doi={10.1109/TPWRD.2012.2197225}, 
ISSN={0885-8977}, 
month={July},}

@ARTICLE{our, 
author={A. Yogarathinam and J. Kaur and N. R. Chaudhuri}, 
journal={IEEE Transactions on Power Delivery}, 
title={Impact of Inertia and Effective Short Circuit Ratio on Control of Frequency in Weak Grids Interfacing {LCC-HVDC} and {DFIG}-based Wind Farms}, 
year={2016}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Frequency control;HVDC transmission;Integrated circuit modeling;Inverters;Mathematical model;Voltage control;Wind farms;Averaged Model;DFIG.;ESCR;Eigenvalue Sensitivity;Participation Factor;Weak Grid}, 
doi={10.1109/TPWRD.2016.2607205}, 
ISSN={0885-8977}, 
month={},}


@article{ABBReview03,
   Author = {Andersson, G.  and Green, T.  and Pal, B.  and Rehtanz, C},
   Title = {Advanced {C}ontrol of {F}lexible {AC} {T}ransmission {S}ystems},
   Journal = {ABB Review},
   Volume = {4},
   Pages = {21-26},
 Year = {2003} }

@article{TPWRS03Mixedsenlocal,
   Author = {Chaudhuri, B. and Pal, B.C. and Zolotas, A.C. and Jaimoukha, I.M. and Green, T.C.},
   Title = {Mixed-sensitivity approach to {H}-infinity control of power system oscillations employing multiple {FACTS} devices},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {18},
   Number = {3},
   Pages = {1149-1156},
   Year = {2003} }
@article{TPWRS04WAMSdelay,
   Author = {Chaudhuri, B. and Majumder, R. and Pal, B.C.},
   Title = {Wide-area measurement-based stabilizing control of power system considering signal transmission delay},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {4},
   Pages = {1971-1979},
   Year = {2004} }
@article{TPWRS04Multiplemodes,
   Author = {Chaudhuri, B. and Pal, B.C.},
   Title = {Robust damping of multiple swing modes employing global stabilizing signals with a {TCSC}},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {1},
   Pages = {499-506},
   Year = {2004} }
@inproceedings{AutoCong04,
   Author = {Chaudhuri, B. and Korba, P. and Pal, B.C.},
   Title = {Damping controller design through simultaneous stabilization technique},
   BookTitle = {World Automation Congress},
   Volume = {16},
   Pages = {13-18},
 Year = {2004} }

@article{TCST04MMAC,
   Author = {Chaudhuri, B. and Majumder, R. and Pal, B.C.},
   Title = {Application of multiple-model adaptive control strategy for robust damping of interarea oscillations in power system},
   Journal = {IEEE Transactions on Control Systems Technology},
   Volume = {12},
   Number = {5},
   Pages = {727-736},
   Year = {2004} }

@article{GTD04Simstab,
   Author = {Pal, B. C. and Chaudhuri, B. and Zolotas, A.C. and Jaimoukha, I.M.},
   Title = {Simultaneous stabilisation approach for power system damping control design through {TCPAR} employing global signals},
   Journal = {IEE Proceedings - Generation, Transmission and Distribution},
   Volume = {151},
   Number = {1},
   Pages = {43-50},
   Year = {2004} }

@article{TPWRS05PCA,
   Author = {Anaparthi, K.K. and Chaudhuri, B. and Thornhill, N.F. and Pal, B.C.},
   Title = {Coherency Identification in Power Systems Through Principal Component Analysis},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {20},
   Number = {3},
   Pages = {1658-1660},
   Year = {2005} }

@phdthesis{PhDthesis05,
   Author = {Chaudhuri, Balarko},
   Title = {Robust control of inter-area oscillations in power systems using {FACTS} controllers},
   Note = {Balarko Chaudhuri.
   Thesis (Ph.D.) - Department of Electrical and Electronic
   Engineering, Imperial College, London 2005.},
   Type = {PhD Thesis},
   Year = {2005} }

@article{TPWRS05MMAC,
   Author = {Majumder, R. and Chaudhuri, B. and Pal, B.C.},
   Title = {A probabilistic approach to model-based adaptive control for damping of interarea oscillations},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {20},
   Number = {1},
   Pages = {367-374},
   Year = {2005} }

@article{TCST05USPdelay,
   Author = {Majumder, R. and Chaudhuri, B. and Pal, B.C. and Zhong, Qing-Chang},
   Title = {A unified Smith predictor approach for power system damping control design using remote signals},
   Journal = {IEEE Transactions on Control Systems Technology},
   Volume = {13},
   Number = {6},
   Pages = {1063-1068},
   Year = {2005} }

@article{GTD05Loopshaping,
   Author = {Majumder, R. and Chaudhuri, B. and El-Zobaidi, H. and Pal, B. C. and Jaimoukha, I.M.},
   Title = {{LMI} approach to normalised {H}-infinity loop-shaping design of power system damping controllers},
   Journal = {IEE Proceedings - Generation, Transmission and Distribution},
   Volume = {152},
   Number = {6},
   Pages = {952-960},
   Year = {2005} }

@book{Book05,
   Author = {Pal, Bikash and Chaudhuri, Balarko},
   Title = {Robust control in power systems},
   Publisher = {Springer},
   Address = {New York},
   Series = {Power electronics and power systems},
   Year = {2005} }

@article{TCST07LGQLTR,
   Author = {Zolotas, A.C. and Chaudhuri, B. and Jaimoukha, I.M. and Korba, P.},
   Title = {A Study on {LQG}/{LTR} Control for Damping Inter-Area Oscillations in Power Systems},
   Journal = {IEEE Transactions on Control Systems Technology},
   Volume = {15},
   Number = {1},
   Pages = {151-160},
   Year = {2007} }

@article{TPWRS06HILRajat,
   Author = {Majumder, R. and Pal, B. C. and Dufour, C. and Korba, P.},
   Title = {Design and real-time implementation of robust {FACTS} controller for damping inter-area oscillation},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {21},
   Number = {2},
   Pages = {809-816},
   Year = {2006}}

@article{GTD07implementationdelay,
   Author = {Majumder, R. and Chaudhuri, B. and Pal, B.C.},
   Title = {Implementation and test results of a wide-area measurement-based controller for damping interarea
   oscillations considering signal-transmission delay},
   Journal = {IET - Generation, Transmission and Distribution},
   Volume = {1},
   Number = {1},
   Pages = {1-7},
   Year = {2007} }

@inproceedings{PESGM07realtimePetr,
   Author = {Korba, P. and Larsson, M. and Chaudhuri, B. and Pal, B. and Majumder, R. and Sadikovic, R. and Andersson, G.},
   Title = {Towards Real-time Implementation of Adaptive Damping Controllers for {FACTS} Devices},
   BookTitle = {IEEE Power Engineering Society General Meeting, 2007, Tampa},
   Year = {2007} }

@inproceedings{PES08SignalSelection,
   Author = {Ray, S. and Chaudhuri, B. and Majumder, R.},
   Title = {Appropriate Signal Selection for Damping Multi-modal Oscillations Using Low Order Controllers},
   BookTitle = {proceedings of IEEE Power Engineering Society General Meeting, 2008, Pittsburgh},
   Year = {2008} }

@article{SMCCompClassicalvsAdaptive,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Chaudhuri, B. and Majumder, R.},
   Title = {Comparison of Adaptive Critic-Based and Classical Wide-Area Controllers for Power Systems},
   Journal = {IEEE Transactions on Systems, Man, and Cybernetics, Part B},
   Volume = {38},
   Number = {4},
   Pages = {1002-1007},
   Year = {2008} }

@inproceedings{PES09WideAreaPhasorPOD,
   Author = {Ray Chaudhuri, N. and Ray, S. and Majumder, R. and Chaudhuri, B.},
   Title = {A Case Study on Challenges for Robust Wide-area Phasor {POD}},
   BookTitle = {proceedings of IEEE Power Engineering Society General Meeting, 2009, Calgary},
   Year = {2009} }

@article{GTD09PSO,
   Author = {Chaudhuri, B. and Ray, S. and Majumder, R.},
   Title = {Robust low-order controller design for multi-modal power oscillation damping using flexible {AC} transmission systems devices},
   Journal = {IET Generation, Transmission \& Distribution},
   Volume = {3},
   Number = {5},
   Pages = {448-459},
   Year = {2009} }


@inproceedings{GM04TCSCglobalSignal,
   author = {Chaudhuri, B. and Pal, B.},
   title = {Robust damping of multiple swing modes employing global stabilizing signals with a {TCSC}},
   booktitle = {IEEE Power Engineering Society General Meeting},
   volume = {2},
   pages = {1709},
   year = {2004}}

@inproceedings{GM06Real-time,
   author = {Majumder, R. and Chaudhuri, B. and Pal, B. C. and Dufour, C.},
   title = {Real time dynamic simulator for power system control applications},
   booktitle = {IEEE Power Engineering Society General Meeting},
   pages = {7},
   year = {2006}}

@article{Alex_Selftuning2009,
   author = {Domahidi, A. and Chaudhuri, B. and Korba, P. and Majumder, R. and Green, T. C.},
   title = {Self-tuning flexible ac transmission system controllers for power oscillation damping: a case study in real time},
   journal = {IET Generation, Transmission & Distribution},
   volume = {3},
   number = {12},
   pages = {1079-1089},
   year = {2009}}

@article{DroopControlMicroGrid2010,
   author = {Majumder, R. and Chaudhuri, B. and Ghosh, A. and Ledwich, G. and Zare, F.},
   title = {Improvement of Stability and Load Sharing in an Autonomous Microgrid Using Supplementary Droop Control Loop},
   journal = {IEEE Transactions on Power Systems},
   volume = {25},
   number = {2},
   pages = {796-808},
   year = {2010}}


@article{Phasor_Modeshape_10,
   author = {Chaudhuri, N. R. and Chaudhuri, B.},
   title = {Damping and Relative Mode-Shape Estimation in Near Real-Time Through Phasor Approach},
   journal = {IEEE Transactions on Power Systems},
   volume = {26},
   number = {1},
   pages = {364-373},
   year = {2011}}


@article{MTDC_Model_10,
   Author = {Chaudhuri, N. R. and Majumder, R. and Chaudhuri, B. and Jiuping, Pan},
   Title = {Stability Analysis of {VSC} {MTDC} Grids Connected to Multimachine {AC} Systems},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {26},
   Number = {4},
   Pages = {2774-2784},
   Year = {2011} }

@article{Copy_TPWRD_10,
   author = {Chaudhuri, N. R. and Chakraborty, D. and Chaudhuri, B.},
   title = {An Architecture for FACTS Controllers to Deal With Bandwidth-Constrained Communication},
   journal = {IEEE Transactions on Power Delivery},
   volume = {26},
   number = {1},
   pages = {188-196},
   year = {2011}}

@article{Copy_TCST_10,
    Author = {Chaudhuri, N. R. and Chakrabarty, D. and Chaudhuri, B.},
    Title = {Damping Control in Power Systems under Constrained Communication Bandwidth: A Predictor Corrector Strategy},
    Journal = {in Early Access in IEEE Transactions on Control Systems Technology},
    year={2012},
    month={Jan},
    volume={20},
    number={1},
    pages={223-231}
    }

@ARTICLE{Xunqi-08-GilbertModel,
author={Xunqi Yu and Modestino, J.W. and Xusheng Tian},
journal={IEEE Transactions on Information Theory},
title={The Accuracy of Markov Chain Models in Predicting Packet-Loss Statistics for a Single Multiplexer},
year={2008},
month={Jan},
volume={54},
number={1},
pages={489-501}}

@article{SelfTuneNordic_10,
    Author = {Chaudhuri, N. R. and Domahidi, A. and Majumder, R. and Chaudhuri, B. and Korba, P. and Ray, S. and Uhlen, K.},
    Title = {Wide-area Power Oscillation Damping Control in Nordic Equivalent System},
    journal = {IET Generation, Transmission & Distribution},
    volume = {4},
    number = {10},
    pages = {1139-1150},
    year = {2010}}

@article{MTDC_Model_GM11,
   Author = {Chaudhuri, N. R. and Majumder, R. and Chaudhuri, B. and Pan, J. and Nuqui, R.},
   Title = {Modeling and Stability Analysis of {MTDC} Grids for Offshore Wind Farms: A Case Study on the North Sea Benchmark System},
   Journal = {to appear in Proceedings of IEEE PES General Meeting, 2011}}

@article{MTDC_Droop_11,
    Author = {Chaudhuri, N. R. and Majumder, R. and Chaudhuri, B. and Pan, J. and Nuqui, R.},
    Title = {Adaptive Droop Control for Effective Power Sharing in Multi-terminal {DC} {(MTDC)} Grids},
    Journal = {accepted for publication in IEEE Transactions on Power Systems}}

%%======================================================================================

%%==============================Books===================================================
@book{Nilanjan_14_MTDC_book,
   author = {Chaudhuri, Nilanjan Ray and Chaudhuri, Balarko and Majumder, Rajat and Yazdani, Amirnaser},
   title = {Multi-terminal Direct Current Grids : Modeling, Analysis, and Control},
   publisher = {Wiley/IEEE Press},
   address = {Oxford},
   Year = {2014} }

@book{MPC_book,
   author = {Karl Johan Astrom and Bjorn Wittenmark },
   title = {Adaptive Control},
   publisher = {Addison-Wesley},
   edition = {2nd ed.},
   Year = {1995 } }

@book{Yazdani_10_VSCinPowerSystem,
   author = {Yazdani, Amirnaser and Iravani, Reza},
   title = {Voltage-sourced converters in power systems : modeling, control, and applications},
   publisher = {Wiley},
   address = {Oxford},
   Year = {2010} }

@book{Mohan_03_PowerElectronics,
   author = {Mohan, Ned and Undeland, Tore M. and Robbins, William P.},
   title = {Power electronics : converters, applications, and design},
   publisher = {Wiley},
   address = {Hoboken, N.J. ; [Chichester]},
   edition = {3rd ed.},
   year = {2003}}

@book{Overschee_96_SubspaceIdent,
   Author = {Overschee, Peter van and Moor, Bart L. R. de},
   Title = {Subspace identification for linear systems : theory, implementation, applications},
   Publisher = {Kluwer Academic},
   Address = {Boston ; London},
   Year = {1996} }

@book{Ljung_99_SystemIdent,
   Author = {Ljung, Lennart},
   Title = {System identification: theory for the user},
   Publisher = {Prentice Hall PTR; London : Prentice-Hall International},
   Address = {Upper Saddle River, N.J.},
   Edition = {2nd ed.},
   Year = {1999} }

@book{Hsia_77_SystemIdent,
   Author = {Hsia, T. C.},
   Title = {System identification: least-squares method},
   Publisher = {Lexington Books},
   Address = {[S.l.]},
      Year = {1977} }

@book{Montgomery,
   author = {Montgomery, Douglas C.},
   title = {Design and analysis of experiments},
   publisher = {John Wiley \& Sons},
   address = {Hoboken},
   edition = {7th ed.},
   year = {2009}
}

@book{Arrillaga,
   author = {Arrillaga, J. and Liu, Y. H. and Watson, N. R.},
   title = {Flexible power transmission: the {HVDC} options},
   publisher = {John Wiley},
   year = {2007}
}

@book{Kailath,
   author = {Kailath, T.},
   title = {Linear systems},
   publisher = {Prentice-Hall},
   address = {Englewood Cliffs; London},
   year = {1980}
}

@book{Sood,
   author = {Sood, Vijay K.},
   title = {{HVDC} and {FACTS} controllers: applications of static converters in power systems},
   publisher = {Kluwer Academic Publishers},
   address = {Boston; London},
   year = {2004}
}


@book{Bhattacharyya,
   Author = {Bhattacharyya, S. P. and Chapellat, H. and Keel, L. H.},
   Title = {Robust control : the parametric approach},
   Publisher = {Prentice Hall ;
   Prentice-Hall International},
   Address = {Upper Saddle River London ;},
   Year = {1995} }

@book{Tsong,
   Author = {Chen, Chi-Tsong},
   Title = {Linear system theory and design},
   Publisher = {Oxford University Press},
   Address = {New York; Oxford},
   Edition = {3rd},
   Year = {1999} }

@book{GreenLimebeer,
   Author = {Green, Michael and Limebeer, David J. N.},
   Title = {Linear robust control},
   Publisher = {Prentice Hall ;
   Prentice-Hall International},
   Address = {Englewood Cliffs London ;},
   Year = {1995} }

@book{Hingorani,
   Author = {Hingorani, N. G. and Gyugyi, L.},
   Title = {Understanding {FACTS}: concepts and technology of flexible AC transmission systems},
   Publisher = {IEEE Press},
   Address = {New York},
   Year = {2000} }




@book{Kundur,
   Author = {Kundur, P.},
   Title = {Power system stability and control},
   Publisher = {McGraw-Hill},
   Address = {New York; London},
   Series = {The EPRI power system engineering series},
   Year = {1994} }

@book{Kuo,
   Author = {Kuo, Benjamin C. and Golnaraghi, Farid},
   Title = {Automatic control systems},
   Publisher = {Wiley},
   Address = {New York ; Chichester},
   Edition = {8th},
   Year = {2003} }

@book{McFarlaneGlover,
   Author = {McFarlane, D. C. and Glover, K.},
   Title = {Robust controller design using normalized coprime factor plant descriptions},
   Publisher = {Springer-Verlag},
   Address = {Berlin; London},
   Series = {Lecture notes in control and information sciences ; 138},
   Year = {1990} }

@book{Padiyar,
   Author = {Padiyar, K. R.},
   Title = {Power system dynamics : stability and control},
   Publisher = {John Wiley ;
   Interline Publishing},
   Address = {Singapore
   Bangalore},
   Year = {1996} }

@book{Rogers,
   Author = {Rogers, Graham},
   Title = {Power system oscillations},
   Publisher = {Kluwer Academic},
   Address = {Boston; London},
   Year = {2000} }

@book{Boyd,
   Author = {S. Boyd and L. El Ghaoui and E. Feron and Balakrishnan, V.},
   Title = {Linear matrix inequalities in system and control theory},
   Publisher = {Society for Industrial and Applied Mathematics},
   Address = {Philadelphia},
   Series = {SIAM studies in applied mathematics ; v.15},
   Year = {1994} }

@book{Pai,
   Author = {Sauer, Peter W. and Pai, M. A.},
   Title = {Power system dynamics and stability},
   Publisher = {Prentice Hall},
   Address = {Upper Saddle River, N.J.},
   Year = {1998} }

@book{Skogestad,
   Author = {Skogestad, Sigurd and Postlethwaite, Ian},
   Title = {Multivariable feedback control: analysis and design},
   Publisher = {Wiley},
   Address = {Chichester},
   Year = {1996} }

@book{Smith,
   Author = {Smith, O.J.M.},
   Title = {Feedback Control Systems},
   Publisher = {McGraw-Hill Book Company, Inc.},
   Address = {New York},
   Year = {1958} }

@book{Song,
   Author = {Song, Yong-Hua and Johns, A. T.},
   Title = {Flexible ac transmission systems ({FACTS})},
   Publisher = {Institution of Electrical Engineers},
   Address = {London},
   Series = {IEE power and energy series ; v. 30},
   Year = {1999} }

@book{Zhou,
   Author = {Zhou, Kemin and Doyle, John C. and Glover, K.},
   Title = {Robust and optimal control},
   Publisher = {Prentice Hall ;
   Prentice-Hall International},
   Address = {Upper Saddle River
   London ;},
   Year = {1996} }

@book{Stoica,
  author        = {Torsten S\"oderstr\"om and Petre Stoica},
  title         = "System Identification",
  publisher     = "Prentice Hall International",
  year          = "1989"
};

@book{Zarrop,
  author        = "P. E. Wellstead and M. B. Zarrop",
  title         = "Self-tuning Systems. Control and Signal Processing",
  publisher     = "John Wiley \& Sons",
  year          = "1991"
}; %address       = "Chichester, UK",

@book{Godfrey,
    author = "Keith Godfrey",
    title = "Perturbation Signals for System Identification",
    year = "1993",
    publisher = "Prentice Hall"
};

@book{Blanke-Fault-tolerant,
   Author = {Blanke, Mogens and Kinnaert, Michel and Lunze, Jan and Staroswiecki, Marcel and Schroeder, Jochen},
   Title = {Diagnosis and fault-tolerant control},
   Publisher = {Springer},
   Address = {Berlin; New York},
   Edition = {2nd ed.},
   Year = {2006} }


@book{Hagan-Martin,
   Author = {Hagan, Martin T. and Demuth, Howard B. and Beale, Mark H.},
   Title = {Neural network design},
   Publisher = {PWS Pub},
   Address = {Boston ; London},
   Year = {1996} }

@book{NN-FLLewis,
   Author = {Kim, Y. H. and Lewis, Frank L.},
   Title = {High-level feedback control with neural networks},
   Publisher = {World Scientific},
   Address = {Singapore ; London},
   Series = {World scientific series in robotics and intelligent systems},
   Year = {1998} }

@book{Astrom,
   Author = {Astrom, Karl J. and Wittenmark, Bjorn},
   Title = {Adaptive control},
   Publisher = {Addison-Wesley},
   Address = {Reading, Mass. ; Wokingham},
   Edition = {2nd ed.},
   Year = {1995} }

@book{Haykin,
   Author = {Haykin, Simon S.},
   Title = {Adaptive filter theory},
   Publisher = {Prentice Hall},
   Address = {Englewood Cliffs, N.J. ; London},
   Edition = {3rd ed.},
   Series = {Prentice Hall information and system sciences series},
   Year = {1995} }

%%======================================================================================


%%==============================Inter-area Oscillation==================================


@article{Kundur91funda,
   Author = {Klein, M. and Rogers, G.J. and Kundur, P.},
   Title = {A fundamental study of inter-area oscillations in power systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {6},
   Number = {3},
   Pages = {914-921},
   Year = {1991} }



@article{Paserba96Cigre,
   Author = {Paserba, J.},
   Title = {Analysis and control of power system oscillation},
   Journal = {Cigre special publication},
   Volume = {Technical brochure 111},
 Year = {1996} }

@article{Kundur_04_stability_definition,
   Author = {Kundur, P. and Paserba, J. and Ajjarapu, V. and Andersson, G. and Bose, A. and Canizares, C. and Hatziargyriou, N. and Hill, D. and Stankovic, A. and Taylor, C. and Van Cutsem, T. and Vittal, V.},
   Title = {Definition and classification of power system stability IEEE/CIGRE joint task force on stability terms and definitions},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {19},
   Number = {3},
   Pages = {1387-1401},
   Year = {2004} }



 %%=======================================================================================



 %%==================================WAMS=================================================

@article{Taylor-05-WACSDemo,
   author = {Taylor, C. W. and Erickson, D. C. and Martin, K. E. and Wilson, R. E. and Venkatasubramanian, V.},
   title = {WACS-Wide-Area Stability and Voltage Control System: {R\&D} and Online Demonstration},
   journal = {Proceedings of the IEEE},
   volume = {93},
   number = {5},
   pages = {892-906},
   year = {2005}}

 @article{Andersson_96_RobustDampingFuzzy,
   Author = {Noroozian, M. and Andersson, G. and Tomsovic, K.},
   Title = {Robust, near time-optimal control of power system oscillations with fuzzy logic},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {11},
   Number = {1},
   Pages = {393-400},
   Year = {1996} }

@article{Debokda_08_WideareaUPFC,
   Author = {Ray, S. and Venayagamoorthy, G. K.},
   Title = {Wide-Area Signal-Based OptimalNeurocontroller for a UPFC},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {23},
   Number = {3},
   Pages = {1597-1605},
   Year = {2008} }

@article{Ericsson_04_UtilityWAN,
   Author = {Ericsson, G. N.},
   Title = {Communication requirements - basis for investment in a utility wide-area network},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {19},
   Number = {1},
   Pages = {92-95},
   Year = {2004} }


 @article{McCalley96GlobalSignals,
   Author = {Aboul-Ela, M.E. and Sallam, A.A. and McCalley, J.D. and Fouad, A.A.},
   Title = {Damping controller design for power system oscillations using global signals},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {11},
   Number = {2},
   Pages = {767-773},
   Year = {1996} }

@inproceedings{Hauer05ExperienceNorthAmerica,
   Author = {Cai, J.Y. and Huang, Zhenyu and Hauer, J. and Martin, K.},
   Title = {Current Status and Experience of {WAMS} Implementation in North America},
   BookTitle = {IEEE-PES Transmission and Distribution Conference and Exhibition: Asia and Pacific},
   Pages = {1-7},
   Year = {2005} }

@article{IEEECSM00Chow,
   Author = {Chow, J.H. and Sanchez-Gasca, J.J. and Ren, Haoxing and Wang, Shaopeng},
   Title = {Power system damping controller design-using multiple input signals},
   Journal = {IEEE Control Systems Magazine},
   Volume = {20},
   Number = {4},
   Pages = {82-90},
   Year = {2000} }

@inproceedings{Hauer04WAMS03Blackout,
   Author = {Hauer, J.F. and Bhatt, N.B. and Shah, K. and Kolluri, S.},
   Title = {Performance of {WAMS East} in providing dynamic information for the North East blackout of August 14, 2003},
   BookTitle = {IEEE Power Engineering Society General Meeting },
   Volume = {2},
   Pages = {1685-1690},
   Year = {2004} }

@inproceedings{Kamwa_00_SMES_damping,
   Author = {Heniche, A. and Kamwa, I.},
   Title = {Using global control and {SMES} to damp inter-area oscillations: an exploratory assessment},
   BookTitle = {IEEE Power Engineering Society Summer Meeting},
   Volume = {3},
   Pages = {1872-1876},
   Year = {2000} }

@article{Vittal_01_solution_crisis,
   Author = {Heydt, G.T. and Liu, C.C. and Phadke, A.G. and Vittal, V.},
   Title = {Solution for the crisis in electric power supply},
   Journal = {IEEE Computer Applications in Power},
   Volume = {14},
   Number = {3},
   Pages = {22-30},
   Year = {2001} }

@inproceedings{Kamwa_98_multiloop_PSS,
   Author = {Kamwa, I. and Gerin-Lajoie, L. and Trudel, G.},
   Title = {Multi-loop power system stabilizers using wide-area synchronous phasor measurements},
   BookTitle = {American Control Conference},
   Volume = {5},
   Pages = {2963-2967},
   Year = {1998} }

@article{Kamwa01WideAreaHierarchical,
   Author = {Kamwa, I. and Grondin, R. and Hebert, Y.},
   Title = {Wide-area measurement based stabilizing control of large power systems-a decentralized/hierarchical approach},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {16},
   Number = {1},
   Pages = {136-153},
   Year = {2001} }

@inproceedings{Mekki_00_signal_loss,
   Author = {Mekki, K. and Snyder, A.F. and HadjSaid, N. and Feuillet, R. and Georges, D. and Margotin, T.},
   Title = {Damping controller input-signal loss effects on the wide-area stability of an interconnected power system},
   BookTitle = {IEEE Power Engineering Society Summer Meeting},
   Volume = {2},
   Pages = {1015-1019},
   Year = {2000} }

@article{Vittal_02_future_reliability,
   Author = {Xie, Zhaoxia and Manimaran, G. and Vittal, V. and Phadke, A.G. and Centeno, V.},
   Title = {An information architecture for future power systems and its reliability analysis},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {17},
   Number = {3},
   Pages = {857-863},
   Year = {2002} }

@article{Xie06ChineseSystem,
   Author = {Xie, Xiaorong and Xin, Yaozhong and Xiao, Jinyu and Wu, Jingtao and Han, Yingdao},
   Title = {{WAMS} applications in Chinese power systems},
   Journal = {IEEE Power and Energy Magazine},
   Volume = {4},
   Number = {1},
   Pages = {54-63},
   Year = {2006} }

@inproceedings{Yuan05RTMonitoring,
   Author = {Yuan, Yue and Ju, Ping and Li, Qiang and Wang, Yongzhi and Hu, Hongbo and Sasaki, H.},
   Title = {A Real-time Monitoring Method for Power System Steady State Angle Stability Based on {WAMS}},
   BookTitle = {The 7th International Power Engineering Conference, IPEC 2005 },
   Pages = {1-4},
   Year = {2005} }

@article{Korba07GTDMonitoring,
   Author = {Korba, P.},
   Title = {Real-time monitoring of electromechanical oscillations in power systems: first findings},
   Journal = {IET Proceedings - Generation, Transmission and Distribution},
   Volume = {1},
   Number = {1},
   Pages = {80-88},
   Year = {2007} }

@article{Korba05WAMSWACS,
   Author = {Zima, M. and Larsson, M. and Korba, P. and Rehtanz, C. and Andersson, G.},
   Title = {Design Aspects for Wide-Area Monitoring and Control Systems},
   Journal = {Proceedings of the IEEE},
   Volume = {93},
   Number = {5},
   Pages = {980-996},
   Year = {2005} }

@inproceedings{KjetilPSCE09,
   Author = {Johansson, E. and Uhlen, K. and Leirbukt, A. B. and Korba, P. and Gjerde, J. O. and Vormedal, L. K.},
   Title = {Coordinating power oscillation damping control using wide area measurements},
   BookTitle = {proceedings of IEEE/PES Power Systems Conference and Exposition, PSCE '09},
   Year = {2009} }

@inproceedings{KorbaPSCE06,
   Author = {Leirbukt, A. B. and Gjerde, J. O. and Korba, P. and Uhlen, K. and Vormedal, L. K. and Warland, L.},
   Title = {Wide Area Monitoring Experiences in {N}orway},
   BookTitle = {proceedings of IEEE PES Power Systems Conference and Exposition, PSCE '06},
   Pages = {353-360},
   Year = {2006} }

@article{Kamwa05PSS4B,
   Author = {Kamwa, I. and Grondin, R. and Trudel, G.},
   Title = {{IEEE} {PSS2B} versus {PSS4B}: the limits of performance of modern power system stabilizers},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {20},
   Number = {2},
   Pages = {903-915},
   Year = {2005} }








%%=========================================================================================


%%============================Self-Tuning Control==========================================
@article{Worden_95_oversampling,
   Author = {Worden, K.},
   Title = {On the over-sampling of data for system identification},
   Journal = {Mechanical Systems and Signal Processing},
   Volume = {9},
   Number = {3},
   Pages = {287-297},
   Note = {doi: DOI: 10.1006/mssp.1995.0024},
      Year = {1995} }


@article{Auto73Astrom,
   Author = {Astrom, K. J. and Wittenmark, B.},
   Title = {On self tuning regulators},
   Journal = {Automatica},
   Volume = {9},
   Number = {2},
   Pages = {185-199},
   Year = {1973} }

@article{Borison79mulvarAutomatica,
   Author = {Borison, Ulf},
   Title = {Self-tuning regulators for a class of multivariable systems},
   Journal = {Automatica},
   Volume = {15},
   Number = {2},
   Pages = {209-215},
   Year = {1979} }

@article{Koivo80multvarAutomatica,
   Author = {Koivo, H. N.},
   Title = {A multivariable self-tuning controller},
   Journal = {Automatica},
   Volume = {16},
   Number = {4},
   Pages = {351-366},
   Year = {1980} }

@article{Penttinen80multvarAutomatica,
   Author = {Penttinen, J. and Koivo, H. N.},
   Title = {Multivariable tuning regulators for unknown systems},
   Journal = {Automatica},
   Volume = {16},
   Number = {4},
   Pages = {393-398},
   Year = {1980} }

@article{TPWRS88Malik,
  author        = "S. Cheng and Y. S. Chow and O. P. Malik and G. S. Hope",
  title         = "An Adaptive Synchronous Machine Stabilizer",
  journal       = "IEEE Transactions on Power Systems",
  volume        = "1",
  number        = "3",
  year          = "1986",
  pages         = "101-109"
};

@article{TAC84Malik,
   Author = {Kanniah, J. and Malik, O. and Hope, G.},
   Title = {Self-tuning regulator based on dual-rate sampling},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {29},
   Number = {8},
   Pages = {755-759},
   Year = {1984} }

@article{Prabhu88adaptPSS,
   Author = {Bandyopadhyay, G. and Prabhu, S.S.},
   Title = {A new apporach to adaptive power system stabilizers},
   Journal = {Electric Machines and Power Systems},
   Volume = {14},
   Pages = {111-125},
   Year = {1988} }

@article{TPWRS88MalikMulti-machine,
   Author = {Chandra, A. and Malik, O.P. and Hope, G.S.},
   Title = {A self-tuning controller for the control of multi-machine power systems},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {3},
   Number = {3},
   Pages = {1065-1071},
   Year = {1988} }

@article{TPWRS88MalikMultimodalDualrate,
   Author = {Cheng, S.J. and Malik, O.P. and Hope, G.S.},
   Title = {Damping of multi-modal oscillations in power systems using a dual-rate adaptive stabilizer},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {3},
   Number = {1},
   Pages = {101-108},
   Year = {1988} }

@article{TPWRS90IdowuModelRefAdapt,
   Author = {Ghandakly, A.A. and Idowu, P.},
   Title = {Design of a model reference adaptive stabilizer for the exciter and governor loops of power generators},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {5},
   Number = {3},
   Pages = {887-893},
   Year = {1990} }

@article{TEC91MalikImpl,
   Author = {Chandra, A. and Wong, K.K. and Malik, O.P. and Hope, G.S.},
   Title = {Implementation and test results of a generalized self-tuning excitation controller},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {6},
   Number = {1},
   Pages = {186-192},
   Year = {1991} }

@inproceedings{Malik_91_fuzzy_PSS,
   Author = {Hassan, M.A.M. and Malik, O.P. and Hope, G.S.},
   Title = {A fuzzy logic based self-tuned power system stabilizer},
   BookTitle = {Third International Conference on Power System Monitoring and Control},
   Pages = {146-151},
   Year = {1991} }

@article{TEC91MalikMultVar,
   Author = {Pahalawaththa, N.C. and Hope, G.S. and Malik, O.P.},
   Title = {Multivariable self-tuning power system stabilizer simulation and implementation studies},
   Journal = { IEEE Transactions on Energy Conversion},
   Volume = {6},
   Number = {2},
   Pages = {310-319},
   Year = {1991} }

@article{IEECTA93MalikSelfOptPS,
   Author = {Malik, O.P. and Chen, G.P. and Hope, G.S. and Qin, Y.H. and Xu, G.Y.},
   Title = {Adaptive self-optimising pole shifting control algorithm},
   Journal = {IEE Proceedings - Control Theory and Applications},
   Volume = {139},
   Number = {5},
   Pages = {429-438},
   Year = {1992} }

@article{TEC93MalikSelfOptPoleShift,
   Author = {Chen, G.P. and Malik, O.P. and Hope, G.S. and Qin, Y.H. and Xu, G.Y.},
   Title = {An adaptive power system stabilizer based on the self-optimizing pole shifting control strategy},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {8},
   Number = {4},
   Pages = {639-645},
   Year = {1993} }

@article{TEC93MalikLabTests,
   Author = {Hassan, M.A.M. and Malik, O.P.},
   Title = {Implementation and laboratory test results for a fuzzy logic based self-tuned power system stabilizer},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {8},
   Number = {2},
   Pages = {221-228},
   Year = {1993} }

@inproceedings{CDC93Malik,
   Author = {Zeng, Y. and Malik, O.P.},
   Title = {Robust adaptive controller design based on pole-shifting technique},
   BookTitle = {32nd IEEE Conference on Decision and Control},
   Volume = {3},
   Pages = {2353-2357},
   Year = {1993} }

@article{TEC93MalikNeuralNet,
   Author = {Zhang, Y. and Chen, G.P. and Malik, O.P. and Hope, G.S.},
   Title = {An artificial neural network based adaptive power system stabilizer},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {8},
   Number = {1},
   Pages = {71-77},
   Year = {1993} }

@inproceedings{PESGM00Malik,
   Author = {Eichmann, A. and Kohler, A. and Malik, O.P. and Taborda, J.},
   Title = {A prototype self-tuning adaptive power system stabilizer for damping of active power swings},
   BookTitle = {IEEE Power Engineering Society Summer Meeting},
   Volume = {1},
   Pages = {122-126},
   Year = {2000} }

@article{TEC04Malik,
   Author = {Ramakrishna, G. and Malik, O.P.},
   Title = {Radial basis function identifier and pole-shifting controller for power system stabilizer application},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {19},
   Number = {4},
   Pages = {663-670},
   Year = {2004} }

@inproceedings{PES07Korba,
   Author = {Korba, P. and Larsson, M. and Chaudhuri, B. and Pal, B. and Majumder, R. and Sadikovic, R. and Andersson, G.},
   Title = {Towards Real-time Implementation of Adaptive Damping Controllers for {FACTS} Devices},
   BookTitle = {proceedings of IEEE Power Engineering Society General Meeting, Tampa},
   Year = {2007} }

@inproceedings{PES06Sadikovic,
   Author = {Sadikovic, R. and Korba, P. and Andersson, G.},
   Title = {Self-tuning controller for damping of power system oscillations with {FACTS} devices},
   BookTitle = {proceedings of IEEE Power Engineering Society General Meeting, Montreal},
   Year = {2006} }

@article{Fortescue,
  author        = "T. R. Fortescue and L. S. Kershenbaum and B. E. Ydstie",
  title         = "Implementation of self-tuning regulators with variable forgetting factors",
  journal       = "Automatica",
  volume        = "17",
  year          = "1981",
  pages         = "831-835"
}

@inproceedings{Korba03Kalman,
   Author = {Korba, P. and Larsson, M. and Rehtanz, C.},
   Title = {Detection of oscillations in power systems using Kalman filtering techniques},
   BookTitle = {Proceedings of 2003 IEEE Conference on Control Applications, CCA 2003},
   Volume = {1},
   Pages = {183-188},
   Year = {2003} }

@article{Auto81Fortescue,
   Author = {Fortescue, T. R. and Kershenbaum, L. S. and Ydstie, B. E.},
   Title = {Implementation of self-tuning regulators with variable forgetting factors},
   Journal = {Automatica},
   Volume = {17},
   Number = {6},
   Pages = {831-835},
   Year = {1981} }


@article{PAS84Ghosh,
   Author = {Ghosh, A. and Ledwich, G. and Malik, O. P. and Hope, G. S.},
   Title = {Power System Stabilizer Based on Adaptive Control Techniques},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {PAS-103},
   Number = {8},
   Pages = {1983-1989},
   Year = {1984} }

@article{InfoSc69Astrom,
   Author = {Astrom, K. J.},
   Title = {On the choice of sampling rates in parametric identification of time series},
   Journal = {Information Sciences},
   Volume = {1},
   Number = {3},
   Pages = {273-278},
   Year = {1969} }






%%==========================================================================================

%%====================NCF and Loop-shaping==================================================
@article{TAC93HydeGlover,
   Author = {Hyde, R.A. and Glover, K.},
   Title = {The application of scheduled {H}-inifinity controllers to a VSTOL aircraft},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {38},
   Number = {7},
   Pages = {1021-1039},
   Year = {1993} }

@inproceedings{IEEEConfCS01Ngamroo,
   Author = {Ngamroo, I.},
   Title = {Design of robust {H}-inifinity PSS via normalized coprime factorization approach},
   BookTitle = {he 2001 IEEE International Symposium on Circuits and Systems, ISCAS 2001},
   Volume = {3},
   Pages = {129-132},
   Year = {2001} }

@inproceedings{CDC88McFarlaneGlover,
   Author = {McFarlane, D. and Glover, K.},
   Title = {An ${calH}_{\infty}$ design procedure using robust stabilization of normalized coprime factors},
   BookTitle = {27th IEEE Conference on Decision and Control},
   Volume ={2},
   Pages = {1343-1348},
   Year = {1988} }

@article{TAC92McFarlaneGlover,
   Author = {McFarlane, D. and Glover, K.},
   Title = {A loop-shaping design procedure using {H}-inifinity synthesis},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {37},
   Number = {6},
   Pages = {759-769},
   Year = {1992} }

@article{TAC00WangChow,
   Author = {Wang, Shaopeng and Chow, J.H.},
   Title = {Low-order controller design for SISO systems using coprime factors and LMI},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {45},
   Number = {6},
   Pages = {1166-1169},
   Year = {2000} }

@article{IEEGTD02Song,
   Author = {Farsangi, M.M. and Song, Y.H. and Fang, W.L. and Wang, X.F.},
   Title = {Robust {FACTS} control design using the {H}-inifinity loop-shaping method},
   Journal = {IEE Proceedings - Generation, Transmission and Distribution},
   Volume = {149},
   Number = {3},
   Pages = {352-358},
   Year = {2002} }

@article{TPWRS03Vittal,
   Author = {Zhu, Chuanjiang and Khammash, M. and Vittal, V. and Qiu, Wenzheng},
   Title = {Robust power system stabilizer design using {H}-inifinity loop shaping approach},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {18},
   Number = {2},
   Pages = {810-818},
   Year = {2003} }

@article{TAC89GloverMcFarlane,
   Author = {Glover, K. and McFarlane, D.},
   Title = {Robust stabilization of normalized coprime factor plant descriptions with {H}-inifinity-bounded uncertainty},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {34},
   Number = {8},
   Pages = {821-830},
   Year = {1989} }

@inproceedings{IEEEPES01Rahim,
   Author = {Rahim, A.H.M.A. and Al-Baiyat, S.A. and Kandlawala, F.M.},
   Title = {A robust STATCOM controller for power system dynamic performance enhancement},
   BookTitle = {Power Engineering Society Summer Meeting, 2001. IEEE},
   Volume = {2},
   Pages = {887-892},
   Year = {2001} }



%%==============================================================================================

%%==============================Robsut Control in Power Systems=================================
@article{zhai2001decentralized,
  title={Decentralized H [infinity] controller design: a matrix inequality approach using a homotopy method* 1},
  author={Zhai, G. and Ikeda, M. and Fujisaki, Y.},
  journal={Automatica},
  volume={37},
  number={4},
  pages={565--572},
  year={2001},
  publisher={Elsevier}
}

@article{chilali2002h,
  title={H? design with pole placement constraints: an LMI approach},
  author={Chilali, M. and Gahinet, P.},
  journal={Automatic Control, IEEE Transactions on},
  volume={41},
  number={3},
  pages={358--367},
  year={1996},
  publisher={IEEE}
}

@article{ramos2004new,
  title={A new methodology for the coordinated design of robust decentralized power system damping controllers},
  author={Ramos, R.A. and Alberto, L.F.C. and Bretas, N.G.},
  journal={Power Systems, IEEE Transactions on},
  volume={19},
  number={1},
  pages={444--454},
  year={2004},
  publisher={IEEE}
}

@article{TPWRS00Martins,
   Author = {Boukarim, G.E. and Wang, Shaopeng and Chow, J.H. and Taranto, G.N. and Martins, N.},
   Title = {A comparison of classical, robust, and decentralized control designs for multiple power system stabilizers},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {15},
   Number = {4},
   Pages = {1287-1292},
   Note = {TY  - JOUR},
   Year = {2000} }

@article{TEC95Malik,
   Author = {Chen, S. and Malik, O.P.},
   Title = {Power system stabilizer design using $\mu$ synthesis},
   Journal = {Energy Conversion, IEEE Transactions on},
   Volume = {10},
   Number = {1},
   Pages = {175-181},
   Year = {1995} }

@inproceedings{ACC95Chow,
   Author = {Chen, Horng-Bin and Shiau, Jaw-Kuen and Chow, J.H.},
   Title = {Simultaneous H-infinity suboptimal control design},
   BookTitle = {American Control Conference},
   Volume = {3},
   Pages = {1946-1950},
   Year = {1995} }

@article{TPWRS99Vittal,
   Author = {Djukanovic, M. and Khammash, M. and Vittal, V.},
   Title = {Sequential synthesis of structured singular value based decentralized controllers in power systems},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {14},
   Number = {2},
   Pages = {635-641},
   Year = {1999} }

@article{TPWRS04Rouco,
   Author = {Elices, A. and Rouco, L. and Bourles, H. and Margotin, T.},
   Title = {Design of Robust Controllers for Damping Interarea Oscillations: Application to the European Power System},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {19},
   Number = {2},
   Pages = {1058-1067},
   Year = {2004} }

@article{IEECTA05Kulkarni,
   Author = {Gupta, R. and Bandyopadhyay, B. and Kulkarni, A.M.},
   Title = {Power system stabiliser for multimachine power system using robust decentralised periodic output feedback},
   Journal = {IEE Proceedings - Control Theory and Applications },
   Volume = {152},
   Number = {1},
   Pages = {3-8},
   Year = {2005} }

@article{CSM89Hauer,
   Author = {Hauer, J.F.},
   Title = {Robust damping controls for large power systems},
   Journal = {Control Systems Magazine, IEEE},
   Volume = {9},
   Number = {1},
   Pages = {12-18},
   Year = {1989} }

@article{TPWRS00Kamwa,
   Author = {Kamwa, I. and Trudel, G. and Gerin-Lajoie, L.},
   Title = {Robust design and coordination of multiple damping controllers using nonlinear constrained optimization},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {15},
   Number = {3},
   Pages = {1084-1092},
   Year = {2000} }

@article{TPWRS95Klein,
   Author = {Klein, M. and Le, L.X. and Rogers, G.J. and Farrokhpay, S. and Balu, N.J.},
   Title = {{H}-inifinity damping controller design in large power systems},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {10},
   Number = {1},
   Pages = {158-166},
   Year = {1995} }

@article{TPWRS01Andersson,
   Author = {Noroozian, M. and Ghandhari, M. and Andersson, G. and Gronquist, J. and Hiskens, I.},
   Title = {A robust control strategy for shunt and series reactive compensators to damp electromechanical oscillations},
   Journal = {Power Delivery, IEEE Transactions on},
   Volume = {16},
   Number = {4},
   Pages = {812-817},
   Year = {2001} }

@article{TPWRS04Ramos,
   Author = {Ramos, R.A. and Alberto, L.F.C. and Bretas, N.G.},
   Title = {A new methodology for the coordinated design of robust decentralized power system damping controllers},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {19},
   Number = {1},
   Pages = {444-454},
   Year = {2004} }

@article{SCL90SeftonGlover,
   Author = {Sefton, J. and Glover, K.},
   Title = {Pole/zero cancellations in the general {H}-inifinity problem with reference to a two block design},
   Journal = {Systems \& Control Letters},
   Volume = {14},
   Number = {4},
   Pages = {295-306},
   Year = {1990} }

@article{TCST95Chow,
   Author = {Taranto, G.N. and Chow, J.H. and Othman, H.A.},
   Title = {Robust redesign of power system damping controllers},
   Journal = {IEEE Transactions on Control Systems Technology},
   Volume = {3},
   Number = {3},
   Pages = {290-298},
   Year = {1995} }

@article{TPWRS95Chow,
   Author = {Taranto, G.N. and Chow, J.H.},
   Title = {A robust frequency domain optimization technique for tuning series compensation damping controllers},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {10},
   Number = {3},
   Pages = {1219-1225},
   Year = {1995} }

@article{IEEGTD97Chow,
   Author = {Taranto, G.N. and Shiau, J.-K. and Chow, J.H. and Othman, H.A.},
   Title = {Robust decentralised design for multiple {FACTS} damping controllers},
   Journal = {IEE Proceedings - Generation, Transmission and Distribution},
   Volume = {144},
   Number = {1},
   Pages = {61-67},
   Year = {1997} }

@inproceedings{ACC01Chow,
   Author = {Wang, Shaopeng and Chow, J.H.},
   Title = {Regional pole placement via low-order controllers with extensions to simultaneous stabilization},
   BookTitle = {American Control Conference},
   Volume = {2},
   Pages = {1663-1668},
   Year = {2001} }

@article{TPWRS95Jiang,
   Author = {Zhao, Qihua and Jiang, Jin},
   Title = {Robust SVC controller design for improving power system damping},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {10},
   Number = {4},
   Pages = {1927-1932},
   Year = {1995} }
%%============================================================================================

%%==============Fixed Structure Control and Simultaneous Stabilization========================

@article{TAC87Bhattacharyya,
   Author = {Biernacki, R. and Hwang, Humor and Bhattacharyya, S.},
   Title = {Robust stability with structured real parameter perturbations},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {32},
   Number = {6},
   Pages = {495-506},
   Year = {1987} }

@inproceedings{ACC95Chow,
   Author = {Chen, Horng-Bin and Shiau, Jaw-Kuen and Chow, J.H.},
   Title = {Simultaneous {H}-inifinity-suboptimal control design},
   BookTitle = {American Control Conference},
   Volume = {3},
   Pages = {1946-1950},
   Year = {1995} }

@article{TPWRS00Pal,
   Author = {Pal, B.C. and Coonick, A.H. and Macdonald, D.C.},
   Title = {Robust damping controller design in power systems with superconducting magnetic energy storage devices},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {15},
   Number = {1},
   Pages = {320-325},
   Year = {2000} }

@article{IEEGTD04Pal,
   Author = {Pal, B.C. and Chaudhuri, B. and Zolotas, A.C. and Jaimoukha, I.M.},
   Title = {Simultaneous stabilisation approach for power system damping control design through TCPAR employing global signals},
   Journal = {IEE Proceedings - Generation, Transmission and Distribution},
   Volume = {151},
   Number = {1},
   Pages = {43-50},
   Year = {2004} }

@article{Automatica86Smith,
   Author = {Smith, M. C. and Sondergeld, K. P.},
   Title = {On the order of stable compensators},
   Journal = {Automatica},
   Volume = {22},
   Number = {1},
   Pages = {127-129},
   Year = {1986} }

@inproceedings{ACC01Chow,
   Author = {Wang, Shaopeng and Chow, J.H.},
   Title = {Regional pole placement via low-order controllers with extensions to simultaneous stabilization},
   BookTitle = {American Control Conference},
   Volume = {2},
   Pages = {1663-1668},
   Year = {2001} }

@article{TPWRS00Taranto-SimultaneousPSSTuningGA,
   Author = {Do Bomfim, A. L. B. and Taranto, G. N. and Falcao, D. M.},
   Title = {Simultaneous tuning of power system damping controllers using genetic algorithms},
   Journal = {EEE Transactions on Power Systems},
   Volume = {15},
   Number = {1},
   Pages = {163-169},
   Year = {2000} }

@article{Geromel_94_decentralized_control,
   Author = {Geromel, J. C. and Bernussou, J. and Peres, P. L. D.},
   Title = {Decentralized control through parameter space optimization},
   Journal = {Automatica},
   Volume = {30},
   Number = {10},
   Pages = {1565-1578},
   Year = {1994} }

%%==============================================================================================

%%==================IEEE Standards==============================================================

@misc{Std06Excitation,
   Title = {{IEEE} Std 421.5 - 2005, {IEEE} Recommended Practice for Excitation System Models for Power System Stability Studies},
   Pages = {1-85},
   Year = {2006} }
 %%=============================================================================================

 %%======================Choice of Remote Signals===============================================
@inproceedings{GM05KamwaWideAreaTechnicalValue,
   Author = {Kamwa, I. and Heniche, A. and Trudel, G. and Dobrescu, M. and Grondin, R. and Lefebvre, D.},
   Title = {Assessing the technical value of {FACTS}-based wide-area damping control loops},
   BookTitle = {proceedings of {IEEE} Power Engineering Society General Meeting, 2005},
   Pages = {1734-1743 Vol. 2},
   Year = {2005} }

 @article{IEEECSM00Chow,
   Author = {Chow, J.H. and Sanchez-Gasca, J.J. and Ren, Haoxing and Wang, Shaopeng},
   Title = {Power system damping controller design-using multiple input signals},
   Journal = {IEEE Control Systems Magazine},
   Volume = {20},
   Number = {4},
   Pages = {82-90},
   Year = {2000} }

@article{Song04Signal,
   Author = {Farsangi, M.M. and Song, Y.H. and Lee, K.Y.},
   Title = {Choice of {FACTS} Device Control Inputs for Damping Interarea Oscillations},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {19},
   Number = {2},
   Pages = {1135-1143},
   Year = {2004} }

@article{Kamwa02Signal,
   Author = {Heniche, A. and Kamwa, I.},
   Title = {Control loops selection to damp inter-area oscillations of electrical networks},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {17},
   Number = {2},
   Pages = {378-384},
   Year = {2002} }

@inproceedings{Kamwa02ICCAsignal,
   Author = {Heniche, A. and Kamwa, I.},
   Title = {Using measures of controllability and observability for input and output selection},
   BookTitle = {International Conference on Control Applications},
   Volume = {2},
   Pages = {1248-1251},
   Year = {2002} }

@article{TPWRS95Larsen,
   Author = {Larsen, E.V. and Sanchez-Gasca, J.J. and Chow, J.H.},
   Title = {Concepts for design of {FACTS} controllers to damp power swings},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {10},
   Number = {2},
   Pages = {948-956},
   Year = {1995} }

@article{Martins90Signal,
   Author = {Martins, N. and Lima, L.T.G.},
   Title = {Determination of suitable locations for power system stabilizers and static VAR compensators for damping electromechanical oscillations in large scale power systems},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {5},
   Number = {4},
   Pages = {1455-1469},
   Year = {1990} }

@article{Mhaskar06Signal,
   Author = {Mhaskar, U.P. and Kulkarni, A.M.},
   Title = {Power oscillation damping using {FACTS} devices: modal controllability, observability in local signals, and location of transfer function zeros},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {21},
   Number = {1},
   Pages = {285-294},
   Year = {2006} }

@article{Pagola89Signal,
   Author = {Pagola, F.L. and Perez-Arriaga, I.J. and Verghese, G.C.},
   Title = {On sensitivities, residues and participations: applications to oscillatory stability analysis and control},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {4},
   Number = {1},
   Pages = {278-285},
   Year = {1989} }

@article{Wang99Signal,
   Author = {Wang, H.F.},
   Title = {Selection of robust installing locations and feedback signals of {FACTS}-based stabilizers in multi-machine power systems},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {14},
   Number = {2},
   Pages = {569-574},
   Year = {1999} }

@inproceedings{Chow02Signal,
   Author = {Wei, Xuan and Chow, J.H. and Sanchez-Gasca, J.J.},
   Title = {On the sensitivities of network variables for {FACTS} device damping control},
   BookTitle = {IEEE Power Engineering Society Winter Meeting},
   Volume = {2},
   Pages = {1188-1193},
   Year = {2002} }

@article{Kamwa08GeoVsRes,
   Author = {Heniche, A. and Kamwa, I.},
   Title = {Assessment of Two Methods to Select Wide-Area Signals for Power System Damping Control},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {2},
   Pages = {572-581},
   Year = {2008} }

@article{Ledwich_96_seqortho,
   Author = {Palmer, E. W. and Ledwich, G.},
   Title = {Optimal placement of angle transducers in power systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {11},
   Number = {2},
   Pages = {788-793},
   Year = {1996} }


%%======================================================================================

%%============================Nordic System=============================================
@inproceedings{PSCE06Nordic,
   Author = {Leirbukt, A. B. and Gjerde, J. O. and Korba, P. and Uhlen, K. and Vormedal, L. K. and Warland, L.},
   Title = {Wide {A}rea {M}onitoring {E}xperiences in {N}orway},
   BookTitle = {IEEE PES Power Systems Conference and Exposition, Atlanta },
   Pages = {353-360},
   Year = {2006} }
%%======================================================================================


%%========================Phasor POD====================================================
@inproceedings{PES2001phasorPOD,
   Author = {Angquist, L. and Gama, C.},
   Title = {Damping algorithm based on phasor estimation},
   BookTitle = {IEEE Power Engineering Society Winter Meeting},
   Volume = {3},
   Pages = {1160-1165},
   Year = {2001} }

@inproceedings{PES03phasorPODEquador,
   Author = {Latorre, H. F. and Angquist, L.},
   Title = {Analysis of {TCSC} providing damping in the interconnection Colombia-Ecuador 230 kV},
   BookTitle = {IEEE Power Engineering Society General Meeting},
   Volume = {4},
   Pages = {2366},
   Year = {2003} }

@inproceedings{CigrePhasorPODBrazil,
   Author = {Gama, C. and Angquist, L. and Ingestrom, G. and Noroozian, M.},
   Title = {Commisioning and operative experience of {TCSC} for damping power oscillation in the Brazilian North-South interconnection},
   BookTitle = {Cigre Session 2000},
   Note = {paper no. 14-104}}


@patent{PhasorPODpatent,
  author        = {Angquist, L.},
  assignee      = {ABB AB},
  address       = {Vasteras, Sweden},
  title         = {Method and A Device For Damping Power Oscillations in Transmission Lines},
  nationality   = {United States},
  number        = {6559561},
  dayfiled      = {20},
  monthfiled    = {March},
  yearfiled     = {2000},
  day           = {6},
  month         = {May},
  year          = {2003}}
  %url          = {http://www.google.com/patents?id=hFcOAAAAEBAJ\&printsec=abstract\&zoom=4\&source=gbs_summary_r\&cad=0_0}}

%%======================================================================================

%%=========================Computational Intelligence Techniques========================

@inproceedings{CNN95KennedyPSO,
   Author = {Kennedy, J. and Eberhart, R.},
   Title = {Particle swarm optimization},
   BookTitle = {IEEE International Conference on Neural Networks},
   Volume = {4},
   Pages = {1942-1948},
   Year = {1995} }

@article{TEC07KumarPSO,
   Author = {del Valle, Y. and Venayagamoorthy, G. K. and Mohagheghi, S. and Hernandez, J. -C. and Harley, R. G.},
   Title = {Particle swarm optimization basic concepts, variants and applications in power system},
   Journal = {IEEE Transactions on Evolutionary Computation},
   Note = {to be published},
   url  = {http://ieeexplore.ieee.org/iel5/4235/26785/101109TEVC2007896686.pdf}}

%%=======================================================================================



%%======================Wide area protection and Emergency Control=======================
@article{Martin_06_wide_area_protection,
   Author = {Adamiak, M. G. and Apostolov, A. P. and Begovic, M. M. and Henville,
   C. F. and Martin, K. E. and Michel, G. L. and
   Phadke A. G. and Thorp J. S.},
   Title = {Wide Area Protection&#8212;Technology and Infrastructures},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {21},
   Number = {2},
   Pages = {601-609},
   Year = {2006} }


@inproceedings{IREP07Miroslav-SIPS,
   Author = {Begovic, Miroslav and Madani, Vahid and Novosel, Damir},
   Title = {System Integrity Protection Schemes {(SIPS)}},
   BookTitle = {iREP Symposium Bulk Power System Dynamics and Control - VII. Revitalizing Operational Reliability},
   Editor = {Madani, Vahid},
   Year = {2007} }


@inproceedings{PES07Miroslav-WAP,
   Author = {Begovic, Miroslav and Novosel, Damir},
   Title = {On Wide Area Protection},
   BookTitle = { IEEE Power Engineering Society General Meeting},
   Editor = {Novosel, Damir},
   Year = {2007} }

@article{Begovic_05_Wide_area_protection,
   Author = {Begovic, M. and Novosel, D. and Karlsson, D. and Henville, C. A. Henville C. and Michel, G. A. Michel G.},
   Title = {Wide-Area Protection and Emergency Control},
   Journal = {Proceedings of the IEEE},
   Volume = {93},
   Number = {5},
   Pages = {876-891},
   Year = {2005} }

@article{TPWRS04Miroslav-Gen-coherency,
   Author = {Jonsson, M. and Begovic, M. and Daalder, J.},
   Title = {A new method suitable for real-time generator coherency determination},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {3},
   Pages = {1473-1482},
   Year = {2004} }

@article{TPWRD04Miroslav-syst-prot-interarea,
   Author = {Jonsson, M. and Daalder, J. and Begovic, M.},
   Title = {A system protection scheme concept to counter interarea oscillations},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {19},
   Number = {4},
   Pages = {1602-1611},
   Year = {2004} }

@article{TPWRS03Miroslav-voltage-stab,
   Author = {Milosevic, B. and Begovic, M.},
   Title = {Voltage-stability protection and control using a wide-area network of phasor measurements},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {18},
   Number = {1},
   Pages = {121-127},
   Year = {2003} }

@article{Begovic_02_voltage_stab_protection,
   Author = {Milosevic, Borka D. and Begovic, Miroslav},
   Title = {Voltage Stability Protection and Control Using a Wide Area Network of Phasor Measurements},
   Journal = {IEEE Power Engineering Review},
   Volume = {22},
   Number = {9},
   Pages = {57-57},
   Year = {2002} }

@article{Begovic_04_Blackouts,
   Author = {Novosel, D. and Begovic, M. M. and Madani, V.},
   Title = {Shedding light on blackouts},
   Journal = {IEEE Power and Energy Magazine},
   Volume = {2},
   Number = {1},
   Pages = {32-43},
   Year = {2004} }

%%=======================================================================================

%%============================Loss of signals============================================


@article{TAC04-Montestruque,
   Author = {Montestruque, L. A. and Antsaklis, P.},
   Title = {Stability of model-based networked control systems with time-varying transmission times},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {49},
   Number = {9},
   Pages = {1562-1572},
   Year = {2004} }

@article{Auto03-Montestruque,
   Author = {Montestruque, Luis A. and Antsaklis, Panos J.},
   Title = {On the model-based control of networked systems},
   Journal = {Automatica},
   Volume = {39},
   Number = {10},
   Pages = {1837-1843},
   Year = {2003} }


@article{Auto03-Middleton,
   Author = {Zhivoglyadov, Peter V. and Middleton, Richard H.},
   Title = {Networked control design for linear systems},
   Journal = {Automatica},
   Volume = {39},
   Number = {4},
   Pages = {743-750},
   Year = {2003} }


@article{TPWRS07Salman-state-predictor,
   Author = {Mohagheghi, S. and Venayagamoorthy, G. K. and Harley, R. G.},
   Title = {Optimal Wide Area Controller and State Predictor for a Power System},
   Journal = {IEEE Transactions on Power Systems,},
   Volume = {22},
   Number = {2},
   Pages = {693-705},
   Year = {2007} }

@inproceedings{JNN03Narayanan-SensorDataRestoration,
   Author = {Narayanan, S. and Vian, J. L. and Choi, J. J. and Marks, R. J. and El-Sharkawi, M. A. and Thompson, B. B.},
   Title = {Missing sensor data restoration for vibration sensors on a jet aircraft engine},
   BookTitle = {Proceedings of the International Joint Conference on Neural Networks},
   Editor = {Vian, J. L.},
   Volume = {4},
   Pages = {3007-3010},
   Year = {2003} }

@article{IJC05NiemannFT,
   Author = {Niemann, H. and Stoustrup, J.},
   Title = {An architecture for fault tolerant controllers},
   Journal = {International Journal of Control},
   Volume = {78},
   Number = {14},
   Pages = {1091 - 1110},
   Year = {2005} }

@article{CSM96PengAntiWindup,
   Author = {Youbin, Peng and Vrancic, D. and Hanus, R.},
   Title = {Anti-windup, bumpless, and conditioned transfer techniques for {PID} controllers},
   Journal = {IEEE Control Systems Magazine},
   Volume = {16},
   Number = {4},
   Pages = {48-57},
   Year = {1996} }

@article{TAC97BRockett,
   Author = {Wing Shing, Wong and Brockett, R. W.},
   Title = {Systems with finite communication bandwidth constraints. {I.} State estimation problems},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {42},
   Number = {9},
   Pages = {1294-1299},
   Year = {1997} }

@article{TAC99Brockett,
   Author = {Wing Shing, Wong and Brockett, R. W.},
   Title = {Systems with finite communication bandwidth constraints. {II.} Stabilization with limited information feedback},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {44},
   Number = {5},
   Pages = {1049-1053},
   Year = {1999} }

@inproceedings{Branicky_94_Stability_switched,
   Author = {Branicky, M. S.},
   Title = {Stability of switched and hybrid systems},
   BookTitle = {Proceedings of the 33rd IEEE Conference on Decision and Control, 1994},
   Volume = {4},
   Pages = {3498-3503 vol.4},
   Year = {1994} }

@article{Sun-08-CompChemEngg-NetCntrl-ProcessSyst,
   author = {Sun, Y. L. and El-Farra, N. H.},
   title = {Quasi-decentralized model-based networked control of process systems},
   journal = {Computers \& Chemical Engineering},
   volume = {32},
   number = {9},
   pages = {2016-2029},
   year = {2008}}

@article{Sun-09-ACC09-Nonlinear,
   author = {Sun, Y. L. and El-Farra, N. H.},
   title = {Resource-aware Quasi-decentralized Control of Nonlinear Plants Over Communication Networks},
   journal = {2009 American Control Conference},
   pages = {154-159},
   year = {2009}}

@article{Sun-09-IndusChem-NetCntrl-FuelCell,
   author = {Sun, Y. L. and Ghantasala, S. and El-Farra, N. H.},
   title = {Networked Control of Distributed Energy Resources: Application to Solid Oxide Fuel Cells},
   journal = {Industrial \& Engineering Chemistry Research},
   volume = {48},
   number = {21},
   pages = {9590-9602},
   year = {2009}}

@article{TCSC-02-Walsh-Stability,
   author = {Walsh, G. C. and Hong, Ye and Bushnell, L. G.},
   title = {Stability analysis of networked control systems},
   journal = {IEEE Transactions on Control Systems Technology},
   volume = {10},
   number = {3},
   pages = {438-446},
   year = {2002}}

@inproceedings{ACC-00-Walsh-Predictors,
   author = {Beldiman, O. and Walsh, G. C. and Bushnell, L.},
   title = {Predictors for networked control systems},
   booktitle = {Proceedings of the 2000 American Control Conference},
   volume = {4},
   pages = {2347-2351},
   year = {2000}}



%%============================================================================


%%==============================Delay/Latency in wide-area signals============================

@patent{DelayPatentABB08,
  author        = {Korba, P. and Segundo, R. and Paice, A. and Berggren, B. and Majumder, R.},
  assignee      = {ABB Corporate Research},
  address       = {Vasteras, Sweden},
  title         = {Time delay compensation in Power System Control},
  nationality   = {European Union},
  number        = {EP08156785},
  note          = {filed on May 23, 2008}}
  %dayfiled      = {23},
%  monthfiled    = {May},
%  yearfiled     = {2008},



@inproceedings{Martin05WAMSstatus,
   Author = {Cai, J. Y. and Zhenyu, Huang and Hauer, J. and Martin, K.},
   Title = {Current Status and Experience of {WAMS} Implementation in North America},
   BookTitle = {IEEE/PES Transmission and Distribution Conference and Exhibition: Asia and Pacific, 2005},
   Pages = {1-7},
   Year = {2005} }



@article{Phadke01Crisis,
   Author = {Heydt, G.T. and Liu, C.C. and Phadke, A.G. and Vittal, V.},
   Title = {Solution for the crisis in electric power supply},
   Journal = {IEEE Computer Applications in Power},
   Volume = {14},
   Number = {3},
   Pages = {22-30},
   Year = {2001} }


@article{Heydt04gainscheduling,
   Author = {Hongxia, Wu and Tsakalis, K. S. and Heydt, G. T.},
   Title = {Evaluation of time delay effects to wide-area power system stabilizer design},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {4},
   Pages = {1935-1941},
   Year = {2004} }

@article{Vittal08LatencyStochastic,
   Author = {Stahlhut, J. W. and Browne, T. J. and Heydt, G. T. and Vittal, V.},
   Title = {Latency Viewed as a Stochastic Process and its Impact on Wide Area Power System Control Signals},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {1},
   Pages = {84-91},
   Year = {2008} }

@article{Dotta09WideAreaTwoLevel,
   Author = {Dotta, D. and e Silva, A. S. and Decker, I. C.},
   Title = {Wide-Area Measurements-Based Two-Level Control Design Considering Signal Transmission Delay},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {1},
   Pages = {208-216},
   Year = {2009} }




%%=============================================================================================

%%======================Non-linear Neural Network Estimation and Control=======================
@article{Debokda_08_Damping_GCSC,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Watanabe, E. H.},
   Title = {A Computational Approach to Optimal Damping Controller Design for a GCSC},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {23},
   Number = {3},
   Pages = {1673-1681},
   Year = {2008} }




@article{NonlinNNMalik07,
   Author = {Chaturvedi, D.K. and Malik, O.P.},
   Title = {Experimental Studies of a Generalized Neuron Based Adaptive Power System Stabilizer},
   Journal = {Soft Computing - A Fusion of Foundations, Methodologies and Applications},
   Volume = {Volume 11},
   Number = { 2 },
   Pages = {149-155},
      Year = {2007} }



@article{NonlinNNDash00,
   Author = {Dash, P. K. and Mishra, S. and Panda, G.},
   Title = {Damping Multimodal Power System Oscillation Using a Hybrid Fuzzy Controller for Series Connected Facts Devices},
   Journal = {IEEE Transaction on Power Systems},
   Volume = {15},
   Number = {4},
   Pages = {1360-1366},
      Year = {2000} }


@inproceedings{AdaptiveNNGanesh03,
   Author = {Liu, W.  and Venayagamoorthy, G.K. and Wunsch, D.C.},
   Title = {Adaptive neural network based power system stabilizer design},
   BookTitle = { Proceedings of the International Joint Conference on Neural Networks.},
   Volume = {4},
   Pages = {2970-2975},
      Year = {2003} }


@inproceedings{Debokda_08_DSP_PSO,
   Author = {Palangpour, P. and Mitra, P. and Ray, S. and Venayagamoorthy, G. K.},
   Title = {DSP-Based PSO Implementation for Online Optimization of Power System Stabilizers},
   BookTitle = {Adaptive Hardware and Systems, 2008. AHS '08. NASA/ESA Conference on},
   Pages = {379-384},
   Year = {2008} }



@inproceedings{RayMLP06,
   Author = {Ray, S. and Venayagamoorthy, G. K.},
   Title = {Nonlinear Modified PI Control of Multi-Module GCSCs in a Large Power System},
   BookTitle = {Conference Record of the 2006 IEEE Industry Applications Society},
   Volume = {3},
   Pages = {1345-1351},
   Year = {2006} }



@inproceedings{Debokda_06_RT_NN_GCSC,
   Author = {Ray, S. and Venayagamoorthy, G. K.},
   Title = {Real-Time Implementation of an Optimal Transient Neurocontroller for a {GCSC}},
   BookTitle = {International Joint Conference on Neural Networks},
   Pages = {2261-2266},
   Year = {2006} }



@article{RaySRN08,
   Author = {Ray, S. and Venayagamoorthy, G. K.},
   Title = {Real-time implementation of a measurement-based adaptive wide-area control system considering communication delays},
   Journal = {IET Generation, Transmission \& Distribution},
   Volume = {2},
   Number = {1},
   Pages = {62-70},
   Year = {2008} }



@article{Debokda_08_WideareaUPFC,
   Author = {Ray, S. and Venayagamoorthy, G. K.},
   Title = {Wide-Area Signal-Based Optimal Neurocontroller for a {UPFC}},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {23},
   Number = {3},
   Pages = {1597-1605},
   Year = {2008} }



@inproceedings{Debokda_07_MISO_TCSC,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Chaudhuri, B. and Majumder, R.},
   Title = {MISO damping controller design for a TCSC using particle swarm},
   BookTitle = {iREP Symposium Bulk Power System Dynamics and Control - VII },
   Year = {2007} }



@article{Debokda_08_Dampcont_GCSC,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Watanabe, E. H.},
   Title = {A Computational Approach to Optimal Damping Controller Design for a {GCSC}},
   Journal = { IEEE Transactions on Power Delivery},
   Volume = {23},
   Number = {3},
   Pages = {1673-1681},
   Year = {2008} }



@inproceedings{Debokda_08_optimal_dampcont_GCSC,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Watanabe, E. H.},
   Title = {Computational approach to optimal damping controller design for a {GCSC}},
   BookTitle = {IEEE Power and Energy Society General Meeting },
   Year = {2008} }



@inproceedings{Debokda_05_GCSC_multimachine,
   Author = {Ray, S. and Venayagamoorthy, G. K. and Watanabe, E. H. and de Jesus, F. D.},
   Title = {Optimal dynamic neurocontrol of a gate-controlled series capacitor in a multi-machine power system},
   BookTitle = {Proceedings of the 13th International Conference on Intelligent Systems Application to Power Systems},
   Year = {2005} }



@inproceedings{Ganesh_05_FACTS_controllers,
   Author = {Venayagamoorthy, G. K. and del Valle, Y. and Mohagheghi, S. and Qiao, W. and Ray, S. and Harley, R. G. and Falcao, D. M. and Taranto, G. N. and Assis, T. M. L.},
   Title = {Effects of a STATCOM, a SCRC and a UPFC on the dynamic behavior of a 45 bus section of the Brazilian power system},
   BookTitle = {IEEE Power Engineering Society Inaugural Conference and Exposition in Africa},
   Pages = {305-312},
   Year = {2005} }



@inproceedings{Debokda_05_NN_widearea_control,
   Author = {Venayagamoorthy, G. K. and Ray, S.},
   Title = {A neural network based optimal wide area control scheme for a power system},
   BookTitle = {Fourtieth IAS Annual Meeting. Conference Record of the 2005 Industry Applications Conference},
   Volume = {1},
   Pages = {700-706},
   Year = {2005} }


@article{Malik_97_NN_PSS,
   Author = {Shamsollahi, P. and Malik, O.P. },
   Title = {An adaptive power system stabilizer using on-line trained neural networks},
   Journal = { IEEE Transaction on Energy Conversion,},
   Volume = {12},
   Number = {4},
    Year = {1997} }

%%=============================================================================================


%%=============================== H-infinity control of dead time systems ====================================
@ARTICLE{H_inf_delay,
 author={Q. - C. Zhong},
 title={ ${H}_\infty $ control of dead time systems based on a transformation},
 journal={Automatica},
 volume={39},
 month ={February},
 year={2003},
 pages={361-366},
}

@ARTICLE{H_inf_delay1,
 author={Q. - C. Zhong},
 title={ On standard ${H}_\infty $ control process with a single delay},
 journal={IEEE Transactions on Automatic Control},
 volume={48},
 number={6},
 month={June},
 year={2003},
 pages={1097- 1103
},
}


@ARTICLE{mirkin,
 author={L. Mirkin},
 title={ On the extraction of dead-time controllers from delay-free parameterization.},
 journal={IEEE Transactions on Automatic Control},
 volume={48},
 number={4},
 month={April},
 year={2003},
 pages={543-553
},
}

@ARTICLE{nagravi,
 author={K.M. Nagpal and R. Ravi},
 title={ ${H}_\infty $ control and estimation problems with delayed measurements: State space solutions},
 journal={SIAM Journal on Control and Optimization},
 volume={35(4)},
 year={1997},
 pages={1217-1243},
}

@ARTICLE{palmor,
 author={Z.J. Palmor},
 title={Time delay compensation-Smith predictor and its modifications.},
 journal={The control handbook, CRC Press},
 year={1996},
 pages={224-237},
}

@ARTICLE{tadmor,
 author={G. Tadmor},
 title={ The standard ${H}_\infty $ problem in systems with a single input delay.},
 journal={IEEE Transactions on Automatic Control},
 volume={45(3)},
 year={2000},
 pages={382-397},
}


@ARTICLE{olbrot,
 author={A.Z. Manitius and A.W. Olbrot},
 title={ Finite spectrum assignment problem for systems with delays},
 journal={IEEE Transactions on Automatic Control},
 volume={24},
 number={4},
 month ={August},
 year={1979},
 pages={541-553},
}
@ARTICLE{Zwart,
 author={G. Meinsma and H. Zwart},
 title={On ${H}_\infty $ control for dead time systems},
 journal={IEEE Transactions on Automatic Control},
 volume={45},
 number={2},
 month ={February},
 year={2000},
 pages={272-285},
}
@ARTICLE{smith,
 author={O.J.M. Smith},
 title={Closer control of loops with dead time},
 journal={Chem. Eng. Progress},
 volume={53},
 number={5},
 year={1957},
 pages={217-219},
}

@ARTICLE{wantanable,
 author={K. Wantanable and M. Ito},
 title={A process-model control for linear systems with delay},
 journal={IEEE Transactions on Automatic Control},
 volume={26},
 number={6},
 month={December},
 year={1981},
 pages={1261-1269},
}

@ARTICLE{van,
 author={V.V. Assche and M. Dambrine and J.F. Lafay and J.P. Richard},
 title={Some problems arising in the implementation of distributed-delay control laws},
 journal={Proc of the 38th IEEE Conf on Decision and Control, Phoenix, Arizona, USA },
 month = {December},
 year={1999},
 pages={4668-4672},
}

@article{Mirkin08TimeVaryingDelay,
   Author = {Mirkin, B. and Gutman, P. O.},
   Title = {Robust Output-Feedback Model Reference Adaptive Control of SISO Plants With Multiple Uncertain, Time-Varying State Delays},
   Journal = {IEEE Transactions on Automatic Control},
   Volume = {53},
   Number = {10},
   Pages = {2414-2419},
   Year = {2008} }




%%=========================================================================================

%%=========================================Added By Nilanjan for Transfer Report================================

@inproceedings{Feliachi02_virginia_wams_delay,
   Author = {Naduvathuparambil, B. and Valenti, M. C. and Feliachi, A.},
   Title = {Communication delays in wide area measurement systems},
   BookTitle = {Proceedings of the Thirty-Fourth Southeastern Symposium on System Theory},
   Pages = {118-122},
   Year = {2002} }

@article{Dostert90_freqhopping_powerline,
   Author = {Dostert, K. M.},
   Title = {Frequency-hopping spread-spectrum modulation for digital communications over electrical power lines},
   Journal = {IEEE Journal on Selected Areas in Communications},
   Volume = {8},
   Number = {4},
   Pages = {700-710},
   Year = {1990} }

@article{Radford96_Spreadspectrum_powerline,
   Author = {Radford, D.},
   Title = {Spread spectrum data leap through AC power wiring},
   Journal = {IEEE Spectrum},
   Volume = {33},
   Number = {11},
   Pages = {48-53},
   Year = {1996} }

@article{EPRI_97_communications,
   Author = {Lamarre, L.},
   Title = {At home with communications},
   Journal = {EPRI Journal},
   Pages = {7-15},
   Year = {January/February 1997} }

@inproceedings{Taylor_WACS_simulations,
   Author = {Wilson, R. E. and Taylor, C. W.},
   Title = {Using dynamic simulations to design the wide-area stability and voltage control system (WACS)},
   BookTitle = {IEEE PES Power Systems Conference and Exposition},
   Pages = {100-107 vol.1},
   Year = {2004} }

@inproceedings{Taylor00_widearea_stab_voltcont,
   Author = {Taylor, C. W. and Venkatasubramanian, M. V. and Chen, Y.},
   Title = {Wide-Area Stability and Voltage Control},
   BookTitle = {VII Symposium of Specialists in Electric Operational and Expansion Planning},
   Pages = {1-9},
   Year = {2000} }

@article{IEEE93_subcommittee_microwave_communication,
   title = {Analog/digital microwave considerations for electric/gas utilities},
   journal = {IEEE Transactions on Power Delivery},
   volume = {8},
   number = {3},
   pages = {798-815},
   year = {1993}
}



@article{spectrum09_PLC_brdband,
   Author = {Schneider, D.},
   Title = {Is this the moment for broadband over power lines?},
   Journal = {IEEE Spectrum},
   Volume = {46},
   Number = {7},
   Pages = {17-17},
      Year = {2009} }



%%=============================Monitoring Power System Oscillations=================================
@inproceedings{Mani_09_osc_monitoring_syst,
   Author = {Liu, G. and Venkatasubramanian, V. M. and Carroll, J. R.},
   Title = {Oscillation monitoring system using synchrophasors},
   BookTitle = {Power \& Energy Society General Meeting, 2009. PES '09. IEEE},
   Pages = {1-4},
   Year = {2009} }

@article{Hauer_97_keepingeye,
   Author = {Hauer, J. and Trudnowski, D. and Rogers, G. and Mittelstadt, B. and Litzenberger, W. and Johnson, J.},
   Title = {Keeping an eye on power system dynamics},
   Journal = {IEEE Computer Applications in Power},
   Volume = {10},
   Number = {4},
   Pages = {50-54},
   Year = {1997} }

@article{Hauer_91_Prony,
   Author = {Hauer, J. F.},
   Title = {Application of Prony analysis to the determination of modal content and equivalent models for measured power system response},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {6},
   Number = {3},
   Pages = {1062-1068},
   Year = {1991} }

@article{Hauer_09_WECC_WAMSprobing,
   Author = {Hauer, J. F. and Mittelstadt, W. A. and Martin, K. E. and Burns, J. W. and Lee, H. and Pierre, J. W. and Trudnowski, D. J.},
   Title = {Use of the WECC WAMS in Wide-Area Probing Tests for Validation of System Performance and Modeling},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {1},
   Pages = {250-257},
   Year = {2009} }

@article{Hauer_90_Oscdetect_BPA,
   Author = {Hauer, J. F. and Vakili, F.},
   Title = {An oscillation detector used in the BPA power system disturbance monitor},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {5},
   Number = {1},
   Pages = {74-79},
   Year = {1990} }

@article{Kamwa_96_blackbox,
   Author = {Kamwa, I. and Trudel, G. and Gerin-Lajoie, L.},
   Title = {Low-order black-box models for control system design in large power systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {11},
   Number = {1},
   Pages = {303-311},
   Year = {1996} }

@article{ManiVenky_97_Osccalc,
   Author = {Kim, K. and Schattler, H. and Venkatasubramanian, V. and Zaborszky, J. and Hirsch, P.},
   Title = {Methods for calculating oscillations in large power systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {12},
   Number = {4},
   Pages = {1639-1648},
   Year = {1997} }

@article{Hauer_06_probing_subspace,
   Author = {Zhou, N. and Pierre, J. W. and Hauer, J. F.},
   Title = {Initial results in power system identification from injected probing signals using a subspace method},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {21},
   Number = {3},
   Pages = {1296-1302},
   Year = {2006} }

@article{Pierre_07_RRLS,
   Author = {Zhou, N. and Pierre, J. W. and Trudnowski, D. J. and Guttromson, R. T.},
   Title = {Robust RLS Methods for Online Estimation of Power System Electromechanical Modes},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {22},
   Number = {3},
   Pages = {1240-1249},
   Year = {2007} }

@article{Trud_08_RRRLS,
   Author = {Zhou, N. and Trudnowski, D. J. and Pierre, J. W. and Mittelstadt, W. A.},
   Title = {Electromechanical Mode Online Estimation Using Regularized Robust RLS Methods},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {4},
   Pages = {1670-1680},
   Year = {2008} }

@article{Trud_08_modemeter,
   Author = {Trudnowski, D. J. and Pierre, J. W. and Zhou, N. and Hauer, J. F. and Parashar, M.},
   Title = {Performance of Three Mode-Meter Block-Processing Algorithms for Automated Dynamic Stability Assessment},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {2},
   Pages = {680-690},
   Year = {2008} }

@article{Pierre_02_ARMAblock,
   Author = {Wies, R. W. and Pierre, J. W. and Trudnowski, D. J.},
   Title = {Use of ARMA Block Processing for Estimating Stationary Low-Frequency Electromechanical Modes of Power Systems},
   Journal = {IEEE Power Engineering Review},
   Volume = {22},
   Number = {11},
   Pages = {57-57},
   Year = {2002} }

@inproceedings{Pierre_04_GM_LMS,
   Author = {Wies, R. W. and Pierre, J. W. and Trudnowski, D. J.},
   Title = {Use of least mean squares (LMS) adaptive filtering technique for estimating low-frequency electromechanical modes in power systems},
   BookTitle = {IEEE Power Engineering Society General Meeting, 2004},
   Pages = {1863-1870 Vol.2},
   Year = {2004} }

@article{Begovic_04_gencoherency,
   Author = {Jonsson, M. and Begovic, M. and Daalder, J.},
   Title = {A new method suitable for real-time generator coherency determination},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {3},
   Pages = {1473-1482},
   Year = {2004} }



@article{Hauer_90_Prony_initial,
   Author = {Hauer, J. F. and Demeure, C. J. and Scharf, L. L.},
   Title = {Initial results in Prony analysis of power system response signals},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {5},
   Number = {1},
   Pages = {80-89},
   Year = {1990} }

@article{Kamwa_93_minimal_realization,
   Author = {Kamwa, I. and Grondin, R. and Dickinson, E. J. and Fortin, S.},
   Title = {A minimal realization approach to reduced-order modelling and modal analysis for power system response signals},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {8},
   Number = {3},
   Pages = {1020-1029},
   Year = {1993} }

@article{Trudnowski_08_modeshape,
   Author = {Trudnowski, D. J.},
   Title = {Estimating Electromechanical Mode Shape From Synchrophasor Measurements},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {3},
   Pages = {1188-1195},
   Year = {2008} }

@inproceedings{Trud_09_Modeshape_TF_LS,
   Author = {Zhou, N. and Huang, Z. and Dosiek, L. and Trudnowski, D. and Pierre, J. W.},
   Title = {Electromechanical mode shape estimation based on transfer function identification using PMU measurements},
   BookTitle = {IEEE Power and Energy Society General Meeting},
   Pages = {1-7},
   Year = {2009} }

@inproceedings{Trud_09_Modeshape_coherency_Channelmatch,
   Author = {Dosiek, L. and Pierre, J. W. and Trudnowski, D. J. and Zhou, N.},
   Title = {A channel matching approach for estimating electromechanical mode shape and coherence},
   BookTitle = {IEEE Power and Energy Society General Meeting},
   Pages = {1-8},
   Year = {2009} }

@inproceedings{Trudnowski_08_PESGM_modeshape,
   Author = {Dosiek, L. and Trudnowski, D. J. and Pierre, J. W.},
   Title = {New algorithms for mode shape estimation using measured data},
   BookTitle = {IEEE Power and Energy Society General Meeting - Conversion and Delivery of Electrical Energy in the 21st Century},
   Pages = {1-8},
   Year = {2008} }

@inproceedings{Ledwich_02_mdshp_spectral,
   Author = {Banejad, M. and Ledwich, G.},
   Title = {Correlation based mode shape determination of a power system},
   BookTitle = {Proceedings of  IEEE International Conference on Acoustics, Speech, and Signal Processing, 2002 (ICASSP '02).},
   Volume = {4},
   Pages = {IV-3832-IV-3835 vol.4},
   Year = {2002} }

@inproceedings{Liu_09_mdshp_matrixpencil,
   Author = {Li, W. and Gardner, R. M. and Dong, J. and Lei, Wang and Tao, Xia and Yingchen, Zhang and Liu, Y. and Guorui, Zhang and Xue, Y.},
   Title = {Wide area synchronized measurements and inter-area oscillation study},
   BookTitle = {Proceedings of IEEE/PES Power Systems Conference and Exposition, 2009. PSCE '09. },
   Pages = {1-8},
   Year = {2009} }

@inproceedings{Mani_08_FDD_mdshps,
   Author = {Liu, G. and Venkatasubramanian, V.},
   Title = {Oscillation monitoring from ambient PMU measurements by Frequency Domain Decomposition},
   BookTitle = {Proceedings of IEEE International Symposium on Circuits and Systems, 2008 (ISCAS 2008)},
   Pages = {2821-2824},
   Year = {2008} }

@inproceedings{Koessler_07_PronyModshp,
   Author = {Koessler, R. J. and Prabhakara, F. S. and Al-Mubarak, A. H.},
   Title = {Analysis of Oscillations with Eigenanalysis and Prony Techniques},
   BookTitle = {IEEE Power Engineering Society General Meeting, 2007},
   Pages = {1-8},
   Year = {2007} }

@inproceedings{Toyoda_02_online_modal_LS,
   Author = {Saitoh, H. and Miura, K. and Ishioka, O. and Sato, H. and Toyoda, J.},
   Title = {On-line modal analysis based on synchronized measurement technology},
   BookTitle = {Proceedings of International Conference on Power System Technology, 2002, PowerCon 2002. },
   Volume = {2},
   Pages = {817-822 vol.2},
   Year = {2002} }

@inproceedings{Martins_07_Modeshape_moment_matching,
   Author = {Freitas, F. D. and Martins, N. and Fernandes, L.},
   Title = {Reliable mode-shapes for major system modes extracted from concentrated WAMS measurements processed by a SIMO identification algorithm},
   BookTitle = {IEEE Power and Energy Society General Meeting - Conversion and Delivery of Electrical Energy in the 21st Century, 2008 },
   Pages = {1-8},
   Year = {2008} }

@inproceedings{Rogers_03_dynamic_model_verification,
   Author = {Wilson, D. H. and Hay, K. and Rogers, G. J.},
   Title = {Dynamic model verification using a continuous modal parameter estimator},
   BookTitle = {IEEE Power Tech Conference Proceedings, 2003 Bologna},
   Volume = {2},
   Pages = {6 pp. Vol.2},
   Year = {2003} }

@article{Vittal_07_EMD_Modeshape,
   Author = {Messina, A. R. and Vittal, V.},
   Title = {Extraction of Dynamic Patterns From Wide-Area Measurements Using Empirical Orthogonal Functions},
   Journal = {IEEE Transactions on Power Systems, },
   Volume = {22},
   Number = {2},
   Pages = {682-692},
   Year = {2007} }

@inproceedings{Mani_07_three_ringdown_methods,
   Author = {Liu, G. and Quintero, J. and Venkatasubramanian, V.},
   Title = {Oscillation monitoring system based on wide area synchrophasors in power systems},
   BookTitle = {Proceedings of Bulk Power System Dynamics and Control - VII. Revitalizing Operational Reliability, 2007 iREP Symposium},
   Pages = {1-13},
   Year = {2007} }




@inproceedings{Hauer_07_WAMS_osc_monitoring,
   Author = {Hauer, A. J. F. and Trudnowski, D. J. and DeSteese, J. G.},
   Title = {A Perspective on WAMS Analysis Tools for Tracking of Oscillatory Dynamics},
   BookTitle = {Proceedings of IEEE Power Engineering Society General Meeting, 2007.},
   Pages = {1-10},
   Year = {2007} }

@article{Hauer_81_spectral,
   Author = {Hauer, J. F. and Cresap, R. L.},
   Title = {Measurement and Modeling of Pacific AC Intertie Response to Random Load Switching},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {PAS-100},
   Number = {1},
   Pages = {353-359},
      Year = {1981} }

@article{Trud_97_ambient_modal_estimation,
   Author = {Pierre, J. W. and Trudnowski, D. J. and Donnelly, M. K.},
   Title = {Initial results in electromechanical mode identification from ambient data},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {12},
   Number = {3},
   Pages = {1245-1251},
   Year = {1997} }

@article{Chow_99_comparison_threemethods,
   Author = {Sanchez-Gasca, J. J. and Chow, J. H.},
   Title = {Performance comparison of three identification methods for the analysis of electromechanical oscillations},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {14},
   Number = {3},
   Pages = {995-1002},
   Year = {1999} }

@article{Pierre_05_bootstrap_multioutput_ambient,
   Author = {Anderson, M. G. and Zhou, N. and Pierre, J. W. and Wies, R. W.},
   Title = {Bootstrap-based confidence interval estimates for electromechanical modes from multiple output analysis of measured ambient data},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {20},
   Number = {2},
   Pages = {943-950},
   Year = {2005} }

@inproceedings{Trud_04_LMS_modalestim,
   Author = {Wies, R. W. and Pierre, J. W. and Trudnowski, D. J.},
   Title = {Use of least mean squares (LMS) adaptive filtering technique for estimating low-frequency electromechanical modes in power systems},
   BookTitle = {Proceedings of IEEE Power Engineering Society General Meeting, 2004},
   Pages = {1863-1870 Vol.2},
   Year = {2004} }








%%=============================================================================================================================


%%===============================EMD=================================================

@inproceedings{Deering_05_EMDmasking,
   Author = {Deering, R. and Kaiser, J. F.},
   Title = {The use of a masking signal to improve empirical mode decomposition},
   BookTitle = {Proceedings of IEEE International Conference on Acoustics, Speech, and Signal Processing, 2005(ICASSP '05)},
   Volume = {4},
   Pages = {iv/485-iv/488 Vol. 4},
   Year = {2005} }

@article{Vittal_06_HHT_inter_area_osc,
   Author = {Messina, A. R. and Vittal, V.},
   Title = {Nonlinear, non-stationary analysis of interarea oscillations via Hilbert spectral analysis},
   Journal = {IEEE Transactions on Power Systems, },
   Volume = {21},
   Number = {3},
   Pages = {1234-1241},
   Year = {2006} }



%%========================================================================================


%%===========================Micro-Grid======================================================
@article{Yazdani_09_Multimode_DFIG,
   Author = {Bhuiyan, F. A. and Yazdani, A.},
   Title = {Multimode Control of a {DFIG}-Based Wind-Power Unit for Remote Applications},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {24},
   Number = {4},
   Pages = {2079-2089},
   Year = {2009} }

@inproceedings{Divan_94_parallel_UPS,
   Author = {Chandrokar, M. C. and Divan, D. M. and Banerjee, B.},
   Title = {Control of distributed UPS systems},
   BookTitle = {25th Annual IEEE Power Electronics Specialists Conference, PESC '94 Record},
   Pages = {197-204 vol.1},
   Year = {1994} }

@article{Iravani_06_Parallel_DG_Microgrid,
   Author = {Katiraei, F. and Iravani, M. R.},
   Title = {Power Management Strategies for a Microgrid With Multiple Distributed Generation Units},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {21},
   Number = {4},
   Pages = {1821-1831},
   Year = {2006} }




%%===========================================================================================

%%========================================DFIG===============================================

@article{Miller_10_DFIGfaultTolerance,
   Author = {Piwko, R. and Miller, N. and Girad, R. and MacDowell, J. and Clark, K. and Murdoch, A.},
   Title = {Generator Fault Tolerance and Grid Codes},
   Journal = {IEEE Power and Energy Magazine},
   Volume = {8},
   Number = {2},
   Pages = {18-26},
   Year = {2010} }


@inproceedings{Kling_01_DFIG_Model,
   Author = {Slootweg, J. G. and Polinder, H. and Kling, W. L.},
   Title = {Dynamic modelling of a wind turbine with doubly fed induction generator},
   BookTitle = {IEEE Power Engineering Society Summer Meeting, 2001},
   Volume = {1},
   Pages = {644-649 vol.1},
   Year = {2001} }


@inproceedings{Pinheiro_06_LossReduction_DFIG,
   Author = {Rabelo, B. and Hofmann, W. and Pinheiro, L.},
   Title = {Loss reduction methods for doubly-fed induction generator drives for wind turbines},
   BookTitle = {International Symposium on Power Electronics, Electrical Drives, Automation and Motion, 2006, SPEEDAM 2006. },
   Pages = {1217-1222},
   Year = {2006} }

@article{Pena_96_DFIG_VariableSpd,
   Author = {Pena, R. and Clare, J. C. and Asher, G. M.},
   Title = {Doubly fed induction generator using back-to-back {PWM} converters and its application to variable-speed wind-energy generation},
   Journal = {IEE Proceedings on Electric Power Applications},
   Volume = {143},
   Number = {3},
   Pages = {231-241},
   Year = {1996} }


@article{Pena_96_DFIG_Isolated,
   Author = {Pena, R. and Clare, J. C. and Asher, G. M.},
   Title = {A Doubly fed induction generator using back-to-back {PWM} converters supplying an isolated load from a variable-speed wind turbine},
   Journal = {IEE Proceedings on Electric Power Applications},
   Volume = {143},
   Number = {5},
   Pages = {380-387},
   Year = {1996} }

@article{BPal_08_DFIG_modelingAdequacy,
   Author = {Pal, B. C. and Mei, F.},
   Title = {Modelling adequacy of the doubly fed induction generator for small-signal stability studies in power systems},
   Journal = {IET Renewable Power Generation},
   Volume = {2},
   Number = {3},
   Pages = {181-190},
   Year = {2008} }

@article{Vieira_09_GEA_DFIGcontroller,
   Author = {Vieira, J. P. A. and Nunes, M. V. A. and Bezerra, U. H. and do Nascimento, A. C.},
   Title = {Designing optimal controllers for doubly fed induction generators using a genetic algorithm},
   Journal = {IET Generation, Transmission & Distribution},
   Volume = {3},
   Number = {5},
   Pages = {472-484},
   Year = {2009} }

@article{Jenkins_09_DFIG_modeling,
   Author = {Ekanayake, J. B. and Holdsworth, L. and XueGuang, Wu and Jenkins, N.},
   Title = {Dynamic modeling of doubly fed induction generator wind turbines},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {18},
   Number = {2},
   Pages = {803-809},
   Year = {2003} }

@article{Vittal_09_Stability_DFIG_penetration,
   Author = {Gautam, D. and Vittal, V. and Harbour, T.},
   Title = {Impact of Increased Penetration of DFIG-Based Wind Turbine Generators on Transient and Small Signal Stability of Power Systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {3},
   Pages = {1426-1434},
   Year = {2009} }


@article{Usaola_05_DFIG_transientStab,
   Author = {Ledesma, P. and Usaola, J.},
   Title = {Doubly fed induction generator model for transient stability analysis},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {20},
   Number = {2},
   Pages = {388-397},
   Year = {2005} }

@article{Fan_09_DFIG_oscDamp,
   Author = {Zhixin, Miao and Lingling, Fan and Osborn, D. and Yuvarajan, S.},
   Title = {Control of {DFIG}-Based Wind Generation to Improve Interarea Oscillation Damping},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {24},
   Number = {2},
   Pages = {415-422},
   Year = {2009} }

@article{Lei_06_Modeling_DFIG_gridIntegration,
   Author = {Yazhou, Lei and Mullane, A. and Lightbody, G. and Yacamini, R.},
   Title = {Modeling of the wind turbine with a doubly fed induction generator for grid integration studies},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {21},
   Number = {1},
   Pages = {257-264},
   Year = {2006} }

@article{Godfrey_07_SmallSignalDFIG,
   Author = {Wu, F. and Zhang, X. P. and Godfrey, K. and Ju, P.},
   Title = {Small signal stability analysis and optimal control of a wind turbine with doubly fed induction generator},
   Journal = {IET Generation Transmission & Distribution},
   Volume = {1},
   Number = {5},
   Pages = {751-760},
   Year = {2007} }

@article{Yazdani_09_StabilityDFIGseriescomp,
   Author = {Ostadi, A. and Yazdani, A. and Varma, R. K.},
   Title = {Modeling and Stability Analysis of a DFIG-Based Wind-Power Generator Interfaced With a Series-Compensated Line},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {24},
   Number = {3},
   Pages = {1504-1514},
   Year = {2009} }

@article{BC_07_DFIG_modal,
   Author = {Mei, F. and Pal, B.},
   Title = {Modal Analysis of Grid-Connected Doubly Fed Induction Generators},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {22},
   Number = {3},
   Pages = {728-736},
   Year = {2007} }

@article{Klin_03_WTgeneralModel,
   Author = {Slootweg, J. G. and de Haan, S. W. H. and Polinder, H. and Kling, W. L.},
   Title = {General model for representing variable speed wind turbines in power system dynamics simulations},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {18},
   Number = {1},
   Pages = {144-151},
   Year = {2003} }

@article{Yamamoto_91_DFIG_PQcontrol,
   Author = {Yamamoto, M. and Motoyoshi, O.},
   Title = {Active and reactive power control for doubly-fed wound rotor induction generator},
   Journal = {IEEE Transactions on Power Electronics},
   Volume = {6},
   Number = {4},
   Pages = {624-629},
   Year = {1991} }

@article{Sterling_08_NonlinearControlDFIG,
   Author = {Feng, Wu and Xiao-Ping, Zhang and Ping, Ju and Sterling, M. J. H.},
   Title = {Decentralized Nonlinear Control of Wind Turbine With Doubly Fed Induction Generator},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {2},
   Pages = {613-621},
   Year = {2008} }

@article{Jenkins_03_DFIGinitializeDirect,
   Author = {Holdsworth, L. and Wu, X. G. and Ekanayake, J. B. and Jenkins, N.},
   Title = {Direct solution method for initialising doubly-fed induction wind turbines in power system dynamic models},
   Journal = {IEE Proceedings Generation, Transmission and Distribution},
   Volume = {150},
   Number = {3},
   Pages = {334-342},
   Year = {2003} }

@article{Milanovic_08_DFIGsimplification,
   Author = {Kayikci, M. and Milanovic, J. V.},
   Title = {Assessing Transient Response of DFIG-Based Wind Plants-The Influence of Model Simplifications and Parameters},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {23},
   Number = {2},
   Pages = {545-554},
   Year = {2008} }

@article{Niiranen_06_DFIG_ridethru,
   Author = {Seman, S. and Niiranen, J. and Arkkio, A.},
   Title = {Ride-Through Analysis of Doubly Fed Induction Wind-Power Generator Under Unsymmetrical Network Disturbance},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {21},
   Number = {4},
   Pages = {1782-1789},
   Year = {2006} }

@article{Niiranan_06_DFIGdisturbance,
   Author = {Seman, S. and Niiranen, J. and Kanerva, S. and Arkkio, A. and Saitz, J.},
   Title = {Performance Study of a Doubly Fed Wind-Power Induction Generator Under Network Disturbances},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {21},
   Number = {4},
   Pages = {883-890},
   Year = {2006} }

@article{Dinavai_09_RealTimeDFIG,
   Author = {Lok-Fu, Pak and Dinavahi, V.},
   Title = {Real-Time Simulation of a Wind Energy System Based on the Doubly-Fed Induction Generator},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {3},
   Pages = {1301-1309},
   Year = {2009} }

@article{Jenkins_04_CoordinatedDFIG,
   Author = {Cartwright, P. and Holdsworth, L. and Ekanayake, J. B. and Jenkins, N.},
   Title = {Co-ordinated voltage control strategy for a doubly-fed induction generator (DFIG)-based wind farm},
   Journal = {IEE Proceedings- Generation, Transmission and Distribution},
   Volume = {151},
   Number = {4},
   Pages = {495-502},
   Year = {2004} }

@article{Jenkins_03_DFIGvsSEIG,
   Author = {Holdsworth, L. and Wu, X. G. and Ekanayake, J. B. and Jenkins, N.},
   Title = {Comparison of fixed speed and doubly-fed induction wind turbines during power system disturbances},
   Journal = {IEE Proceedings- Generation, Transmission and Distribution},
   Volume = {150},
   Number = {3},
   Pages = {343-352},
   Year = {2003} }

@article{Ostolaza_06_WindFarmModeling,
   Author = {Tapia, G. and Tapia, A. and Ostolaza, J. X.},
   Title = {Two Alternative Modeling Approaches for the Evaluation of Wind Farm Active and Reactive Power Performances},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {21},
   Number = {4},
   Pages = {909-920},
   Year = {2006} }

@article{Jenkins_08_WindnTowershadowDFIG,
   Author = {Hughes, F. M. and Anaya-Lara, O. and Ramtharan, G. and Jenkins, N. and Strbac, G.},
   Title = {Influence of Tower Shadow and Wind Turbulence on the Performance of Power System Stabilizers for DFIG-Based Wind Farms},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {23},
   Number = {2},
   Pages = {519-528},
   Year = {2008} }

@article{Lopes_04_DFIGstabMargin,
   Author = {Nunes, M. V. A. and Lopes, J. A. P. and Zurn, H. H. and Bezerra, U. H. and Almeida, R. G.},
   Title = {Influence of the variable-speed wind generators in transient stability margin of the conventional generators integrated in electrical grids},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {19},
   Number = {4},
   Pages = {692-701},
   Year = {2004} }

@article{Thiringer_05_ModelDFIG,
   Author = {Petersson, A. and Thiringer, T. and Harnefors, L. and Petru, T.},
   Title = {Modeling and experimental verification of grid interaction of a DFIG wind turbine},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {20},
   Number = {4},
   Pages = {878-886},
   Year = {2005} }

@article{Jenkins_05_DFIGcontrol,
   Author = {Hughes, F. M. and Anaya-Lara, O. and Jenkins, N. and Strbac, G.},
   Title = {Control of {DFIG}-based wind generation for power network support},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {20},
   Number = {4},
   Pages = {1958-1966},
   Year = {2005} }

@article{Udaya_10_EigenstructDFIG,
   Author = {Kshatriya, N. and Annakkage, U. D. and Hughes, F. M. and Gole, A. M.},
   Title = {Optimized Partial Eigenstructure Assignment-Based Design of a Combined PSS and Active Damping Controller for a DFIG},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {25},
   Number = {2},
   Pages = {866-876},
   Year = {2010} }

@inproceedings{Lopes_07_Simultune_PSS_DFIG,
   Author = {Mendonca, A. and Lopes, J. A. P.},
   Title = {Simultaneous Tuning of Power System Stabilizers Installed in DFIG-Based Wind Generation},
   BookTitle = {IEEE Lausanne Power Tech, 2007},
   Pages = {219-224},
   Year = {2007} }


@article{Barnes_08_DFIGstability,
   Author = {Chondrogiannis, S. and Barnes, M.},
   Title = {Stability of doubly-fed induction generator under stator voltage orientated vector control},
   Journal = {IET Renewable Power Generation},
   Volume = {2},
   Number = {3},
   Pages = {170-180},
   Year = {2008} }

@article{Jenkins_07_FreqsupportDFIG,
   Author = {Ramtharan, G. and Ekanayake, J. B. and Jenkins, N.},
   Title = {Frequency support from doubly fed induction generator wind turbines},
   Journal = {IET Renewable Power Generation},
   Volume = {1},
   Number = {1},
   Pages = {3-9},
   Year = {2007} }

@article{Ooi_06_DFIGstability,
   Author = {Banakar, H. and Luo, C. and Ooi, B. T.},
   Title = {Steady-state stability analysis of doubly-fed induction generators under decoupled P-Q control},
   Journal = {IEE Proceedings - Electric Power Applications},
   Volume = {153},
   Number = {2},
   Pages = {300-306},
   Year = {2006} }

@inproceedings{SanchezGasca_04_DFIGmodal,
   Author = {Sanchez-Gasca, J. J. and Miller, N. W. and Price, W. W.},
   Title = {A modal analysis of a two-area system with significant wind power penetration},
   BookTitle = {IEEE PES Power Systems Conference and Exposition, 2004.},
   Pages = {1148-1152 vol.2},
   Year = {2004} }

@inproceedings{SanchezGasca_03_GEwtgmodel,
   Author = {Miller, N. W. and Sanchez-Gasca, J. J. and Price, W. W. and Delmerico, R. W.},
   Title = {Dynamic modeling of GE 1.5 and 3.6 MW wind turbine-generators for stability simulations},
   BookTitle = {IEEE Power Engineering Society General Meeting, 2003},
   Volume = {3},
   Pages = {1977-1983 Vol. 3},
   Year = {2003} }

@article{Mishra_09_DFIGdampcont,
   Author = {Mishra, Y. and Mishra, S. and Tripathy, M. and Senroy, N. and Dong, Z. Y.},
   Title = {Improving Stability of a DFIG-Based Wind Power System With Tuned Damping Controller},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {24},
   Number = {3},
   Pages = {650-660},
   Year = {2009} }

    @article{SMishra_09_DFIGstab,
       Author = {Mishra, Y. and Mishra, S. and Fangxing, Li and Zhao Yang, Dong and Bansal, R. C.},
       Title = {Small-Signal Stability Analysis of a DFIG-Based Wind Power System Under Different Modes of Operation},
       Journal = {IEEE Transactions on Energy Conversion},
       Volume = {24},
       Number = {4},
       Pages = {972-982},
       Year = {2009} }

@article{Jenkins_06_DFIGPSS,
   Author = {Hughes, F. M. and Anaya-Lara, O. and Jenkins, N. and Strbac, G.},
   Title = {A power system stabilizer for DFIG-based wind generation},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {21},
   Number = {2},
   Pages = {763-772},
   Year = {2006} }

@article{Mulijadi_07_DFIGstability,
   Author = {Muljadi, E. and Butterfield, C. P. and Parsons, B. and Ellis, A.},
   Title = {Effect of Variable Speed Wind Turbine Generator on Stability of a Weak Grid},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {22},
   Number = {1},
   Pages = {29-36},
   Year = {2007} }

@article{Jenkins_07_DFIG_synchrTorque,
   Author = {Anaya-Lara, O. and Hughes, F. M. and Jenkins, N. and Strbac, G.},
   Title = {Provision of a synchronising power characteristic on DFIG-based wind farms},
   Journal = {IET Generation, Transmission & Distribution},
   Volume = {1},
   Number = {1},
   Pages = {162-169},
   Year = {2007} }

@article{Feijoo_09_PQmodel_SEIG,
   Author = {Feijoo, A.},
   Title = {On PQ Models for Asynchronous Wind Turbines},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {4},
   Pages = {1890-1891},
   Year = {2009} }

@article{Vournas_09_DampgCntrbutionDFIG,
   Author = {Tsourakis, G. and Nomikos, B. M. and Vournas, C. D.},
   Title = {Contribution of Doubly Fed Wind Generators to Oscillation Damping},
   Journal = {IEEE Transactions on Energy Conversion},
   Volume = {24},
   Number = {3},
   Pages = {783-791},
   Year = {2009} }

@article{Milanovic_09_DFIG_AGC,
   Author = {Kayikci, M. and Milanovic, J. V.},
   Title = {Dynamic Contribution of DFIG-Based Wind Plants to System Frequency Disturbances},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {2},
   Pages = {859-867},
   Year = {2009} }

@article{Kennedy_10_Wind_OscMonitoring,
   Author = {Liu, X. and McSwiggan, D. and Littler, T. B. and Kennedy, J.},
   Title = {Measurement-based method for wind farm power system oscillations monitoring},
   Journal = {Renewable Power Generation, IET},
   Volume = {4},
   Number = {2},
   Pages = {198-209},
      Year = {2010} }

@article{Iravani_08_Wind_Model,
   Author = {Tabesh, A. and Iravani, R.},
   Title = {Small-signal model and dynamic analysis of variable speed induction machine wind farms},
   Journal = {IET Renewable Power Generation},
   Volume = {2},
   Number = {4},
   Pages = {215-227},
   Year = {2008} }

@article{OMalley_10_WndGenonFreqControl,
   Author = {Doherty, R. and Mullane, A. and Nolan, G. and Burke, D. J. and Bryson, A. and O'Malley, M.},
   Title = {An Assessment of the Impact of Wind Generation on System Frequency Control},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {25},
   Number = {1},
   Pages = {452-460},
   Year = {2010} }

@article{Kjetil-05-Wind-Nordic,
   author = {Hagstr�m, Espen and Norheim, Ian and Uhlen, Kjetil},
   title = {Large-scale wind power integration in Norway and impact on damping in the Nordic grid},
   journal = {Wind Energy},
   volume = {8},
   number = {3},
   pages = {375-384},
   year = {2005}
}

@inproceedings{Vowles-08-WindStabilityNZ,
   author = {Vowles, D. J. and Samarasinghe, C. and Gibbard, M. J. and Ancell, G.},
   title = {Effect of wind generation on small-signal stability; A New Zealand Example},
   booktitle = {proceedings of IEEE Power and Energy Society General Meeting},
   pages = {1-8},
    year = {2008}
}














































%%==============================PLL=========================================================
@article{Chung_00_PLL,
   Author = {Se-Kyo, Chung},
   Title = {A phase tracking system for three phase utility interface inverters},
   Journal = {IEEE Transactions on Power Electronics },
   Volume = {15},
   Number = {3},
   Pages = {431-438},
   Year = {2000} }

@article{Shinnaka_08_singlephase_PLL,
   Author = {Shinji, Shinnaka},
   Title = {A Robust Single-Phase PLL System With Stable and Fast Tracking},
   Journal = {IEEE Transactions on Industry Applications },
   Volume = {44},
   Number = {2},
   Pages = {624-633},
   Year = {2008} }

@inproceedings{Cataliotti_05_PLL_PowerQuality,
   Author = {Cataliotti, A. and Cosentino, V. and Nuccio, S.},
   Title = {A new Phase Locked Loop Strategy for Power Quality Instruments Synchronisation},
   BookTitle = {Proceedings of the IEEE Instrumentation and Measurement Technology Conference, 2005. IMTC 2005. },
   Volume = {2},
   Pages = {941-946},
   Year = {2005} }

@article{Iravani_04_QPLL,
   Author = {Karimi-Ghartemani, M. and Karimi, H. and Iravani, M. R.},
   Title = {A magnitude/phase-locked loop system based on estimation of frequency and in-phase/quadrature-phase amplitudes},
   Journal = {IEEE Transactions on Industrial Electronics },
   Volume = {51},
   Number = {2},
   Pages = {511-517},
   Year = {2004} }

@inproceedings{Iravani_01_NewPLL,
   Author = {Karimi-Ghartemani, M. and Iravani, M. R.},
   Title = {A new phase-locked loop (PLL) system},
   BookTitle = {Proceedings of the 44th IEEE 2001 Midwest Symposium onCircuits and Systems, 2001. MWSCAS 2001.},
   Volume = {1},
   Pages = {421-424 vol.1},
   Year = {2001} }

@inproceedings{Iravani_02_PLL_powersystem,
   Author = {Ghartemani, M. K. and Iravani, M. R.},
   Title = {A novel system for measurement of power system parameters and signals},
   BookTitle = {The 2002 45th Midwest Symposium on Circuits and Systems, 2002. MWSCAS-2002. },
   Volume = {1},
   Pages = {I-13-16 vol.1},
   Year = {2002} }

@inproceedings{Blaabjerg_06_FLL_Unbalanced,
   Author = {Rodriguez, P. and Luna, A. and Ciobotaru, M. and Teodorescu, R. and Blaabjerg, F.},
   Title = {Advanced Grid Synchronization System for Power Converters under Unbalanced and Distorted Operating Conditions},
   BookTitle = {IECON 2006 - 32nd Annual Conference on IEEE Industrial Electronics },
   Pages = {5173-5178},
   Year = {2006} }

@inproceedings{Silva_00_WideBandPLL_PV,
   Author = {Amuda, L. N. and Cardoso Filho, B. J. and Silva, S. M. and Silva, S. R. and Diniz, A. S. A. C.},
   Title = {Wide bandwidth single and three-phase PLL structures for grid-tied},
   BookTitle = {Conference Record of the Twenty-Eighth IEEE Photovoltaic Specialists Conference, 2000. },
   Pages = {1660-1663},
   Year = {2000} }

@inproceedings{Blaabjerg_06_SecondOrder_PLL,
   Author = {Ciobotaru, M. and Teodorescu, R. and Blaabjerg, F.},
   Title = {A New Single-Phase PLL Structure Based on Second Order Generalized Integrator},
   BookTitle = {37th IEEE Power Electronics Specialists Conference, 2006. PESC '06. },
   Pages = {1-6},
   Year = {2006} }

@inproceedings{Blaabjerg_06_Robust_PLL_griffault,
   Author = {Timbus, A. V. and Teodorescu, T. and Blaabjerg, F. and Liserre, M. and Rodriguez, P.},
   Title = {PLL Algorithm for Power Generation Systems Robust to Grid Voltage Faults},
   BookTitle = {37th IEEE Power Electronics Specialists Conference, 2006. PESC '06. },
   Pages = {1-7},
   Year = {2006} }

@article{Shinnaka_04_MirrorPhasePLL,
   Author = {Shinnaka, S.},
   Title = {New "mirror-phase vector control" for sensorless drive of permanent-magnet synchronous motor with pole saliency},
   Journal = {IEEE Transactions on Industry Applications },
   Volume = {40},
   Number = {2},
   Pages = {599-606},
   Year = {2004} }

@article{Profumo_05_CurrentControl_SynchFrame,
   Author = {Bojoi, R. I. and Griva, G. and Bostan, V. and Guerriero, M. and Farina, F. and Profumo, F.},
   Title = {Current control strategy for power conditioners using sinusoidal signal integrators in synchronous reference frame},
   Journal = {IEEE Transactions on Power Electronics },
   Volume = {20},
   Number = {6},
   Pages = {1402-1412},
   Year = {2005} }

@article{Diaz_98_newDFT_powrsyst_protection_I,
   Author = {de la O, J. A. and Altuve, H. J. and Diaz, I.},
   Title = {A new digital filter for phasor computation. I. Theory [power system protection]},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {13},
   Number = {3},
   Pages = {1026-1031},
   Year = {1998} }

@article{Diaz_98_newDFT_powrsyst_protection_II,
   Author = {Altuve, H. J. and Diaz, I. and de la O, J. A.},
   Title = {A new digital filter for phasor computation. II. Evaluation [power system protection]},
   Journal = {IEEE Transactions on Power Systems },
   Volume = {13},
   Number = {3},
   Pages = {1032-1037},
   Year = {1998} }

@article{Phadke_83_Recursive_DFT_PMU,
   Author = {Phadke, A. G. and Thorp, J. S. and Adamiak, M. G.},
   Title = {A New Measurement Technique for Tracking Voltage Phasors, Local System Frequency, and Rate of Change of Frequency},
   Journal = {IEEE Transactions on Power Apparatus and Systems },
   Volume = {PAS-102},
   Number = {5},
   Pages = {1025-1038},
   Year = {1983} }

@article{Yeom_09_Kalman_PLL,
   Author = {Yeom, D. H.},
   Title = {Adaptive phase locked loop to improve the readability of optical disc drive},
   Journal = {IEEE Transactions on Consumer Electronics },
   Volume = {55},
   Number = {3},
   Pages = {1380-1382},
   Year = {2009} }

@article{McLaughlin_06_CramerRao_PLL_Postprocessor,
   Author = {Nayak, A. R. and Barry, J. R. and Feyh, G. and McLaughlin, S. W.},
   Title = {Timing Recovery With Frequency Offset and Random Walk: Cram&eacute;r&ndash;Rao Bound and a Phase- Locked Loop Postprocessor},
   Journal = {IEEE Transactions on Communications },
   Volume = {54},
   Number = {11},
   Pages = {2004-2013},
   Year = {2006} }

@article{Patapoutian_99_KalmanPLL,
   Author = {Patapoutian, A.},
   Title = {On phase-locked loops and Kalman filters},
   Journal = {IEEE Transactions on Communications },
   Volume = {47},
   Number = {5},
   Pages = {670-672},
   Year = {1999} }

@article{Driessen_94_AdaptiveKalman_PLL,
   Author = {Driessen, P. F.},
   Title = {DPLL bit synchronizer with rapid acquisition using adaptive Kalman filtering techniques},
   Journal = {IEEE Transactions on Communications},
   Volume = {42},
   Number = {9},
   Pages = {2673-2675},
   Year = {1994} }

@inproceedings{Christiansen_94_PRML_Kalman,
   Author = {Christiansen, G. S.},
   Title = {Modeling of PRML timing loop as a Kalman filter},
   BookTitle = {IEEE Global Telecommunications Conference, 1994. GLOBECOM '94. Communications: The Global Bridge. },
   Volume = {2},
   Pages = {1157-1161 vol.2},
   Year = {1994} }

@article{Lai_96_PLL_SpecialSection,
   Author = {Mao-Fu, Lai and Nakano, M.},
   Title = {Special section on phase-locked loop techniques},
   Journal = {IEEE Transactions on Industrial Electronics},
   Volume = {43},
   Number = {6},
   Pages = {607-608},
   Year = {1996} }

@article{Takano_96_PLL_drives,
   Author = {Takano, A.},
   Title = {Quick-response torque-controlled induction motor drives using phase-locked loop speed control with disturbance compensation},
   Journal = {IEEE Transactions on Industrial Electronics },
   Volume = {43},
   Number = {6},
   Pages = {640-646},
   Year = {1996} }

@article{Nakano_96_DigitalPLL,
   Author = {Kobayashi, F. and Haratsu, M. and Yabumoto, M. and Nakano, M.},
   Title = {Efficient digital techniques for implementing a class of fast phase-locked loops (PLL's)},
   Journal = {IEEE Transactions on Industrial Electronics },
   Volume = {43},
   Number = {6},
   Pages = {616-620},
   Year = {1996} }

@article{Hung_96_PLL_Survey,
   Author = {Guan-Chyun, Hsieh and Hung, J. C.},
   Title = {Phase-locked loop techniques. A survey},
   Journal = {IEEE Transactions on Industrial Electronics},
   Volume = {43},
   Number = {6},
   Pages = {609-615},
   Year = {1996} }

@article{Margaris_96_Nonlinearity_Analog_PLL,
   Author = {Margaris, N. and Mastorocostas, P.},
   Title = {On the Nonlinear Behavior of the Analog Phase-Locked Loop: Synchronization},
   Journal = {IEEE Transactions on Industrial Electronics},
   Volume = {43},
   Number = {6},
   Pages = {621-629},
   Year = {1996} }

@article{Lindsey_81_PLL_Survey,
   Author = {Lindsey, W. C. and Chak Ming, Chie},
   Title = {A survey of digital phase-locked loops},
   Journal = {Proceedings of the IEEE},
   Volume = {69},
   Number = {4},
   Pages = {410-431},
   Year = {1981} }




%%=============================================================================================


%%=======================================Relaying==============================================
@article{Toshiba_98_Wide_area_Protection,
   Author = {Serizawa, Y. and Myoujin, M. and Kitamura, K. and Sugaya, N. and Hori, M. and Takeuchi, A. and Shuto, I. and Inukai, M.},
   Title = {Wide-area current differential backup protection employing broadband communications and time transfer systems},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {13},
   Number = {4},
   Pages = {1046-1052},
   Year = {1998} }

@article{Sidhu_05_NewHalfCycleDFT,
   Author = {Sidhu, T. S. and Xudong, Zhang and Balamourougan, V.},
   Title = {A new half-cycle phasor estimation algorithm},
   Journal = {IEEE Transactions on Power Delivery },
   Volume = {20},
   Number = {2},
   Pages = {1299-1305},
   Year = {2005} }

@article{Sachdev_85_LES_FreqEstimation,
   Author = {Sachdev, M. S. and Giray, M. M.},
   Title = {A Least Error Squares Technique For Determining Power System Frequency},
   Journal = {IEEE Transactions on Power Apparatus and Systems },
   Volume = {PAS-104},
   Number = {2},
   Pages = {437-444},
   Year = {1985} }

@article{Sachdev_85_Kalman_Relaying,
   Author = {Woxd, H. C. and Johnson, N. G. and Sachdev, M. S.},
   Title = {Kulman Filtering Applied to Power System Measurements Relaying},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {PAS-104},
   Number = {12},
   Pages = {3565-3573},
   Year = {1985} }

@article{Phadke_06_Wide-areaProtection,
   Author = {Adamiak, M. G. and Apostolov, A. P. and Begovic, M. M. and Henville, C. F. and Martin, K. E. and Michel, G. L. and Phadke, A. G. and Thorp, J. S.},
   Title = {Wide Area Protection: Technology and Infrastructures},
   Journal = {IEEE Transactions on Power Delivery},
   Volume = {21},
   Number = {2},
   Pages = {601-609},
   Year = {2006} }




%%============================================================================================


%%=============================Kalman Filtering in Power Electronics==========================
@inproceedings{Ghosh_09_Kalman,
   Author = {Zadeh, Ramin Agha and Ghosh, Arindam and Ledwich, Gerard and Zare, Firuz},
   Title = {Online estimation of signal parameters in the presence of harmonic and noise distortion},
   BookTitle = {13th European Conference on Power Electronics and Applications, 2009. EPE '09. },
   Pages = {1-10},
   Year = {2009} }

%%===========================HVDC=========================================================
@ARTICLE{Asher-08-LCC-DFIG,
author={Risheng Li and Bozhko, Serhiy and Asher, G.},
journal={IEEE Transactions on Power Electronics},
title={Frequency Control Design for Offshore Wind Farm Grid With {LCC-HVDC} Link Connection},
year={2008},
month={May},
volume={23},
number={3},
pages={1085-1092}}

@ARTICLE{Bumby-06-DFIG-HVDC,
author={Dawei Xiang and Ran, L. and Bumby, J.R. and Tavner, P.J. and Yang, S.},
journal={IEEE Transactions on Power Delivery},
title={Coordinated control of an {HVDC} link and doubly fed induction generators in a large offshore wind farm},
year={2006},
month={Jan},
volume={21},
number={1},
pages={463-471}}

@article{Fan_09_Windfarm_HVDC_LFC,
   Author = {Lingling, Fan and Zhixin, Miao and Osborn, D.},
   Title = {Wind Farms With {HVDC} Delivery in Load Frequency Control},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {24},
   Number = {4},
   Pages = {1894-1895},
   Year = {2009} }

@ARTICLE{Miao-10-HVDC-WF-FreqSupport,
author={Zhixin Miao and Lingling Fan and Osborn, D. and Yuvarajan, S.},
journal={IEEE Transactions on Energy Conversion},
title={Wind Farms With {HVdc} Delivery in Inertial Response and Primary Frequency Control},
year={2010},
month={Dec},
volume={25},
number={4},
pages={1171-1178}}

@article{ICreport_81_HVDC_dynamics,
   Author = {Report, I. C.},
   Title = {Dynamic Performance Characteristics of North American HVDC Systems for Transient and Dynamic Stability Evaluations},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {PAS-100},
   Number = {7},
   Pages = {3356-3364},
      Year = {1981} }

@article{Taylor_91_HVDcontrols,
   Author = {Taylor, C. W. and Lefebvre, S.},
   Title = {HVDC controls for system dynamic performance},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {6},
   Number = {2},
   Pages = {743-752},
   Year = {1991} }

@article{Stott_77_HVDCloadflow,
   Author = {Reeve, J. and Fahny, G. and Stott, B.},
   Title = {Versatile load flow method for multiterminal HVDC systems},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {96},
   Number = {3},
   Pages = {925-933},
      Year = {1977} }

@article{Mathur_80_HVDCloadflow,
   Author = {El-Marsafawy, M. M. and Mathur, R. M.},
   Title = {A New, Fast Technique for Load-Flow Solution of Integrated Multi-Terminal DC/AC Systems},
   Journal = {IEEE Transactions on Power Apparatus and Systems},
   Volume = {PAS-99},
   Number = {1},
   Pages = {246-255},
      Year = {1980} }


@inproceedings{Hao-93-GuangdongHVDC,
   author = {Chang, Hao},
   title = {Design of modulation controller to damp power oscillations of parallel {AC} line in the Tianshenqiao to Guangdong {HVDC} transmission},
   booktitle = {TENCON '93. IEEE Region 10 Conference on Computer, Communication, Control and Power Engineering},
   pages = {244-247 vol.5},
   year = {1993}
}

@inproceedings{Chen-06-CoordinatedPSSHVDC,
   author = {Chen, R. Y. and Zhang, Y.},
   title = {Coordinated Control of Power System Stabilizers and {HVDC} Damping Controller using Decentralized r-synthesis},
   booktitle = {proceedings of PowerCon International Conference on Power System Technology},
   pages = {1-5},
   year = {2006}
}

@article{Taylor-78-HVDC-Pacific,
   author = {Cresap, R. L. and Mittelstadt, W. A. and Scott, D. N. and Taylor, C. W.},
   title = {Operating Experience with Modulation of the Pacific {HVDC} Intertie},
   journal = {IEEE Transactions on Power Apparatus and Systems},
   volume = {PAS-97},
   number = {4},
   pages = {1053-1059},
   year = {1978}
}

@article{He-GTD09-CSG-HVDC,
   author = {He, J. and Lu, C. and Wu, X. and Li, P. and Wu, J.},
   title = {Design and experiment of wide area {HVDC} supplementary damping controller considering time delay in China southern power grid},
   journal = {IET Generation, Transmission \& Distribution},
   volume = {3},
   number = {1},
   pages = {17-25},
   year = {2009}
}

@inproceedings{Gandhari-09-LocRemVSC-HVDC,
   author = {Latorre, H. F. and Ghandhari, M. and Soder, L.},
   title = {Use of local and remote information in {POD} control of a {VSC-HVDC}},
   booktitle = {proceedings of PowerTech, 2009 IEEE Bucharest},
   pages = {1-6},
   year = {2009}
}

@inproceedings{Peng-07-MultipleHVDC-CSG,
   author = {Li, Licheng and Wu, Xiaochen and Li, Peng},
   title = {Coordinated Control of Multiple {HVDC} systems for damping interarea oscillations in {CSG}},
   booktitle = {proceedings of IEEE PowerAfrica Power Engineering Society Conference and Exposition in Africa},
   pages = {1-7},
   year = {2007}
}

@inproceedings{peng-09-CSGWACS-HVDC-experience,
   author = {Li, Peng and Wu, Xiaochen and Lu, Chao and Shi, Jinghai and Hu, Jiong and He, Jingbo and Zhao, Yong and Xu, Aidong},
   title = {Implementation of {CSG'}s Wide-Area Damping Control System: Overview and experience},
   booktitle = {proceedings of IEEE/PES PSCE Power Systems Conference and Exposition},
   pages = {1-9},
   year = {2009}
}

@article{Melvold-91-WSCC-HVDC-Pacific,
   author = {Martin, D. E. and Wong, W. K. and Dickmander, D. L. and Lee, R. L. and Melvold, D. J.},
   title = {Increasing {WSCC} power system performance with modulation controls on the Intermountain Power Project {HVDC} system},
   journal = {IEEE Transactions on Power Delivery},
   volume = {7},
   number = {3},
   pages = {1634-1642},
   year = {1992}
}

@inproceedings{SiYe07-VSCHVDC-Damping,
   author = {Si-Ye, Ruan and Guo-Jie, Li and Yuan-Zhang, Sun},
   title = {Damping of power swing by the control of {VSC-HVDC}},
   booktitle = {proceedings of IPEC 2007 International Power Engineering Conference},
   pages = {614-618},
   year = {2007}
}

@article{Smed-93-HVDCDamping,
   author = {Smed, T. and Andersson, G.},
   title = {Utilizing {HVDC} to damp power oscillations},
   journal = {IEEE Transactions on Power Delivery},
   volume = {8},
   number = {2},
   pages = {620-627},
   year = {1993}
}

@article{Taylor-91-HVDCControls,
   author = {Taylor, C. W. and Lefebvre, S.},
   title = {{HVDC} controls for system dynamic performance},
   journal = {IEEE Transactions on Power Systems},
   volume = {6},
   number = {2},
   pages = {743-752},
   year = {1991}
}

@article{Hammad-94-coordinated-HVDC-control,
   author = {To, K. W. V. and David, A. K. and Hammad, A. E.},
   title = {A robust co-ordinated control scheme for {HVDC} transmission with parallel AC systems},
   journal = {IEEE Transactions on Power Delivery},
   volume = {9},
   number = {3},
   pages = {1710-1716},
   year = {1994}
}

@inproceedings{Zhang-07-HVDCDamping,
   author = {Xiao-ming, Mao and Yao, Zhang},
   title = {Application of {HVDC} Modulation in Damping Electromechanical Oscillations},
   booktitle = {proceedings of IEEE Power Engineering Society General Meeting},
   pages = {1-6},
   year = {2007}
}

@inproceedings{Xie-06-Coordinated-SVC-HVDC,
   author = {Yong, Chang and Zheng, Xu and Gaihong, Cheng and Jiani, Xie},
   title = {Coordinate damping control of {HVDC} and {SVC} based on wide area signal},
   booktitle = {proceedings of IEEE Power Engineering Society General Meeting},
   pages = {1-7},
   year = {2006}
}

@inproceedings{Wang-03-RGA-FACTS,
   author = {Wang, H. F. and Chen, S. J. and Zhang, P. X. and Cao, Y. J.},
   title = {{RGA} applications in the control of flexible {AC} transmission systems},
   booktitle = {proceedings of IEEE International Symposium on Micro-NanoMechatronics and Human Science},
   volume = {3},
   pages = {1104-1107 Vol. 3},
   year = {2003}
}

@article{Wang-06-GTD-RGA-FACTS,
   author = {Zhang, L. and Zhang, P. X. and Wang, H. F. and Chen, Z. and Du, W. and Cao, Y. J. and Chen, S. J.},
   title = {Interaction assessment of {FACTS} control by {RGA} for the effective design of {FACTS} damping controllers},
   journal = {IEE Proceedings Generation, Transmission and Distribution, },
   volume = {153},
   number = {5},
   pages = {610-616},
   year = {2006}
}

@inproceedings{BristolRGA77,
   author = {Bristol, E. H.},
   title = {Dynamic effects of interaction},
   booktitle = {proceedings IEEE Conference on Decision and Control},
   volume = {16},
   pages = {1096-1100},
   year = {1977}
}

@inproceedings{Cigre_04_VSCHVDCPOD_ABB,
   Author = {Johansson, S. G. and Asplund, G. and Jansson, E. and Rudervall, R.},
   Title = {Power system benefits with VSC DC-transmission systems},
   BookTitle = {Cigre Session 2004},
   Year = {2004}}

@inproceedings{Cigre_07_VSCHVDCPOD_ABB,
   Author = {Zhang, L. and Harnefors, L. and Rey, P.},
   Title = {Power system reliability and transfer capability improvement by {VSC-HVDC}},
   BookTitle = {proceedings of Cigre Regional Meeting 20007},
   Year = {2007}}

@inproceedings{Kling_02_PvsTorq_Eigval,
   Author = {Slootweg, J.G. and Persson, J. and van Voorden, A.M. and Paap, G.C. and Kling, W.L.},
   Title = {A study of the eigenvalue analysis capabilities of power system dynamics simulation software},
   BookTitle = {proceedings of the 14th PSCC, Sevilla, 24-28 June 2002},
   Year = {2002} }

@electronic{ABB,
  title         = "{HVDC} {L}ight",
  url           = "www.abb.com",
 };


@electronic{Siemens,
  title         = "{HVDC} {PLUS}",
  url           = "www.siemens.com",
 };

@electronic{DigSilent,
  title         = "DIgSILENT",
  url           = "http://www.digsilent.de/",
 };

@article{Schauder_93_VectorCntrlASVC,
   Author = {Schauder, C. and Mehta, H.},
   Title = {Vector analysis and control of advanced static VAr compensators},
   Journal = {IEE Proceedings on Generation, Transmission and Distribution},
   Volume = {140},
   Number = {4},
   Pages = {299-306},
   Year = {1993} }

%%===========================Decentralized PSS Design=================================================

@article{Gibbard_04_PSS_design_review,
   Author = {Gibbard, M. J. and Vowles, D. J.},
   Title = {Reconciliation of methods of compensation for PSSs in multimachine systems},
   Journal = {IEEE Transactions on Power Systems},
   Volume = {19},
   Number = {1},
   Pages = {463-472},
   Year = {2004} }

%%=========================Min Norm Controller=========================================================
@article{Kautsky85RobustPlace,
   author = {Kautsky, J. and N.K. Nichols},
   title = {Robust Pole Assignment in Linear State Feedback},
   journal = {International Journal of Control},
   volume = {41},
   pages = {1129-1155},
   year = {1985}
}

@inproceedings{Varga-00-RobustMinNorm,
   author = {Varga, A.},
   title = {Robust pole assignment techniques via state feedback},
   booktitle = {Proceedings of the 39th IEEE Conference on Decision and Control},
   volume = {5},
   pages = {4655-4660},
   year = {2000}
}

%%============================MTDC=====================================================================

@book{Arrillaga-ACDC,
   author = {Arrillaga, J. and Smith, Bruce Dec},
   title = {{AC-DC} power system analysis},
   publisher = {Institution of Electrical Engineers},
   address = {Stevenage},
   year = {1998}
}

@article{Blau-10-Spec-NorthGrid,
   author = {Blau, J.},
   title = {Europe plans a North Sea grid},
   journal = {IEEE Spectrum},
   volume = {47},
   number = {3},
   pages = {12-13},
   year = {2010}
}

@inproceedings{Rudion-10-MTDCoffshoreWind,
  author = {Rudion, K. and Orths, A. and Eriksen, P. B. and Styczynski, Z. A.},
   title = {Toward a benchmark test system for the offshore grid in the north sea},
   booktitle = {IEEE Power and Energy Society General Meeting, 2010},
   pages = {1-8},
   year = {2010}
}

@article{Belmamans10MTDCmodel,
   author = {Cole, S. and Beerten, J. and Belmans, R.},
   title = {Generalized Dynamic {VSC} {MTDC} Model for Power System Stability Studies},
   journal = {IEEE Transactions on Power Systems},
   volume = {25},
   number = {3},
   pages = {1655-1662},
   year = {2010}
}


@article{Zhang01MTDCstateEstim,
   author = {Ding, Q. and Chung, T. S. and Zhang, B. M.},
   title = {An Improved Sequential Method for AC/MTDC Power System State Estimation},
   journal = {IEEE Power Engineering Review},
   volume = {21},
   number = {8},
   pages = {59-59},
   year = {2001}
}

@inproceedings{AnayaLara-08-MTDCwind,
   author = {Gonzalez-Hernandez, S. and Moreno-Goytia, E. and Fraga-Aguilar, M. and Anaya-Lara, O.},
   title = {Integration of wind power using a multiterminal VSC-HVDC link: Steady-state analysis},
   booktitle = {IEEE/PES Transmission and Distribution Conference and Exposition: Latin America, 2008},
   pages = {1-6},
   year = {2008}
}

@inproceedings{Hairong-06-VSCMTDCcontrol,
   author = {Hairong, Chen and Chao, Wang and Fan, Zhang and Wulue, Pan},
   title = {Control Strategy Research of {VSC} Based Multiterminal {HVDC} System},
   booktitle = {IEEE PES Power Systems Conference and Exposition, 2006. PSCE '06. 2006},
   pages = {1986-1990},
   year = {2006}
}

@inproceedings{Zhang-91-MTDCcontrol,
   author = {Hanchu, Zheng and Shousun, Chen and Yixin, Ni and Baolin, Zhang},
   title = {A study of multi-terminal DC modulation control},
   booktitle = {International Conference on Advances in Power System Control, Operation and Management, 1991. APSCOM-91., 1991},
   pages = {615-620 vol.2},
   year = {1991}
}

@inproceedings{Jenkins-09-MTDCcontrol,
   author = {Jun, Liang and Gomis-Bellmunt, O. and Ekanayake, J. and Jenkins, N.},
   title = {Control of multi-terminal VSC-HVDC transmission for offshore wind power},
   booktitle = {13th European Conference on Power Electronics and Applications, 2009. EPE '09},
   pages = {1-10},
   year = {2009}
}

@article{Lefebvre-91-MTDCstability,
   author = {Lefebvre, S. and Wong, W. K. and Reeve, J. and Baker, M. and Chapman, D.},
   title = {Considerations for modeling {MTDC} systems in transient stability programs},
   journal = {IEEE Transactions on Power Delivery},
   volume = {6},
   number = {1},
   pages = {397-404},
   year = {1991}
}

@article{Lefebvre-91-MTDCstability2,
   author = {Lefebvre, S. and Wong, W. K. and Reeve, J. and Gagnon, J. M. and Johnson, B. K.},
   title = {Experience with modeling {MTDC} systems in transient stability programs},
   journal = {IEEE Transactions on Power Delivery},
   volume = {6},
   number = {1},
   pages = {405-413},
   year = {1991}
}

@inproceedings{Bjorklund-08-MTDCchallenge,
   author = {Lescale, V. F. and Kumar, A. and Juhlin, L. E. and Bjorklund, H. and Nyberg, K.},
   title = {Challenges with Multi-Terminal UHVDC Transmissions},
   booktitle = {Joint International Conference on Power System Technology and IEEE Power India Conference, 2008. POWERCON 2008},
   pages = {1-7},
   year = {2008}
}

@inproceedings{Bazargan-09-MTDCoffshoreWind,
   author = {Lie, Xu and Liangzhong, Yao and Bazargan, M.},
   title = {{DC} grid management of a multi-terminal {HVDC} transmission system for large offshore wind farms},
   booktitle = {International Conference on Sustainable Power Generation and Supply, 2009. SUPERGEN '09},
   pages = {1-7},
   year = {2009}
}

@inproceedings{Lie-08-MTDCoffshoreWind,
  author = {Lie, Xu and Williams, B. W. and Liangzhong, Yao},
   title = {Multi-terminal {DC} transmission systems for connecting large offshore wind farms},
   booktitle = {IEEE Power and Energy Society General Meeting - Conversion and Delivery of Electrical Energy in the 21st Century, 2008},
   pages = {1-7},
   year = {2008}
}

@inproceedings{Padiyar-91-MTDCssr,
   author = {Padiyar, K. R. and Geetha, M. K.},
   title = {Study of torsional interactions in multi-terminal DC systems through small signal stability analysis},
   booktitle = {International Conference on AC and DC Power Transmission, 1991},
   pages = {411-413},
   year = {1991}
}

@article{Zhang-01-MTDCstateEstim,
   author = {Qifeng, Ding and Chung, T. S. and Boming, Zhang},
   title = {An improved sequential method for AC/MTDC power system state estimation},
   journal = {IEEE Transactions on Power Systems},
   volume = {16},
   number = {3},
   pages = {506-512},
   year = {2001}
}

@inproceedings{Jenkins-09-MTDCoffshoreWind,
   author = {Shu, Zhou and Jun, Liang and Ekanayake, J. B. and Jenkins, N.},
   title = {Control of multi-terminal VSC-HVDC transmission system for offshore wind power generation},
   booktitle = {Proceedings of the 44th International Universities Power Engineering Conference (UPEC), 2009},
   pages = {1-5},
   year = {2009}
}

@inproceedings{Tao-09-MTDCcoordinatedWind,
   author = {Tao, Ding and Chengxue, Zhang and Zhijian, Hu and Zhiyuan, Duan},
   title = {Coordinated control strategy for multi-terminal {VSC-HVDC} based wind farm interconnection},
   booktitle = {International Conference on Sustainable Power Generation and Supply, 2009. SUPERGEN '09},
   pages = {1-6},
   year = {2009}
}

@inproceedings{Undeland-09-MTDCunbalance,
   author = {Torres-Olguin, R. E. and Undeland, T. M.},
   title = {An adaptive direct power control for multi-terminal {HVDC} transmission system under unbalanced conditions},
   booktitle = {International Conference on Electric Power and Energy Conversion Systems, 2009. EPECS '09},
   pages = {1-6},
   year = {2009}
}

@article{Ooi-01-MTDCwind,
   author = {Weixing, Lu and Boon Teck, Ooi},
   title = {Multi-terminal {DC} transmission system for wind-farms},
   booktitle = {IEEE Power Engineering Society Winter Meeting, 2001},
   volume = {3},
   pages = {1091-1096 vol.3},
   year = {2001}
}

@article{Ooi-05-MTDCwind,
   author = {Weixing, Lu and Boon-Teck, Ooi},
   title = {Premium quality power park based on multi-terminal {HVDC}},
   journal = {IEEE Transactions on Power Delivery},
   volume = {20},
   number = {2},
   pages = {978-983},
   year = {2005}
}

@article{Zhang-04-MTDCpowerFlow,
   author = {Xiao-Ping, Zhang},
   title = {Multiterminal voltage-sourced converter-based {HVDC} models for power flow analysis},
   journal = {IEEE Transactions on Power Systems},
   volume = {19},
   number = {4},
   pages = {1877-1884},
   year = {2004}
}

@article{Ooi-07-MTDCFault,
   author = {Lianxiang, Tang and Boon-Teck, Ooi},
   title = {Locating and Isolating {DC} Faults in Multi-Terminal {DC} Systems},
   journal = {IEEE Transactions on Power Delivery},
   volume = {22},
   number = {3},
   pages = {1877-1884},
   year = {2007}
}

@article{Ooi-02-MTDCprotection,
   author = {Tang, Lianxiang and Ooi, Boon-Teck},
   title = {Protection of {VSC}-multi-terminal {HVDC} against {DC} faults},
   journal = {in IEEE Annual Power Electronics Specialists Conference},
   volume = {2},
   pages = {719-724},
   year = {2002}
}

@article{Ooi-08-MTDCprotection,
   author = {Lianxiang, Tang and Boon-Teck, Ooi},
   title = {Elimination of "Harmonic Transfer Through Converters" in {VSC}-Based Multiterminal {DC} Systems by {AC/DC} Decoupling},
   journal = {IEEE Transactions on Power Delivery},
   volume = {23},
   number = {1},
   pages = {402-409},
   year = {2008}
}

@inproceedings{Lin-05-MTDCcontrol,
   author = {Fei, Lin and Zhiwen, Ma and Xiaojie, You and Trillion, Zheng},
   title = {The grid connected converter control of multi-terminal {DC} system for wind farms},
   booktitle = {Proceedings of the Eighth International Conference on Electrical Machines and Systems, 2005. ICEMS 2005},
   volume = {2},
   pages = {1021-1023 Vol. 2},
   year = {2005}
}

@inproceedings{Zheng-06-MTDCcontrol,
   author = {Zheng, Chao and Zhou, Xiaoxin and Ruomei, L.},
   title = {Dynamic Modeling and Transient Simulation for {VSC} based {HVDC} in Multi-Machine System},
   booktitle = {International Conference on Power System Technology, 2006. PowerCon 2006},
   pages = {1-7},
   year = {2006}
}

@inproceedings{Padiyar-04-VSC-HVDC,
   author = {Padiyar, K. R. and Prabhu, N.},
   title = {Modelling, control design and analysis of VSC based HVDC transmission systems},
   booktitle = {International Conference on Power System Technology, 2004. PowerCon 2004},
   volume = {1},
   pages = {774-779},
   year = {2004}
}

@inproceedings{Padiyar-04-VSC-HVDC,
   author = {Giddani, O. A. and Adam, G. P. and Anaya-Lara, O. and Lo, K. L.},
   title = {Grid integration of a large offshore wind farm using {VSC-HVDC} in parallel with an {AC} submarine cable},
   booktitle = {Universities Power Engineering Conference (UPEC), 2009 Proceedings of the 44th International},
   pages = {1-5},
   year = {2009}
}

@inproceedings{Kjetil-10-FreqCntrlMTDC,
  author = {Haileselassie, T. M. and Uhlen, K.},
   title = {Primary Frequency Control of Remote Grids Connected by Multi-terminal {HVDC}},
   booktitle = {IEEE Power and Energy Society General Meeting},
   year = {2010}
}

@inproceedings{Kling-10-WindMTDC,
  author = {van der Meer, A. A. and Hendriks, R.L. and Kling, W.L.},
   title = {Combined Stability and Electro-Magnetic Transients Simulation of Offshore Wind Power Connected through Multi-Terminal {VSC-HVDC}},
   booktitle = {IEEE Power and Energy Society General Meeting},
   year = {2010}
}

@inproceedings{PSCAD,
   year = {PSCAD/EMTDC v. 4.2.1, Manitoba HVDC Research Centre, Winnipeg, MB, Canada}
}

@article{Yazdani-06-DCsideControlNPC,
   author = {Yazdani, A. and Iravani, R.},
   title = {An accurate model for the {DC}-side voltage control of the neutral point diode clamped converter},
   journal = {IEEE Transactions on Power Delivery},
   volume = {21},
   number = {1},
   pages = {185-193},
   year = {2006}
}

@article{Udaya-09-MIDC-interaction,
   author = {Karawita, C. and Annakkage, U. D.},
   title = {Multi-Infeed {HVDC} Interaction Studies Using Small-Signal Stability Assessment},
   journal = {IEEE Transactions on Power Delivery},
   volume = {24},
   number = {2},
   pages = {910-918},
   year = {2009}
}

@article{Sanders-91-StateSpaceAveraging,
   author = {Sanders, S. R. and Noworolski, J. M. and Liu, X. Z. and Verghese, G. C.},
   title = {Generalized averaging method for power conversion circuits},
   journal = {IEEE Transactions on Power Electronics},
   volume = {6},
   number = {2},
   pages = {251-259},
   year = {1991}
}

@article{Yang-10-MTDCProtection,
   author = {Jin, Yang and Fletcher, J. E. and O'Reilly, J.},
   title = {Multiterminal DC Wind Farm Collection Grid Internal Fault Analysis and Protection Design},
   journal = {IEEE Transactions on Power Delivery},
   volume = {25},
   number = {4},
   pages = {2308-2318},
   year = {2010}
}

@inproceedings{Pipelzadeh-10-WideAreaHVDC,
   author = {Pipelzadeh, Y. and Chaudhuri, B. and Green, T. C.},
   title = {Wide-area power oscillation damping control through HVDC: A case study on Australian equivalent system},
   booktitle = {2010 IEEE Power and Energy Society General Meeting},
   pages = {1-7}
}


%%%%% For IP %%%%%%%%%%%%%%
@article{Nee-10-VSC_PowSynchCntrl,
    author = {Lidong, Zhang and Harnefors, L. and Nee, H. P.},
   title = {Power-Synchronization Control of Grid-Connected Voltage-Source Converters},
   journal = {IEEE Transactions on Power Systems},
   volume = {25},
   number = {2},
   pages = {809-820},
   year = {2010}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Smart Grids %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@article{NIST-10-SmartGridStandard,
    author = {Office of the National -Coordinator for Smart Grid Interoperability},
   title = {{NIST} framework and roadmap for smart grid interoperability standards, Release 1.0},
   journal = {National Institute of Standards and Technology},
   year = {2010}
}

@article{NETL-09-SmartGridVision,
    author = {National Energy Technology Laboratory and U.S. DOE Office of Electricity Delivery and Energy Reliability},
   title = {A vision for the smart grid},
   year = {2009}
}

@article{Myrda-10-SmartGridAssetManagaement,
    author = {Myrda, Paul},
   title = {Optimizing Assets: Smart grid-enabled asset management},
   journal = {http://www.ieee-pes.org/enews-update/292-optimizing-assets-smart-grid-enabled-asset-management}
}

@article{IEEE-P2030-WorkinGroup,
    author = {Heile, Bob},
   title = {{IEEE} Standard 2030 Guide for Smart Grid Interoperability of Energy Technology and Information Technology operation with the Electric Power System ({EPS}) and End-Use Applications and Loads
},
   journal = {www.ieee802.org/}
}


@Misc{AustralianSystem,
                author = {Gibbard, M and Vowles, D. },
                title = {Simplified 14-Generator Model Of The SE Australian Power System},
                year = 2007,
                howpublished = {http://www.eleceng.adelaide.edu.au/groups/PCON/PowerSystems/IEEE/}}

%============================2014==============================================
@book{Flood,
   author = {Flood, J. E.},
   title = {Telecommunication Networks},
   publisher = {IET},
   address = {London, UK},
   year = {1997}
}
@article{Nee-10-VSC_PowSynchCntrl,
    author = {Lidong, Zhang and Harnefors, L. and Nee, H. P.},
   title = {Power-Synchronization Control of Grid-Connected Voltage-Source Converters},
   journal = {IEEE Transactions on Power Systems},
   volume = {25},
   number = {2},
   pages = {809-820},
   year = {2010}
}

@ARTICLE{Wang-12-DelayNCS,
author={Shaobu Wang and Xiangyu Meng and Tongwen Chen},
journal={IEEE Transactions on Control Systems Technology},
title={Wide-Area Control of Power Systems Through Delayed Network Communication},
year={2012},
month={March},
volume={20},
number={2},
pages={495-503},
}

@ARTICLE{Hongbo-09-EDA_NCS,
author={Hongbo Li and Mo-Yuen Chow and ZengQi Sun},
journal={IEEE Transactions on Industrial Electronics},
title={EDA-Based Speed Control of a Networked DC Motor System With Time Delays and Packet Losses},
year={2009},
month={May},
volume={56},
number={5},
pages={1727-1735}
}
@inproceedings{Sastry-08-LQGpacketLoss,
   author = {Sinopoli, B. and Schenato, L. and Franceschetti, M. and Poolla, K. and Sastry, S.},
   title = {Optimal linear {LQG} control over lossy networks without packet acknowledgment},
   booktitle = {Asian J. Control},
   volume = {10},
   pages = {3-13},
   year = {2008}
}

@inproceedings{Yu-08-MarkovChain,
   author = {Yu, X. and Modestino, J. W. and Tian X.},
   title = {The accuracy of Markov chain models in predicting packet-loss statistics for a single multiplexer,},
   booktitle = {IEEE Trans. Inf. Theory},
   volume = {54},
   number={1},
   pages = {489-501},
   year = {2008}
}

@inproceedings{Nilanjan-13-DFIG-POD,
   author = {Chaudhuri, N. R. and Chaudhuri, B.},
   title = {Considerations Toward Coordinated Control of DFIG-Based WInd Farms},
   booktitle = {IEEE Transactions on Power Delivery},
   volume = {28},
   number={3},
   pages = {1263-1270},
   year = {2013}
}

@inproceedings{Sinopoli-04-IntermittentKalman,
   author = {Sinopoli, B. and Schenato, L. and Franceschetti, M. and Poolla, K. and Jordan, M. and
Sastry, S.},
   title = {Kalman filtering with intermittent observations,},
   booktitle = {IEEE Transactions on Automatic Control},
   volume = {49},
   number={9},
   pages = {1453-1464},
   year = {2004}
}

@INPROCEEDINGS{Nilanjan-11-DFIG_HVDC,
author={Chaudhuri, N.R. and Chaudhuri, B.},
booktitle={IEEE Power and Energy Society General Meeting, 2011 },
title={Impact of wind penetration and HVDC upgrades on dynamic performance of future grids},
year={2011},
month={July}
}

@book{Mariton,
   author = {Mariton, M.},
   title = {Jump Linear Systems in Automatic Control},
   publisher = {Marcel Dekker},
   address = {New York},
   year = {1990}
}

@ARTICLE{Gilbert,
author={Gilbert, E. K.},
journal={Bell Sys. Tech. Journal},
title={Capacity of a burst-noise channel},
month={Sept},
volume={39},
pages={1253},
year = {1960}
}

%============================2015==============================================
@inproceedings{Adibi-87-Restoration,
   author = {Adibi, M. M. et al.},
   title = {Power system restoration - a task force report,},
   booktitle = {IEEE Transactions on Power Systems},
   volume = {2},
   number={2},
   pages = {271-277},
   year = {1987}
}
@ARTICLE{RestorationTF-87,
author={Adibi, M.M. and Borkoski, J.N. and Kafka, R.J.},
journal={IEEE Transactions on Power Systems},
title={Power System Restoration - The Second Task Force Report},
year={1987},
month={Nov},
volume={2},
number={4},
pages={927-932}
}

@ARTICLE{Fink-95-Restoration,
author={Fink, L.H. and Liou, Kan-Lee and Chen-Ching Liu},
journal={IEEE Transactions on Power Systems},
title={From generic restoration actions to specific restoration strategies},
year={1995},
month={May},
volume={10},
number={2},
pages={745-752}}

@ARTICLE{Vittal-10-WindVstab,
author={Vittal, E. and O'Malley, M. and Keane, A.},
journal={IEEE Transactions on Power Systems},
title={A Steady-State Voltage Stability Analysis of Power Systems With High Penetrations of Wind},
year={2010},
month={Feb},
volume={25},
number={1},
pages={433-442}}

@INPROCEEDINGS{Ledwich-06-DFIG_BlackStart,
author={Aktarujjaman, M. and Kashem, M.A. and Negnevitsky, M. and Ledwich, G.},
booktitle={International Conference on Power Electronics, Drives and Energy Systems, 2006. PEDES '06},
title={Black start with {DFIG} based distributed generation after major emergencies},
year={2006},
month={Dec},
pages={1-6}}

@article{PJM-13-Restoration,
   title = {{PJM} Manual 36: System Restoration},
   year={2013},
    month={Jun},
   journal = {http://www.pjm.com/~/ media/documents/manuals/m36.ashx.}
}

@article{MISO-12-Restoration,
    author = {MISO},
   title = {{MISO} Real Time Operations - Power System Restoration Plan, Version 4.2.},
   year={2012},
    month={Dec},
}

@inproceedings{CPLEX,
   year = {IBM ILOG CPLEX Optimization Studio. Online: http://www-03.ibm.com/software/products/ en/ibmilogcpleoptistud}
}

@ARTICLE{Kling-06-WindInertia,
author={Morren, J. and de Haan, S.W.H. and Kling, W.L. and Ferreira, J.A.},
journal={IEEE Transactions on Power Systems},
title={Wind turbines emulating inertia and supporting primary frequency control},
year={2006},
month={Feb},
volume={21},
number={1},
pages={433-434}}

@ARTICLE{Hansen-13-WF_FrequencyControl,
author={Wang-Hansen, M. and Josefsson, R. and Mehmedovic, H.},
journal={IEEE Transactions on Sustainable Energy},
title={Frequency Controlling Wind Power Modeling of Control Strategies},
year={2013},
month={Oct},
volume={4},
number={4},
pages={954-959}}

@MISC{Dupacova03scenarioreduction,
    author = {J. Dupacova and N. Growe-Kuska and W. Romisch},
    title = {Scenario Reduction in Stochastic Programming: An Approach Using Probability Metrics},
    year = {2003}
}

@INPROCEEDINGS{Growe-03-ScenarioReduction,
author={Growe-Kuska, N. and Heitsch, H. and Romisch, W.},
booktitle={2003 IEEE Bologna Power Tech Conference Proceedings},
title={Scenario reduction and scenario tree construction for power management problems},
year={2003},
month={June},
volume={3},
pages={7}}

@ARTICLE{Trodden-14-Islanding,
author={Trodden, P.A. and Bukhsh, W.A. and Grothey, A. and McKinnon, K.I.M.},
journal={IEEE Transactions on Power Systems},
title={Optimization-Based Islanding of Power Networks Using Piecewise Linear {AC} Power Flow},
year={2014},
month={May},
volume={29},
number={3},
pages={1212-1220}}

@ARTICLE{Wei-11-OptimalStartup,
author={Wei Sun and Chen-Ching Liu and Li Zhang},
journal={IEEE Transactions on Power Systems},
title={Optimal Generator Start-Up Strategy for Bulk Power System Restoration},
year={2011},
month={Aug},
volume={26},
number={3},
pages={1357-1366}}

@INPROCEEDINGS{Wei-13-OptimalTransmissionPathSearch,
author={Wei Sun and Chen-Ching Liu},
booktitle={Bulk Power System Dynamics and Control - IX Optimization, Security and Control of the Emerging Power Grid (IREP), 2013 IREP Symposium},
title={Optimal transmission path search in power system restoration},
year={2013},
month={Aug},
pages={1-5}}

@ARTICLE{Adibi-99-PrimeMoverResponse,
author={Adibi, M.M. and Borkoski, J.N. and Kafka, R.J. and Volkmann, T.L.},
journal={IEEE Transactions on Power Systems},
title={Frequency response of prime movers during restoration},
year={1999},
month={May},
volume={14},
number={2},
pages={751-756}}

@INPROCEEDINGS{Wei-14-BatteryRestoration,
author={Kadel, N. and Wei Sun and Qun Zhou},
booktitle={2014 IEEE PES General Meeting Conference Exposition},
title={On battery storage system for load pickup in power system restoration},
year={2014},
month={July},
pages={1-5}}

@book{glasserman2003monte,
  author={Glasserman, P.},
  title={Monte Carlo Methods in Financial Engineering},
  series={Applications of mathematics},
  year={2003},
  publisher={Springer}
}

@inproceedings{NERCstandard,
   year = {NERC Standard EOP-005-2 - System Restoration from Blackstart Resources. Online: http://www.nerc.com/files/EOP-005-2.pdf}
}

@INPROCEEDINGS{Adibi-08-RestorationDynamics,
author={Adibi, M.M. and Martins, N.},
booktitle={2008 IEEE Power and Energy Society General Meeting - Conversion and Delivery of Electrical Energy in the 21st Century},
title={Power system restoration dynamics issues},
year={2008},
month={July},
pages={1-8}}

@inproceedings{PSSE,
   year = {PSS/E, "Program Operation Manual," {SIEMENS} Power Technologies, Inc., New York, USA}
}

@inproceedings{ETRAN_PLUS,
   year = {E-TRAN PLUS, ELECTRANIX Corporation, Winnipeg, Canada, http://www.electranix.com/software/e-tran-plus/}
}

@ARTICLE{Abdelkader-12-TheveninPMU,
author={Abdelkader, S.M. and Morrow, D.J.},
journal={IEEE Transactions on Power Systems},
title={Online Tracking of Thevenin Equivalent Parameters Using PMU Measurements},
year={2012},
month={May},
volume={27},
number={2},
pages={975-983}}
	
@phdthesis{Sunthesis09,
   Author = {Sun, Rui},
   Title = {Voltage stability indices based on active power transfer using simulated phasor measurements},
   Note = {Department of Electrical and Computer
   Engineering, Clemson University.},
   Type = {PhD Dissertation},
   Year = {2009} }

@article{Carlsson2005147,
title = "Using cheap talk as a test of validity in choice experiments ",
journal = "Economics Letters ",
volume = "89",
number = "2",
pages = "147 - 152",
year = "2005",
author = "Fredrik Carlsson and Peter Frykblom and Carl Johan Lagerkvist"
}

@article{Chang-13-WTP,
title = "Consumer Characteristics and Willingness to Pay for Locally Produced Rib-eye Steaks: A Case Study of Consumers at Farmers' Markets",
journal = "Journal of Agriculture, Food system, and Community Development",
pages = "1�23",
year = "2013",
author = "Chang, Kuo-Liang and Xu, P. and Warmann, G. and Lone, T. and Munzimi, Z. and Opoku, E"
}

@article{Faruqui-01-CaliforniaCrisis,
title = "Analyzing {California's} Power Crisis",
journal = "Energy Journal",
pages = "29-52",
year = "2001",
author = "Faruqui, A. and H-P. Chao and V. Niemeyer and J. Platt and K. Stahlkopf"
}

@article{Lancaster-66-Consumer,
title = "A new approach to consumer theory",
journal = "Journal of Political Economy",
volume="74",
pages = "132-157",
year = "1966",
author = "Lancaster, K."
}

@article{Lagerkvist-06-Consumer,
title = "Swedish consumer preference for animal welfare and biotech: A choice experiment",
journal = "AgBioForum",
volume="9",
number = "1",
pages = "51-58",
year = "2006",
author = "Lagerkvist, C. J. and F. Carlsson and D. Viske"
}

@article{Scarpa-13-Attributes,
title = "Inferred and stated attribute non-attendance in food choice experiments",
journal = "American Journal of Agricultural Economics",
volume="95",
number = "1",
pages = "165-180",
year = "2013",
author = "Scarpa, R. and Zanoli and R. Bruschi and and V. Naspetti"
}


@article{Thaler-85-Consumer,
title = "Mental accounting and consumer choice",
journal = "Marketing Science",
volume="4",
pages = "199-214",
year = "1985",
author = "Thaler, R.H."
}

@article{Thaler-99-Mental,
title = "Mental accounting matters",
journal = "Journal of Behavioral Decision Making",
volume="12",
pages = "183-206",
year = "1999",
author = "Thaler, R.H."
}

@inproceedings{NOAA,
   year = {National Climate Data Center {(NOAA)} (2015). Billion Dollar Weather and Climate Disasters: Tables and Events. Last Retrieved 02/12/15: http://www.ncdc.noaa.gov/billions/events.}
}

@INPROCEEDINGS{Zhou-09-Blackstart,
author={Mingxia Zhou and Sheng Li and Jianhua Zhang and Zongqi Liu and Yinhui Li},
booktitle={IEEE 6th International Power Electronics and Motion Control Conference, 2009. IPEMC '09},
title={A study on the black start capability of {VSC-HVDC} using soft-starting mode},
year={2009},
month={May},
pages={910-914}}

@INPROCEEDINGS{Hafner-08-VSCHVDC,
author={Ying Jiang-Hafner and Duchen, H. and Karlsson, M. and Ronstrom, L. and Abrahamsson, B.},
booktitle={IEEE/PES Transmission and Distribution Conference and Exposition, 2008. T\&D},
title={{HVDC} with voltage source converters - a powerful standby black start facility},
year={2008},
month={April},
pages={1-9}}

@INPROCEEDINGS{Li-09-BlackStart,
author={Sheng Li and Mingxia Zhou and Zongqi Liu and Jianhua Zhang and Yinhui Li},
booktitle={SUPERGEN '09. International Conference on Sustainable Power Generation and Supply, 2009},
title={A study on {VSC-HVDC} based black start compared with traditional black start},
year={2009},
month={April},
pages={1-6}}

@article{Cook-15-Draught,
	author = {Cook, Benjamin I. and Ault, Toby R. and Smerdon, Jason E.},
	title = {Unprecedented 21st century drought risk in the {American} {Southwest} and {Central} {Plains}},
	volume = {1},
	number = {1},
	year = {2015},
	publisher = {American Association for the Advancement of Science},
	journal = {Science Advances}
}


@inproceedings{Caring,
   year = {{IUCN/UNEP/WWF} (1991). "Caring for the Earth: A Strategy for Sustainable Living." Gland, Switzerland.}
}


@article{IPCC,
	author = {Working Group III of the IPCC},
	title = {{IPCC} (2011a): {IPCC} Special Report on Renewable Energy Sources and Climate Change Mitigation},
	publisher = {Cambridge University Press},
pages = {1075}
}
@ARTICLE{Hopkinson-06-EPOCHS,
author={Hopkinson, K. and Xiaoru Wang and Giovanini, R. and Thorp, J. and Birman, K. and Coury, D.},
journal={IEEE Transactions on Power Systems},
title={{EPOCHS}: a platform for agent-based electric power and communication simulation built from commercial off-the-shelf components},
year={2006},
month={May},
volume={21},
number={2},
pages={548-558}}

@ARTICLE{Lin-12-GECO,
author={Hua Lin and Veda, S.S. and Shukla, S.S. and Mili, L. and Thorp, J.},
journal={IEEE Transactions on Smart Grid},
title={{GECO}: Global Event-Driven Co-Simulation Framework for Interconnected Power System and Communication Network},
year={2012},
month={Sept},
volume={3},
number={3},
pages={1444-1456}}

@INPROCEEDINGS{Deng-13-CoSimulation,
author={Yi Deng and Hua Lin and Shukla, S. and Thorp, J. and Mili, L.},
booktitle={2013 Workshop on Modeling and Simulation of Cyber-Physical Energy Systems (MSCPES)},
title={Co-simulating power systems and communication network for accurate modeling and simulation of {PMU} based wide area measurement systems using a global event scheduling technique},
year={2013},
month={May},
pages={1-6}}

@INPROCEEDINGS{Lin-12-CyberSecurity,
author={Hua Lin and Yi Deng and Shukla, S. and Thorp, J. and Mili, L.},
booktitle={2012 IEEE Third International Conference on Smart Grid Communications (SmartGridComm)},
title={Cyber security impacts on all-{PMU} state estimator - a case study on co-simulation platform {GECO}},
year={2012},
month={Nov},
pages={587-592}}

@inproceedings{DOE2008,
   year = {U.S. Department of Energy, Tech. Rep. May 2008. ``20\% wind energy by 2030: Increasing wind energy's contribution
to U.S. electricity supply" }
}

@inproceedings{JCSP2008,
   year = {Midwest ISO, PJM, SPP and TVA, Tech. Rep., 2008. ``Joint coordinated system plan 2008," Available: http://www.jcspstudy.org/}
}

@inproceedings{DOE2009,
   year = {U.S. Department of Energy, Dec 2009. "National electric transmission congestion
study."}
}

@INPROCEEDINGS{McCally-12-NationalTransmission,
author={J. McCalley and J. Bushnell and V. Krishnan, and S. Cano},
booktitle={in PSERC, White Paper},
title={Transmission design at the national level: Benefits, risks, and possible paths forward},
year={2012},
month={Jan}}

@inproceedings{FrndsOfSuperGrid,
   year = {Website of "Position Papers and Proposals for Friends of the Supergrid,"},
   title = {www.friendsofthesupergrid.eu/position_papers_proposals.aspx.}
}

@INPROCEEDINGS{McDonald-14-Seminar,
author={A.E. McDonald, and C. Clack},
booktitle={Sustainable Energy and Atmospheric Sciences Seminar, NOAA, NREL, and CU-Boulder RASEI},
title={Low Cost and Low Carbon Emission Wind and Solar Energy Systems are Feasible for Large Geographic Domains},
year={2014},
month={May}}

@ARTICLE{McCalley-14-InterRegionalGrid,
author={Yifan Li and McCalley, J.D.},
journal={IEEE Transactions on Power Systems},
title={Design of a High Capacity Inter-Regional Transmission Overlay for the U.S.},
year={2015},
month={Jan},
volume={30},
number={1},
pages={513-521}}

@inproceedings{HVDC_market,
   year = {"Report: HVDC converters globally to hit 89.6 billion by 2020," http://www.windpowerengineering.com/featured/business-news-projects/report-hvdc-converters-globally-hit-89-6-billion-2020/}
}

@inproceedings{CigreB4,
   year = {CIGRE' B4 website, http://b4.cigre.org/}
}

@inproceedings{Twenties,
   year = {Twenties project website, http://www.twenties-project.eu/node/1}
}

@inproceedings{Atlantic,
   year = {Atlantic Wind Connection, http://atlanticwindconnection.com/awc-projects/awc-technology}
}


@inproceedings{clean,
   year = {Clean Line Energy, http://www.rockislandcleanline.com/site/home}
}
@INPROCEEDINGS{HMTDC-Nguyen-12,
author={Mai Huong Nguyen and Saha, T.K. and Eghbal, M.},
booktitle={2012 22nd Australasian Universities Power Engineering Conference (AUPEC)},
title={Investigation on the impact of hybrid multi-terminal HVDC system combining LCC and VSC technologies using system identification},
year={2012},
month={Sept},
pages={1-6}}

@INPROCEEDINGS{HMTDC-Yuan-06,
author={Yuan, X.F. and Cheng, S.J.},
booktitle={2005/2006 IEEE PES Transmission and Distribution Conference and Exhibition},
title={Simulation Study for a Hybrid Multi-terminal HVDC System},
year={2006},
month={May},
pages={720-725}}

@INPROCEEDINGS{HMTDC-Yulule-06,
author={Wulue Pan and Yong Chang and Hairong Chen},
booktitle={2006 IEEE PES Power Systems Conference and Exposition, 2006. PSCE '06.},
title={Hybrid Multi-terminal HVDC System for Large Scale Wind Power},
year={2006},
month={Oct},
pages={755-759}}

@ARTICLE{HMTDC-Dong-15_TPWRD,
author={Dong, S. and Chi, Yong-Ning and Li, Y.},
journal={Power Delivery, IEEE Transactions on},
title={Active Voltage Feedback Control for Hybrid Multi-terminal HVDC System Adopting Improved Synchronverters},
year={2015},
month={},
volume={PP},
number={99},
pages={1-1}}

@ARTICLE{HMTDC-IET-Nguyen-15,
author={Nguyen, M.H. and Saha, T.K. and Eghbal, M.},
journal={IET Generation, Transmission Distribution},
title={Input/output selection for wide-area power oscillation damper of hybrid multi-terminal high-voltage direct current to connect remotely located renewable energy resources},
year={2015},
month={},
volume={9},
number={5},
pages={483-493}}

@INPROCEEDINGS{HMTDC-Cheng-13,
author={Cheng-hao Li and Peng Zhan and Jin-yu Wen and Mei-qi Yao and Nai-hu Li and Wei-Jen Lee},
booktitle={2013 IEEE Industry Applications Society Annual Meeting},
title={Offshore wind farms integration and frequency support control utilizing hybrid multi-terminal HVDC transmission},
year={2013},
month={Oct},
pages={1-9}}

@ARTICLE{Almeida-07-DFIG_FreqSupport,
author={de Almeida, R.G. and Peas Lopes, J.A.},
journal={IEEE Transactions on Power Systems},
title={Participation of Doubly Fed Induction Wind Generators in System Frequency Regulation},
year={2007},
month={Aug},
volume={22},
number={3},
pages={944-950}}

@ARTICLE{Nilanjan-13-MTDCfreqSupport,
author={Chaudhuri, N.R. and Majumder, R. and Chaudhuri, B.},
journal={IEEE Transactions on Power Systems},
title={System Frequency Support Through Multi-Terminal DC (MTDC) Grids},
year={2013},
month={Feb},
volume={28},
number={1},
pages={347-356}}


